The Most Metal-Poor Stars. II. Chemical Abundances of 190 Metal-Poor Stars Including 10 New Stars With [Fe/H] < -3.5

We present a homogeneous chemical abundance analysis of 16 elements in 190 metal-poor Galactic halo stars (38 program and 152 literature objects). The sample includes 171 stars with [Fe/H] < -2.5, of which 86 are extremely metal poor, [Fe/H] < -3.0. Our program stars include ten new objects with [Fe/H] < -3.5. We identify a sample of "normal" metal-poor stars and measure the trends between [X/Fe] and [Fe/H], as well as the dispersion about the mean trend for this sample. Using this mean trend, we identify objects that are chemically peculiar relative to "normal" stars at the same metallicity. These chemically unusual stars include CEMP-no objects, one star with high [Si/Fe], another with high [Ba/Sr], and one with unusually low [X/Fe] for all elements heavier than Na. The Sr and Ba abundances indicate that there may be two nucleosynthetic processes at lowest metallicity that are distinct from the main r-process. Finally, for many elements, we find a significant trend between [X/Fe] versus Teff which likely reflects non-LTE and/or 3D effects. Such trends demonstrate that care must be exercised when using abundance measurements in metal-poor stars to constrain chemical evolution and/or nucleosynthesis predictions.

==> tab3.tex <==
\begin{deluxetable}{lrcccr}
\tabletypesize{\small}
%\rotate
\tablecolumns{6} 
\tablewidth{0pc} 
\tablecaption{Chemical Abundances (Na-Ba) for the Program Stars \label{tab:abund}}
\tablehead{ 
\colhead{Star} & 
\colhead{A(X)} & 
\colhead{N$_{\rm lines}$} & 
\colhead{s.e.$_{\rm log \epsilon}$\tablenotemark{a}} & 
\colhead{Total Error\tablenotemark{b}} & 
\colhead{[X/Fe]} \\
\colhead{(1)} &
\colhead{(2)} &
\colhead{(3)} &
\colhead{(4)} &
\colhead{(5)} &
\colhead{(6)} 
}
\startdata
 \noalign{\vskip +0.5ex}
 \multicolumn{6}{c}{Na} \cr
 \noalign{\vskip  .8ex}% 
 \hline
 \noalign{\vskip-2ex}\\
 52972-1213-507                 &    4.86 &      2 &     0.32 &     0.33 &    1.60 \\ 
 53327-2044-515\tablenotemark{c}&    2.35 &      1 &   \ldots &   \ldots &    0.11 \\ 
 53327-2044-515\tablenotemark{d}&    2.32 &      1 &   \ldots &   \ldots &    0.17 \\ 
 53436-1996-093                 &    2.58 &      1 &   \ldots &   \ldots & $-$0.13 \\ 
 54142-2667-094                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
BS~16545-089                    &    2.64 &      2 &     0.00 &     0.14 & $-$0.16 \\ 
CS~30336-049                    &    2.13 &      2 &     0.01 &     0.15 & $-$0.01 \\ 
HE~0049-3948                    &    2.49 &      2 &     0.20 &     0.20 & $-$0.08 \\ 
HE~0057-5959                    &    4.14 &      2 &     0.06 &     0.17 &    1.98 \\ 
HE~0102-1213                    &    2.94 &      1 &   \ldots &   \ldots & $-$0.02 \\ 
HE~0146-1548                    &    3.94 &      2 &     0.12 &     0.19 &    1.17 \\ 
HE~0207-1423                    &    3.90 &      1 &   \ldots &   \ldots &    0.61 \\ 
HE~0228-4047\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0231-6025                    &    3.15 &      2 &     0.10 &     0.15 &    0.01 \\ 
HE~0253-1331                    &    3.06 &      2 &     0.06 &     0.16 & $-$0.17 \\ 
HE~0314-1739                    &    2.93 &      1 &   \ldots &   \ldots & $-$0.45 \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{c}   &    3.30 &      2 &     0.08 &     0.15 & $-$0.07 \\ 
HE~1055+0104\tablenotemark{d}   &    3.30 &      2 &     0.09 &     0.15 & $-$0.06 \\ 
HE~1116-0054\tablenotemark{c}   &    2.52 &      2 &     0.04 &     0.15 & $-$0.23 \\ 
HE~1116-0054\tablenotemark{d}   &    2.53 &      2 &     0.04 &     0.15 & $-$0.23 \\ 
HE~1142-1422                    &    3.34 &      2 &     0.04 &     0.15 & $-$0.06 \\ 
HE~1201-1512\tablenotemark{c}   &    2.03 &      2 &     0.03 &     0.15 & $-$0.35 \\ 
HE~1201-1512\tablenotemark{d}   &    2.00 &      2 &     0.03 &     0.15 & $-$0.32 \\ 
HE~1204-0744                    &    3.48 &      1 &   \ldots &   \ldots & $-$0.05 \\ 
HE~1207-3108                    &    4.09 &      2 &     0.24 &     0.24 &    0.54 \\ 
HE~1320-2952                    &    2.64 &      2 &     0.06 &     0.16 &    0.09 \\ 
HE~1346-0427\tablenotemark{c}   &    2.52 &      2 &     0.05 &     0.14 & $-$0.15 \\ 
HE~1346-0427\tablenotemark{d}   &    2.53 &      2 &     0.05 &     0.14 & $-$0.14 \\ 
HE~1402-0523\tablenotemark{c}   &    2.92 &      2 &     0.11 &     0.17 & $-$0.15 \\ 
HE~1402-0523\tablenotemark{d}   &    2.92 &      2 &     0.11 &     0.17 & $-$0.13 \\ 
HE~1506-0113                    &    4.35 &      2 &     0.07 &     0.18 &    1.65 \\ 
HE~2020-5228                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2032-5633                    &    2.61 &      2 &     0.07 &     0.15 &    0.00 \\ 
HE~2047-5612                    &    2.84 &      2 &     0.08 &     0.16 & $-$0.26 \\ 
HE~2135-1924                    &    2.89 &      2 &     0.36 &     0.37 & $-$0.04 \\ 
HE~2136-6030                    &    2.97 &      2 &     0.02 &     0.17 & $-$0.39 \\ 
HE~2139-5432                    &    4.37 &      2 &     0.05 &     0.19 &    2.15 \\ 
HE~2141-0726                    &    3.16 &      2 &     0.02 &     0.16 & $-$0.36 \\ 
HE~2142-5656                    &    4.18 &      2 &     0.01 &     0.17 &    0.81 \\ 
HE~2202-4831                    &    4.90 &      1 &   \ldots &   \ldots &    1.44 \\ 
HE~2246-2410                    &    4.69 &      2 &     0.00 &     0.19 &    1.42 \\ 
HE~2247-7400                    &    4.19 &      1 &   \ldots &   \ldots &    0.82 \\ 
\cutinhead{Mg}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    4.96 &      3 &     0.06 &     0.13 &    0.34 \\ 
 53327-2044-515\tablenotemark{c}&    3.92 &      3 &     0.05 &     0.12 &    0.32 \\ 
 53327-2044-515\tablenotemark{d}&    3.99 &      3 &     0.05 &     0.12 &    0.48 \\ 
 53436-1996-093                 &    4.27 &      2 &     0.04 &     0.15 &    0.21 \\ 
 54142-2667-094                 &    4.87 &      3 &     0.09 &     0.13 &    0.23 \\ 
BS~16545-089                    &    4.41 &      3 &     0.02 &     0.12 &    0.25 \\ 
CS~30336-049                    &    3.64 &      7 &     0.05 &     0.08 &    0.15 \\ 
HE~0049-3948                    &    4.21 &      3 &     0.03 &     0.13 &    0.29 \\ 
HE~0057-5959                    &    4.03 &      6 &     0.08 &     0.10 &    0.51 \\ 
HE~0102-1213                    &    4.38 &      4 &     0.09 &     0.11 &    0.06 \\ 
HE~0146-1548                    &    5.01 &      3 &     0.15 &     0.15 &    0.87 \\ 
HE~0207-1423                    &    5.19 &      3 &     0.03 &     0.15 &    0.54 \\ 
HE~0228-4047\tablenotemark{c}   &    4.11 &      3 &     0.07 &     0.12 &    0.26 \\ 
HE~0228-4047\tablenotemark{d}   &    4.12 &      3 &     0.07 &     0.12 &    0.26 \\ 
HE~0231-6025                    &    4.89 &      4 &     0.06 &     0.11 &    0.39 \\ 
HE~0253-1331                    &    4.84 &      4 &     0.04 &     0.11 &    0.25 \\ 
HE~0314-1739                    &    4.78 &      3 &     0.02 &     0.12 &    0.04 \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &    3.72 &      2 &     0.00 &     0.14 & $-$0.10 \\ 
HE~0945-1435\tablenotemark{d}   &    3.72 &      2 &     0.00 &     0.14 & $-$0.09 \\ 
HE~1055+0104\tablenotemark{c}   &    4.94 &      3 &     0.07 &     0.13 &    0.21 \\ 
HE~1055+0104\tablenotemark{d}   &    5.06 &      3 &     0.09 &     0.13 &    0.35 \\ 
HE~1116-0054\tablenotemark{c}   &    4.18 &      3 &     0.03 &     0.12 &    0.07 \\ 
HE~1116-0054\tablenotemark{d}   &    4.20 &      3 &     0.03 &     0.12 &    0.08 \\ 
HE~1142-1422                    &    5.16 &      4 &     0.10 &     0.12 &    0.40 \\ 
HE~1201-1512\tablenotemark{c}   &    3.94 &      4 &     0.11 &     0.11 &    0.20 \\ 
HE~1201-1512\tablenotemark{d}   &    3.96 &      4 &     0.09 &     0.11 &    0.28 \\ 
HE~1204-0744                    &    4.82 &      1 &   \ldots &   \ldots & $-$0.07 \\ 
HE~1207-3108                    &    4.52 &      6 &     0.04 &     0.10 & $-$0.38 \\ 
HE~1320-2952                    &    4.31 &      5 &     0.03 &     0.11 &    0.40 \\ 
HE~1346-0427\tablenotemark{c}   &    4.28 &      3 &     0.03 &     0.12 &    0.25 \\ 
HE~1346-0427\tablenotemark{d}   &    4.30 &      3 &     0.04 &     0.12 &    0.28 \\ 
HE~1402-0523\tablenotemark{c}   &    4.71 &      3 &     0.03 &     0.12 &    0.29 \\ 
HE~1402-0523\tablenotemark{d}   &    4.77 &      3 &     0.03 &     0.12 &    0.36 \\ 
HE~1506-0113                    &    4.95 &      4 &     0.06 &     0.13 &    0.89 \\ 
HE~2020-5228                    &    4.90 &      6 &     0.08 &     0.10 &    0.22 \\ 
HE~2032-5633                    &    4.26 &      3 &     0.03 &     0.12 &    0.29 \\ 
HE~2047-5612                    &    4.44 &      3 &     0.08 &     0.12 & $-$0.02 \\ 
HE~2135-1924                    &    4.23 &      3 &     0.00 &     0.12 & $-$0.05 \\ 
HE~2136-6030                    &    4.80 &      5 &     0.16 &     0.16 &    0.08 \\ 
HE~2139-5432                    &    5.19 &      3 &     0.09 &     0.16 &    1.61 \\ 
HE~2141-0726                    &    4.93 &      4 &     0.04 &     0.10 &    0.06 \\ 
HE~2142-5656                    &    5.07 &      3 &     0.10 &     0.13 &    0.33 \\ 
HE~2202-4831                    &    4.94 &      2 &     0.03 &     0.17 &    0.12 \\ 
HE~2246-2410                    &    4.77 &      3 &     0.14 &     0.14 &    0.13 \\ 
HE~2247-7400                    &    5.06 &      3 &     0.05 &     0.12 &    0.33 \\ 
\cutinhead{Al}                 &         &        &          &          &         \\ 
 52972-1213-507                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{c}&    2.26 &      1 &   \ldots &   \ldots & $-$0.19 \\ 
 53327-2044-515\tablenotemark{d}&    2.20 &      1 &   \ldots &   \ldots & $-$0.16 \\ 
 53436-1996-093                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 54142-2667-094                 &    2.77 &      2 &     0.10 &     0.16 & $-$0.72 \\ 
BS~16545-089                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
CS~30336-049                    &    1.58 &      2 &     0.06 &     0.15 & $-$0.77 \\ 
HE~0049-3948                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0057-5959                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0102-1213                    &    2.48 &      2 &     0.01 &     0.15 & $-$0.69 \\ 
HE~0146-1548                    &    3.13 &      1 &   \ldots &   \ldots &    0.14 \\ 
HE~0207-1423                    &    3.60 &      1 &   \ldots &   \ldots &    0.10 \\ 
HE~0228-4047\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0231-6025                    &    2.72 &      2 &     0.07 &     0.15 & $-$0.64 \\ 
HE~0253-1331                    &    2.83 &      2 &     0.00 &     0.15 & $-$0.61 \\ 
HE~0314-1739                    &    2.73 &      1 &   \ldots &   \ldots & $-$0.86 \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{c}   &    2.91 &      2 &     0.07 &     0.15 & $-$0.66 \\ 
HE~1055+0104\tablenotemark{d}   &    2.89 &      2 &     0.07 &     0.15 & $-$0.67 \\ 
HE~1116-0054\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1116-0054\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1142-1422                    &    3.03 &      2 &     0.07 &     0.14 & $-$0.57 \\ 
HE~1201-1512\tablenotemark{c}   &    1.86 &      1 &   \ldots &   \ldots & $-$0.73 \\ 
HE~1201-1512\tablenotemark{d}   &    1.81 &      1 &   \ldots &   \ldots & $-$0.72 \\ 
HE~1204-0744                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1207-3108                    &    2.57 &      2 &     0.24 &     0.24 & $-$1.19 \\ 
HE~1320-2952                    &    2.16 &      2 &     0.25 &     0.26 & $-$0.60 \\ 
HE~1346-0427\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1346-0427\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{c}   &    2.49 &      1 &   \ldots &   \ldots & $-$0.79 \\ 
HE~1402-0523\tablenotemark{d}   &    2.49 &      1 &   \ldots &   \ldots & $-$0.77 \\ 
HE~1506-0113                    &    2.38 &      1 &   \ldots &   \ldots & $-$0.53 \\ 
HE~2020-5228                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2032-5633                    &    2.31 &      1 &   \ldots &   \ldots & $-$0.51 \\ 
HE~2047-5612                    &    2.42 &      1 &   \ldots &   \ldots & $-$0.89 \\ 
HE~2135-1924                    &    2.34 &      2 &     0.05 &     0.15 & $-$0.80 \\ 
HE~2136-6030                    &    2.93 &      1 &   \ldots &   \ldots & $-$0.64 \\ 
HE~2139-5432                    &    2.79 &      1 &   \ldots &   \ldots &    0.36 \\ 
HE~2141-0726                    &    2.86 &      2 &     0.07 &     0.16 & $-$0.87 \\ 
HE~2142-5656                    &    2.96 &      1 &   \ldots &   \ldots & $-$0.62 \\ 
HE~2202-4831                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2246-2410                    &    2.65 &      2 &     0.17 &     0.19 & $-$0.83 \\ 
HE~2247-7400                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
\cutinhead{Si}                 &         &        &          &          &         \\ 
 52972-1213-507                 & $<$6.03 &      1 &   \ldots &   \ldots & $<$1.50\tablenotemark{e} \\ 
 53327-2044-515\tablenotemark{c}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{d}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53436-1996-093                 & $<$5.78 &      1 &   \ldots &   \ldots & $<$1.80\tablenotemark{e} \\ 
 54142-2667-094                 &    4.50 &      1 &   \ldots &   \ldots & $-$0.05 \\ 
BS~16545-089                    & $<$5.57 &      1 &   \ldots &   \ldots & $<$1.50\tablenotemark{e} \\ 
CS~30336-049                    &    3.84 &      1 &   \ldots &   \ldots &    0.43 \\ 
HE~0049-3948                    &    3.82 &      1 &   \ldots &   \ldots & $-$0.01 \\ 
HE~0057-5959                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0102-1213                    &    4.39 &      1 &   \ldots &   \ldots &    0.16 \\ 
HE~0146-1548                    &    4.55 &      1 &   \ldots &   \ldots &    0.50\tablenotemark{e} \\ 
HE~0207-1423                    &    5.06 &      1 &   \ldots &   \ldots &    0.50\tablenotemark{e} \\ 
HE~0228-4047\tablenotemark{c}   &    4.11 &      1 &   \ldots &   \ldots &    0.35 \\ 
HE~0228-4047\tablenotemark{d}   &    4.10 &      1 &   \ldots &   \ldots &    0.34 \\ 
HE~0231-6025                    &    4.43 &      1 &   \ldots &   \ldots &    0.02 \\ 
HE~0253-1331                    &    4.57 &      1 &   \ldots &   \ldots &    0.07 \\ 
HE~0314-1739                    &    4.55 &      1 &   \ldots &   \ldots & $-$0.10 \\ 
HE~0355-3728\tablenotemark{c}   &    4.19 &      1 &   \ldots &   \ldots &    0.10 \\ 
HE~0355-3728\tablenotemark{d}   &    4.30 &      1 &   \ldots &   \ldots &    0.20 \\ 
HE~0945-1435\tablenotemark{c}   & $<$5.74 &      1 &   \ldots &   \ldots & $<$2.00\tablenotemark{e} \\ 
HE~0945-1435\tablenotemark{d}   & $<$5.73 &      1 &   \ldots &   \ldots & $<$2.00\tablenotemark{e} \\ 
HE~1055+0104\tablenotemark{c}   &    5.10 &      1 &   \ldots &   \ldots &    0.46 \\ 
HE~1055+0104\tablenotemark{d}   &    5.12 &      1 &   \ldots &   \ldots &    0.50 \\ 
HE~1116-0054\tablenotemark{c}   & $<$5.72 &      1 &   \ldots &   \ldots & $<$1.70\tablenotemark{e} \\ 
HE~1116-0054\tablenotemark{d}   & $<$5.73 &      1 &   \ldots &   \ldots & $<$1.70\tablenotemark{e} \\ 
HE~1142-1422                    &    4.55 &      1 &   \ldots &   \ldots & $-$0.12 \\ 
HE~1201-1512\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1201-1512\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1204-0744                    &    4.46 &      1 &   \ldots &   \ldots & $-$0.34 \\ 
HE~1207-3108                    &    4.97 &      1 &   \ldots &   \ldots &    0.16 \\ 
HE~1320-2952                    &    4.50 &      1 &   \ldots &   \ldots &    0.68 \\ 
HE~1346-0427\tablenotemark{c}   & $<$5.74 &      1 &   \ldots &   \ldots & $<$1.80\tablenotemark{e} \\ 
HE~1346-0427\tablenotemark{d}   & $<$5.73 &      1 &   \ldots &   \ldots & $<$1.80\tablenotemark{e} \\ 
HE~1402-0523\tablenotemark{c}   &    4.44 &      1 &   \ldots &   \ldots &    0.10 \\ 
HE~1402-0523\tablenotemark{d}   &    4.41 &      1 &   \ldots &   \ldots &    0.09 \\ 
HE~1506-0113                    &    4.47 &      1 &   \ldots &   \ldots &    0.50\tablenotemark{e} \\ 
HE~2020-5228                    &    4.68 &      1 &   \ldots &   \ldots &    0.10 \\ 
HE~2032-5633                    &    4.21 &      1 &   \ldots &   \ldots &    0.33 \\ 
HE~2047-5612                    &    4.42 &      1 &   \ldots &   \ldots &    0.05 \\ 
HE~2135-1924                    &    4.16 &      1 &   \ldots &   \ldots & $-$0.04 \\ 
HE~2136-6030                    &    5.84 &      1 &   \ldots &   \ldots &    1.21 \\ 
HE~2139-5432                    &    4.49 &      1 &   \ldots &   \ldots &    1.00\tablenotemark{e} \\ 
HE~2141-0726                    &    4.74 &      1 &   \ldots &   \ldots & $-$0.05 \\ 
HE~2142-5656                    &    4.99 &      1 &   \ldots &   \ldots &    0.35\tablenotemark{e} \\ 
HE~2202-4831                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2246-2410                    &    4.57 &      1 &   \ldots &   \ldots &    0.02 \\ 
HE~2247-7400                    &    5.44 & \ldots &   \ldots &   \ldots &    0.80\tablenotemark{e} \\ 
\cutinhead{Ca}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    3.92 &      1 &   \ldots &   \ldots &    0.56 \\ 
 53327-2044-515\tablenotemark{c}&    2.51 &      1 &   \ldots &   \ldots &    0.17 \\ 
 53327-2044-515\tablenotemark{d}&    2.45 &      1 &   \ldots &   \ldots &    0.20 \\ 
 53436-1996-093                 &    3.11 &      1 &   \ldots &   \ldots &    0.30 \\ 
 54142-2667-094                 &    3.71 &      3 &     0.17 &     0.18 &    0.34 \\ 
BS~16545-089                    &    3.43 &      4 &     0.04 &     0.10 &    0.53 \\ 
CS~30336-049                    &    2.46 &      4 &     0.14 &     0.15 &    0.22 \\ 
HE~0049-3948                    &    2.77 &      1 &   \ldots &   \ldots &    0.11 \\ 
HE~0057-5959                    &    2.91 &      4 &     0.13 &     0.14 &    0.65 \\ 
HE~0102-1213                    &    3.48 &      5 &     0.07 &     0.10 &    0.42 \\ 
HE~0146-1548                    &    3.10 &      2 &     0.10 &     0.15 &    0.22 \\ 
HE~0207-1423                    &    3.82 &      6 &     0.04 &     0.12 &    0.43 \\ 
HE~0228-4047\tablenotemark{c}   &    2.98 &      1 &   \ldots &   \ldots &    0.39 \\ 
HE~0228-4047\tablenotemark{d}   &    2.98 &      1 &   \ldots &   \ldots &    0.39 \\ 
HE~0231-6025                    &    3.66 &      2 &     0.08 &     0.15 &    0.42 \\ 
HE~0253-1331                    &    3.91 &      3 &     0.06 &     0.12 &    0.58 \\ 
HE~0314-1739                    &    3.97 &      1 &   \ldots &   \ldots &    0.49 \\ 
HE~0355-3728\tablenotemark{c}   &    3.20 &      1 &   \ldots &   \ldots &    0.28 \\ 
HE~0355-3728\tablenotemark{d}   &    3.67 &      1 &   \ldots &   \ldots &    0.74 \\ 
HE~0945-1435\tablenotemark{c}   &    2.83 &      2 &     0.16 &     0.17 &    0.26 \\ 
HE~0945-1435\tablenotemark{d}   &    2.82 &      2 &     0.16 &     0.16 &    0.26 \\ 
HE~1055+0104\tablenotemark{c}   &    3.87 &      4 &     0.02 &     0.11 &    0.40 \\ 
HE~1055+0104\tablenotemark{d}   &    3.89 &      4 &     0.03 &     0.11 &    0.44 \\ 
HE~1116-0054\tablenotemark{c}   &    3.15 &      2 &     0.08 &     0.14 &    0.30 \\ 
HE~1116-0054\tablenotemark{d}   &    3.15 &      2 &     0.08 &     0.14 &    0.30 \\ 
HE~1142-1422                    &    3.89 &      2 &     0.00 &     0.15 &    0.40 \\ 
HE~1201-1512\tablenotemark{c}   &    2.53 &      1 &   \ldots &   \ldots &    0.05 \\ 
HE~1201-1512\tablenotemark{d}   &    2.49 &      1 &   \ldots &   \ldots &    0.07 \\ 
HE~1204-0744                    &    4.07 &      2 &     0.10 &     0.14 &    0.45 \\ 
HE~1207-3108                    &    3.39 &      8 &     0.06 &     0.11 & $-$0.25 \\ 
HE~1320-2952                    &    2.95 &      4 &     0.03 &     0.12 &    0.31 \\ 
HE~1346-0427\tablenotemark{c}   &    3.14 &      5 &     0.04 &     0.09 &    0.37 \\ 
HE~1346-0427\tablenotemark{d}   &    3.13 &      5 &     0.03 &     0.09 &    0.37 \\ 
HE~1402-0523\tablenotemark{c}   &    3.51 &      2 &     0.03 &     0.14 &    0.35 \\ 
HE~1402-0523\tablenotemark{d}   &    3.53 &      2 &     0.05 &     0.14 &    0.38 \\ 
HE~1506-0113                    &    3.00 &      5 &     0.08 &     0.11 &    0.19 \\ 
HE~2020-5228                    &    3.85 &      4 &     0.06 &     0.12 &    0.44 \\ 
HE~2032-5633                    &    3.32 &      1 &   \ldots &   \ldots &    0.61 \\ 
HE~2047-5612                    &    3.37 &      4 &     0.13 &     0.14 &    0.16 \\ 
HE~2135-1924                    &    3.77 &      2 &     0.56 &     0.56 &    0.74 \\ 
HE~2136-6030                    &    3.97 &      2 &     0.07 &     0.15 &    0.51 \\ 
HE~2139-5432                    & $<$3.02 &      1 &   \ldots &   \ldots & $<$0.70 \\ 
HE~2141-0726                    &    3.78 &      3 &     0.14 &     0.14 &    0.16 \\ 
HE~2142-5656                    &    3.77 &      7 &     0.03 &     0.10 &    0.30 \\ 
HE~2202-4831                    &    3.72 &      6 &     0.06 &     0.13 &    0.17 \\ 
HE~2246-2410                    &    3.78 &      4 &     0.06 &     0.12 &    0.40 \\ 
HE~2247-7400                    &    3.91 &      7 &     0.06 &     0.11 &    0.43 \\ 
\cutinhead{Sc}                 &         &        &          &          &         \\ 
 52972-1213-507                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{c}& $-$0.53 &      1 &   \ldots &   \ldots &    0.32 \\ 
 53327-2044-515\tablenotemark{d}& $-$1.01 &      1 &   \ldots &   \ldots & $-$0.07 \\ 
 53436-1996-093                 &    0.06 &      1 &   \ldots &   \ldots &    0.44 \\ 
 54142-2667-094                 &    0.48 &      2 &     0.03 &     0.20 &    0.30 \\ 
BS~16545-089                    & $-$0.12 &      1 &   \ldots &   \ldots &    0.17 \\ 
CS~30336-049                    & $-$0.98 &      2 &     0.00 &     0.19 & $-$0.03 \\ 
HE~0049-3948                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0057-5959                    & $-$0.76 &      2 &     0.03 &     0.20 &    0.17 \\ 
HE~0102-1213                    & $-$0.03 &      2 &     0.05 &     0.19 &    0.10 \\ 
HE~0146-1548                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0207-1423                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0231-6025                    &    0.32 &      1 &   \ldots &   \ldots &    0.27 \\ 
HE~0253-1331                    &    0.72 &      1 &   \ldots &   \ldots &    0.58 \\ 
HE~0314-1739                    &    0.44 &      1 &   \ldots &   \ldots &    0.15 \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   & $-$0.47 &      1 &   \ldots &   \ldots &    0.15 \\ 
HE~0945-1435\tablenotemark{d}   & $-$0.71 &      1 &   \ldots &   \ldots & $-$0.08 \\ 
HE~1055+0104\tablenotemark{c}   &    0.52 &      2 &     0.05 &     0.19 &    0.24 \\ 
HE~1055+0104\tablenotemark{d}   &    0.30 &      2 &     0.04 &     0.19 &    0.04 \\ 
HE~1116-0054\tablenotemark{c}   & $-$0.06 &      1 &   \ldots &   \ldots &    0.28 \\ 
HE~1116-0054\tablenotemark{d}   & $-$0.24 &      1 &   \ldots &   \ldots &    0.09 \\ 
HE~1142-1422                    &    0.53 &      2 &     0.09 &     0.19 &    0.22 \\ 
HE~1201-1512\tablenotemark{c}   & $-$0.40 &      1 &   \ldots &   \ldots &    0.31 \\ 
HE~1201-1512\tablenotemark{d}   & $-$0.86 &      1 &   \ldots &   \ldots & $-$0.09 \\ 
HE~1204-0744                    &    0.35 &      1 &   \ldots &   \ldots & $-$0.09 \\ 
HE~1207-3108                    & $-$0.09 &      2 &     0.02 &     0.23 & $-$0.55 \\ 
HE~1320-2952                    & $-$0.54 &      2 &     0.04 &     0.21 &    0.00 \\ 
HE~1346-0427\tablenotemark{c}   & $-$0.21 &      1 &   \ldots &   \ldots &    0.21 \\ 
HE~1346-0427\tablenotemark{d}   & $-$0.47 &      1 &   \ldots &   \ldots & $-$0.04 \\ 
HE~1402-0523\tablenotemark{c}   &    0.42 &      2 &     0.11 &     0.21 &    0.44 \\ 
HE~1402-0523\tablenotemark{d}   &    0.23 &      2 &     0.11 &     0.21 &    0.27 \\ 
HE~1506-0113                    &$<-$0.49 &      1 &   \ldots &   \ldots &$<-$0.10 \\ 
HE~2020-5228                    &    0.47 &      1 &   \ldots &   \ldots &    0.25 \\ 
HE~2032-5633                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2047-5612                    &    0.19 &      1 &   \ldots &   \ldots &    0.18 \\ 
HE~2135-1924                    & $-$0.10 &      1 &   \ldots &   \ldots &    0.06 \\ 
HE~2136-6030                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2139-5432                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2141-0726                    &    0.50 &      1 &   \ldots &   \ldots &    0.07 \\ 
HE~2142-5656                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2202-4831                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2246-2410                    &    0.46 &      1 &   \ldots &   \ldots &    0.27 \\ 
HE~2247-7400                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
\cutinhead{TiI}                &         &        &          &          &         \\ 
 52972-1213-507                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{c}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{d}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53436-1996-093                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 54142-2667-094                 &    3.01 &      2 &     0.02 &     0.16 &    1.03 \\ 
BS~16545-089                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
CS~30336-049                    &    1.02 &      2 &     0.05 &     0.16 &    0.17 \\ 
HE~0049-3948                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0057-5959                    &    1.55 &      1 &   \ldots &   \ldots &    0.68 \\ 
HE~0102-1213                    &    2.43 &      3 &     0.05 &     0.13 &    0.76 \\ 
HE~0146-1548                    &    1.65 &      4 &     0.10 &     0.12 &    0.17 \\ 
HE~0207-1423                    &    2.21 &      3 &     0.09 &     0.14 &    0.22 \\ 
HE~0228-4047\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0231-6025                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0253-1331                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0314-1739                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1116-0054\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1116-0054\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1142-1422                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1201-1512\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1201-1512\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1204-0744                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1207-3108                    &    1.96 &      2 &     0.06 &     0.17 & $-$0.29 \\ 
HE~1320-2952                    &    1.79 &      3 &     0.04 &     0.16 &    0.54 \\ 
HE~1346-0427\tablenotemark{c}   &    2.18 &      1 &   \ldots &   \ldots &    0.80 \\ 
HE~1346-0427\tablenotemark{d}   &    2.17 &      1 &   \ldots &   \ldots &    0.80 \\ 
HE~1402-0523\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1506-0113                    &    1.94 &      4 &     0.04 &     0.13 &    0.53 \\ 
HE~2020-5228                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2032-5633                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2047-5612                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2135-1924                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2136-6030                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2139-5432                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2141-0726                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2142-5656                    &    2.39 &      4 &     0.09 &     0.12 &    0.31 \\ 
HE~2202-4831                    &    2.38 &      2 &     0.03 &     0.17 &    0.21 \\ 
HE~2246-2410                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2247-7400                    &    2.43 &      3 &     0.07 &     0.14 &    0.34 \\ 
\cutinhead{TiII}               &         &        &          &          &         \\ 
 52972-1213-507                 &    2.35 &      5 &     0.08 &     0.17 &    0.38 \\ 
 53327-2044-515\tablenotemark{c}&    1.45 &      3 &     0.11 &     0.16 &    0.50 \\ 
 53327-2044-515\tablenotemark{d}&    0.90 &      3 &     0.13 &     0.18 &    0.04 \\ 
 53436-1996-093                 &    1.87 &      8 &     0.04 &     0.15 &    0.45 \\ 
 54142-2667-094                 &    2.38 &     11 &     0.05 &     0.14 &    0.39 \\ 
BS~16545-089                    &    1.95 &     11 &     0.01 &     0.13 &    0.45 \\ 
CS~30336-049                    &    0.87 &     16 &     0.03 &     0.16 &    0.02 \\ 
HE~0049-3948                    &    1.67 &      8 &     0.06 &     0.15 &    0.40 \\ 
HE~0057-5959                    &    1.27 &     13 &     0.03 &     0.13 &    0.40 \\ 
HE~0102-1213                    &    2.02 &     12 &     0.03 &     0.13 &    0.35 \\ 
HE~0146-1548                    &    1.67 &     11 &     0.05 &     0.16 &    0.18 \\ 
HE~0207-1423                    &    2.31 &      9 &     0.08 &     0.15 &    0.31 \\ 
HE~0228-4047\tablenotemark{c}   &    1.77 &      7 &     0.04 &     0.13 &    0.57 \\ 
HE~0228-4047\tablenotemark{d}   &    1.58 &      7 &     0.04 &     0.13 &    0.38 \\ 
HE~0231-6025                    &    2.50 &      8 &     0.05 &     0.16 &    0.65 \\ 
HE~0253-1331                    &    2.56 &      9 &     0.04 &     0.14 &    0.62 \\ 
HE~0314-1739                    &    2.45 &     11 &     0.06 &     0.14 &    0.36 \\ 
HE~0355-3728\tablenotemark{c}   &    2.42 &      4 &     0.13 &     0.18 &    0.89 \\ 
HE~0355-3728\tablenotemark{d}   &    2.49 &      4 &     0.13 &     0.20 &    0.95 \\ 
HE~0945-1435\tablenotemark{c}   &    1.50 &      2 &     0.14 &     0.18 &    0.33 \\ 
HE~0945-1435\tablenotemark{d}   &    1.26 &      2 &     0.15 &     0.19 &    0.09 \\ 
HE~1055+0104\tablenotemark{c}   &    2.62 &     15 &     0.03 &     0.13 &    0.54 \\ 
HE~1055+0104\tablenotemark{d}   &    2.39 &     15 &     0.03 &     0.13 &    0.32 \\ 
HE~1116-0054\tablenotemark{c}   &    1.86 &      8 &     0.04 &     0.14 &    0.40 \\ 
HE~1116-0054\tablenotemark{d}   &    1.68 &      8 &     0.04 &     0.14 &    0.21 \\ 
HE~1142-1422                    &    2.62 &     15 &     0.03 &     0.13 &    0.52 \\ 
HE~1201-1512\tablenotemark{c}   &    1.42 &      6 &     0.03 &     0.15 &    0.33 \\ 
HE~1201-1512\tablenotemark{d}   &    0.93 &      6 &     0.04 &     0.15 & $-$0.10 \\ 
HE~1204-0744                    &    2.42 &      8 &     0.11 &     0.18 &    0.18 \\ 
HE~1207-3108                    &    1.94 &     16 &     0.03 &     0.17 & $-$0.31 \\ 
HE~1320-2952                    &    1.48 &     17 &     0.03 &     0.15 &    0.22 \\ 
HE~1346-0427\tablenotemark{c}   &    1.74 &      9 &     0.03 &     0.14 &    0.36 \\ 
HE~1346-0427\tablenotemark{d}   &    1.48 &      9 &     0.03 &     0.14 &    0.11 \\ 
HE~1402-0523\tablenotemark{c}   &    2.35 &     12 &     0.04 &     0.15 &    0.57 \\ 
HE~1402-0523\tablenotemark{d}   &    2.15 &     12 &     0.04 &     0.15 &    0.39 \\ 
HE~1506-0113                    &    1.86 &     11 &     0.04 &     0.14 &    0.44 \\ 
HE~2020-5228                    &    2.28 &      9 &     0.06 &     0.16 &    0.25 \\ 
HE~2032-5633                    &    1.71 &      5 &     0.08 &     0.15 &    0.39 \\ 
HE~2047-5612                    &    2.05 &     12 &     0.03 &     0.14 &    0.24 \\ 
HE~2135-1924                    &    1.84 &      6 &     0.02 &     0.15 &    0.21 \\ 
HE~2136-6030                    &    2.47 &      9 &     0.04 &     0.16 &    0.40 \\ 
HE~2139-5432                    &    1.24 &      5 &     0.05 &     0.17 &    0.31 \\ 
HE~2141-0726                    &    2.47 &     11 &     0.04 &     0.13 &    0.25 \\ 
HE~2142-5656                    &    2.27 &     12 &     0.05 &     0.15 &    0.18 \\ 
HE~2202-4831                    &    2.63 &     10 &     0.09 &     0.16 &    0.46 \\ 
HE~2246-2410                    &    2.31 &      9 &     0.04 &     0.16 &    0.32 \\ 
HE~2247-7400                    &    2.21 &      8 &     0.06 &     0.17 &    0.13 \\ 
\cutinhead{Cr}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    2.39 &      1 &   \ldots &   \ldots & $-$0.27 \\ 
 53327-2044-515\tablenotemark{c}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{d}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53436-1996-093                 &    2.15 &      4 &     0.08 &     0.10 &    0.05 \\ 
 54142-2667-094                 &    2.54 &      3 &     0.01 &     0.14 & $-$0.14 \\ 
BS~16545-089                    &    2.07 &      3 &     0.06 &     0.12 & $-$0.12 \\ 
CS~30336-049                    &    1.06 &      5 &     0.08 &     0.11 & $-$0.48 \\ 
HE~0049-3948                    &    2.19 &      2 &     0.40 &     0.40 &    0.23 \\ 
HE~0057-5959                    &    1.06 &      1 &   \ldots &   \ldots & $-$0.50 \\ 
HE~0102-1213                    &    2.23 &      4 &     0.10 &     0.12 & $-$0.13 \\ 
HE~0146-1548                    &    1.79 &      3 &     0.08 &     0.12 & $-$0.38 \\ 
HE~0207-1423                    &    2.78 &      3 &     0.13 &     0.14 &    0.09 \\ 
HE~0228-4047\tablenotemark{c}   &    1.88 &      2 &     0.06 &     0.14 & $-$0.01 \\ 
HE~0228-4047\tablenotemark{d}   &    1.89 &      2 &     0.06 &     0.14 &    0.00 \\ 
HE~0231-6025                    &    2.52 &      1 &   \ldots &   \ldots & $-$0.02 \\ 
HE~0253-1331                    &    2.55 &      3 &     0.06 &     0.13 & $-$0.08 \\ 
HE~0314-1739                    &    2.60 &      3 &     0.07 &     0.14 & $-$0.18 \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &    1.63 &      3 &     0.06 &     0.12 & $-$0.24 \\ 
HE~0945-1435\tablenotemark{d}   &    1.63 &      3 &     0.06 &     0.12 & $-$0.23 \\ 
HE~1055+0104\tablenotemark{c}   &    2.54 &      4 &     0.09 &     0.12 & $-$0.23 \\ 
HE~1055+0104\tablenotemark{d}   &    2.52 &      4 &     0.08 &     0.12 & $-$0.23 \\ 
HE~1116-0054\tablenotemark{c}   &    2.08 &      4 &     0.05 &     0.11 & $-$0.07 \\ 
HE~1116-0054\tablenotemark{d}   &    2.09 &      4 &     0.05 &     0.11 & $-$0.07 \\ 
HE~1142-1422                    &    2.80 &      2 &     0.02 &     0.14 &    0.01 \\ 
HE~1201-1512\tablenotemark{c}   &    1.28 &      1 &   \ldots &   \ldots & $-$0.50 \\ 
HE~1201-1512\tablenotemark{d}   &    1.24 &      1 &   \ldots &   \ldots & $-$0.48 \\ 
HE~1204-0744                    &    2.97 &      3 &     0.26 &     0.27 &    0.04 \\ 
HE~1207-3108                    &    2.53 &      5 &     0.09 &     0.10 & $-$0.41 \\ 
HE~1320-2952                    &    1.60 &      4 &     0.09 &     0.13 & $-$0.34 \\ 
HE~1346-0427\tablenotemark{c}   &    1.85 &      4 &     0.02 &     0.10 & $-$0.22 \\ 
HE~1346-0427\tablenotemark{d}   &    1.85 &      4 &     0.02 &     0.10 & $-$0.21 \\ 
HE~1402-0523\tablenotemark{c}   &    2.31 &      3 &     0.03 &     0.14 & $-$0.16 \\ 
HE~1402-0523\tablenotemark{d}   &    2.31 &      3 &     0.03 &     0.14 & $-$0.14 \\ 
HE~1506-0113                    &    1.96 &      3 &     0.07 &     0.12 & $-$0.15 \\ 
HE~2020-5228                    &    2.48 &      2 &     0.07 &     0.17 & $-$0.23 \\ 
HE~2032-5633                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2047-5612                    &    2.52 &      3 &     0.24 &     0.24 &    0.02 \\ 
HE~2135-1924                    &    1.96 &      1 &   \ldots &   \ldots & $-$0.37 \\ 
HE~2136-6030                    &    2.57 &      3 &     0.11 &     0.14 & $-$0.19 \\ 
HE~2139-5432                    &    1.96 &      1 &   \ldots &   \ldots &    0.34 \\ 
HE~2141-0726                    &    2.84 &      4 &     0.04 &     0.12 & $-$0.08 \\ 
HE~2142-5656                    &    2.59 &      3 &     0.16 &     0.17 & $-$0.19 \\ 
HE~2202-4831                    &    2.93 &      2 &     0.07 &     0.14 &    0.08 \\ 
HE~2246-2410                    &    2.40 &      2 &     0.10 &     0.17 & $-$0.27 \\ 
HE~2247-7400                    &    2.66 &      3 &     0.12 &     0.14 & $-$0.11 \\ 
\cutinhead{Mn}                 &         &        &          &          &         \\ 
 52972-1213-507                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{c}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{d}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53436-1996-093                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 54142-2667-094                 &    2.09 &      1 &   \ldots &   \ldots & $-$0.38 \\ 
BS~16545-089                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
CS~30336-049                    &    0.42 &      3 &     0.03 &     0.14 & $-$0.91 \\ 
HE~0049-3948                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0057-5959                    & $<$2.19 &      1 &   \ldots &   \ldots & $<$0.84 \\ 
HE~0102-1213                    &    1.49 &      2 &     0.04 &     0.15 & $-$0.66 \\ 
HE~0146-1548                    &    1.38 &      1 &   \ldots &   \ldots & $-$0.59 \\ 
HE~0207-1423                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0231-6025                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0253-1331                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0314-1739                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{c}   &    1.93 &      2 &     0.12 &     0.16 & $-$0.63 \\ 
HE~1055+0104\tablenotemark{d}   &    1.92 &      2 &     0.12 &     0.16 & $-$0.62 \\ 
HE~1116-0054\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1116-0054\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1142-1422                    &    2.17 &      3 &     0.11 &     0.13 & $-$0.42 \\ 
HE~1201-1512\tablenotemark{c}   &    0.98 &      1 &   \ldots &   \ldots & $-$0.59 \\ 
HE~1201-1512\tablenotemark{d}   &    0.93 &      1 &   \ldots &   \ldots & $-$0.58 \\ 
HE~1204-0744                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1207-3108                    &    2.38 &      3 &     0.12 &     0.14 & $-$0.35 \\ 
HE~1320-2952                    &    0.95 &      3 &     0.08 &     0.16 & $-$0.78 \\ 
HE~1346-0427\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1346-0427\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1506-0113                    &    1.57 &      1 &   \ldots &   \ldots & $-$0.32 \\ 
HE~2020-5228                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2032-5633                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2047-5612                    &    1.68 &      2 &     0.03 &     0.18 & $-$0.61 \\ 
HE~2135-1924                    &    1.71 &      1 &   \ldots &   \ldots & $-$0.41 \\ 
HE~2136-6030                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2139-5432                    & $<$0.83 &      1 &   \ldots &   \ldots &$<-$0.58 \\ 
HE~2141-0726                    &    2.17 &      1 &   \ldots &   \ldots & $-$0.54 \\ 
HE~2142-5656                    &    1.93 &      1 &   \ldots &   \ldots & $-$0.63 \\ 
HE~2202-4831                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2246-2410                    &    2.12 &      2 &     0.04 &     0.17 & $-$0.35 \\ 
HE~2247-7400                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
\cutinhead{\fei}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    4.52 &     29 &     0.03 &     0.15 & $-$2.98 \\ 
 53327-2044-515\tablenotemark{c}&    3.50 &     29 &     0.03 &     0.12 & $-$4.00 \\ 
 53327-2044-515\tablenotemark{d}&    3.41 &     29 &     0.02 &     0.14 & $-$4.09 \\ 
 53436-1996-093                 &    3.97 &     17 &     0.02 &     0.12 & $-$3.53 \\ 
 54142-2667-094                 &    4.54 &     41 &     0.02 &     0.13 & $-$2.96 \\ 
BS~16545-089                    &    4.06 &     24 &     0.01 &     0.11 & $-$3.44 \\ 
CS~30336-049                    &    3.40 &     80 &     0.02 &     0.17 & $-$4.10 \\ 
HE~0049-3948                    &    3.82 &     35 &     0.02 &     0.12 & $-$3.68 \\ 
HE~0057-5959                    &    3.42 &     45 &     0.02 &     0.14 & $-$4.08 \\ 
HE~0102-1213                    &    4.22 &     59 &     0.02 &     0.11 & $-$3.28 \\ 
HE~0146-1548                    &    4.04 &     66 &     0.02 &     0.16 & $-$3.46 \\ 
HE~0207-1423                    &    4.55 &     47 &     0.02 &     0.16 & $-$2.95 \\ 
HE~0228-4047\tablenotemark{c}   &    3.75 &     26 &     0.02 &     0.11 & $-$3.75 \\ 
HE~0228-4047\tablenotemark{d}   &    3.75 &     26 &     0.02 &     0.11 & $-$3.75 \\ 
HE~0231-6025                    &    4.40 &     23 &     0.04 &     0.14 & $-$3.10 \\ 
HE~0253-1331                    &    4.49 &     47 &     0.02 &     0.12 & $-$3.01 \\ 
HE~0314-1739                    &    4.64 &     43 &     0.02 &     0.12 & $-$2.86 \\ 
HE~0355-3728\tablenotemark{c}   &    4.09 &     14 &     0.05 &     0.16 & $-$3.41 \\ 
HE~0355-3728\tablenotemark{d}   &    4.09 &     14 &     0.05 &     0.16 & $-$3.41 \\ 
HE~0945-1435\tablenotemark{c}   &    3.73 &     15 &     0.01 &     0.10 & $-$3.77 \\ 
HE~0945-1435\tablenotemark{d}   &    3.72 &     15 &     0.01 &     0.10 & $-$3.78 \\ 
HE~1055+0104\tablenotemark{c}   &    4.63 &     67 &     0.02 &     0.12 & $-$2.87 \\ 
HE~1055+0104\tablenotemark{d}   &    4.61 &     67 &     0.02 &     0.11 & $-$2.89 \\ 
HE~1116-0054\tablenotemark{c}   &    4.01 &     37 &     0.03 &     0.13 & $-$3.49 \\ 
HE~1116-0054\tablenotemark{d}   &    4.02 &     37 &     0.03 &     0.13 & $-$3.48 \\ 
HE~1142-1422                    &    4.66 &     51 &     0.02 &     0.10 & $-$2.84 \\ 
HE~1201-1512\tablenotemark{c}   &    3.64 &     45 &     0.02 &     0.10 & $-$3.86 \\ 
HE~1201-1512\tablenotemark{d}   &    3.58 &     45 &     0.01 &     0.12 & $-$3.92 \\ 
HE~1204-0744                    &    4.79 &     33 &     0.03 &     0.13 & $-$2.71 \\ 
HE~1207-3108                    &    4.80 &    102 &     0.02 &     0.15 & $-$2.70 \\ 
HE~1320-2952                    &    3.81 &     69 &     0.02 &     0.18 & $-$3.69 \\ 
HE~1346-0427\tablenotemark{c}   &    3.93 &     30 &     0.02 &     0.09 & $-$3.57 \\ 
HE~1346-0427\tablenotemark{d}   &    3.92 &     30 &     0.02 &     0.10 & $-$3.58 \\ 
HE~1402-0523\tablenotemark{c}   &    4.33 &     42 &     0.02 &     0.14 & $-$3.17 \\ 
HE~1402-0523\tablenotemark{d}   &    4.31 &     42 &     0.02 &     0.14 & $-$3.19 \\ 
HE~1506-0113                    &    3.96 &     87 &     0.01 &     0.15 & $-$3.54 \\ 
HE~2020-5228                    &    4.57 &     35 &     0.03 &     0.14 & $-$2.93 \\ 
HE~2032-5633                    &    3.87 &     19 &     0.03 &     0.13 & $-$3.63 \\ 
HE~2047-5612                    &    4.36 &     43 &     0.03 &     0.14 & $-$3.14 \\ 
HE~2135-1924                    &    4.19 &     36 &     0.01 &     0.13 & $-$3.31 \\ 
HE~2136-6030                    &    4.62 &     30 &     0.04 &     0.15 & $-$2.88 \\ 
HE~2139-5432                    &    3.48 &     33 &     0.04 &     0.16 & $-$4.02 \\ 
HE~2141-0726                    &    4.78 &     53 &     0.02 &     0.11 & $-$2.72 \\ 
HE~2142-5656                    &    4.63 &     62 &     0.02 &     0.15 & $-$2.87 \\ 
HE~2202-4831                    &    4.72 &     35 &     0.03 &     0.15 & $-$2.78 \\ 
HE~2246-2410                    &    4.54 &     38 &     0.02 &     0.14 & $-$2.96 \\ 
HE~2247-7400                    &    4.63 &     47 &     0.03 &     0.16 & $-$2.87 \\ 
\cutinhead{\feii}                &         &        &          &          &         \\ 
 52972-1213-507                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{c}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{d}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53436-1996-093                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 54142-2667-094                 &    4.60 &      1 &   \ldots &   \ldots & $-$2.90 \\ 
BS~16545-089                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
CS~30336-049                    &    3.40 &      5 &     0.10 &     0.15 & $-$4.10 \\ 
HE~0049-3948                    &    3.99 &      1 &   \ldots &   \ldots & $-$3.51 \\ 
HE~0057-5959                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0102-1213                    &    4.47 &      2 &     0.28 &     0.30 & $-$3.03 \\ 
HE~0146-1548                    &    4.17 &      3 &     0.03 &     0.15 & $-$3.33 \\ 
HE~0207-1423                    &    4.63 &      4 &     0.14 &     0.18 & $-$2.87 \\ 
HE~0228-4047\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0231-6025                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0253-1331                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0314-1739                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{c}   &    4.54 &      1 &   \ldots &   \ldots & $-$2.96 \\ 
HE~1055+0104\tablenotemark{d}   &    4.31 &      1 &   \ldots &   \ldots & $-$3.19 \\ 
HE~1116-0054\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1116-0054\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1142-1422                    &    4.86 &      3 &     0.08 &     0.15 & $-$2.64 \\ 
HE~1201-1512\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1201-1512\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1204-0744                    &    5.74 &      1 &   \ldots &   \ldots & $-$1.76 \\ 
HE~1207-3108                    &    4.88 &      6 &     0.08 &     0.15 & $-$2.62 \\ 
HE~1320-2952                    &    3.88 &      3 &     0.16 &     0.28 & $-$3.62 \\ 
HE~1346-0427\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1346-0427\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1506-0113                    &    4.01 &      2 &     0.07 &     0.17 & $-$3.49 \\ 
HE~2020-5228                    &    4.69 &      2 &     0.23 &     0.25 & $-$2.81 \\ 
HE~2032-5633                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2047-5612                    &    4.37 &      1 &   \ldots &     0.11 & $-$3.13 \\ 
HE~2135-1924                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2136-6030                    &    4.86 &      1 &   \ldots &     0.10 & $-$2.64 \\ 
HE~2139-5432                    &    3.98 &      1 &   \ldots &   \ldots & $-$3.52 \\ 
HE~2141-0726                    &    4.97 &      4 &     0.10 &     0.15 & $-$2.53 \\ 
HE~2142-5656                    &    4.68 &      5 &     0.04 &     0.13 & $-$2.82 \\ 
HE~2202-4831                    &    4.95 &      3 &     0.10 &     0.17 & $-$2.55 \\ 
HE~2246-2410                    &    4.63 &      1 &   \ldots &     0.11 & $-$2.87 \\ 
HE~2247-7400                    &    4.84 &      2 &     0.24 &     0.26 & $-$2.66 \\ 
\cutinhead{Co}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    2.66 &      1 &   \ldots &   \ldots &    0.65 \\ 
 53327-2044-515\tablenotemark{c}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53327-2044-515\tablenotemark{d}&  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 53436-1996-093                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 54142-2667-094                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
BS~16545-089                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
CS~30336-049                    &    1.27 &      4 &     0.07 &     0.12 &    0.38 \\ 
HE~0049-3948                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0057-5959                    & $<$1.14 &      1 &   \ldots &   \ldots & $<$0.23 \\ 
HE~0102-1213                    &    2.35 &      2 &     0.24 &     0.25 &    0.64 \\ 
HE~0146-1548                    &    1.82 &      4 &     0.13 &     0.13 &    0.30 \\ 
HE~0207-1423                    &    1.97 &      1 &   \ldots &   \ldots & $-$0.07 \\ 
HE~0228-4047\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0228-4047\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0231-6025                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0253-1331                    &    2.42 &      1 &   \ldots &   \ldots &    0.44 \\ 
HE~0314-1739                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{c}   &    2.52 &      2 &     0.04 &     0.16 &    0.40 \\ 
HE~1055+0104\tablenotemark{d}   &    2.51 &      2 &     0.04 &     0.16 &    0.41 \\ 
HE~1116-0054\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1116-0054\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1142-1422                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1201-1512\tablenotemark{c}   &    1.96 &      1 &   \ldots &   \ldots &    0.83 \\ 
HE~1201-1512\tablenotemark{d}   &    1.89 &      1 &   \ldots &   \ldots &    0.82 \\ 
HE~1204-0744                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1207-3108                    &    1.98 &      3 &     0.07 &     0.15 & $-$0.31 \\ 
HE~1320-2952                    &    1.59 &      2 &     0.06 &     0.18 &    0.29 \\ 
HE~1346-0427\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1346-0427\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{c}   &    2.81 &      1 &   \ldots &   \ldots &    0.99 \\ 
HE~1402-0523\tablenotemark{d}   &    2.81 &      1 &   \ldots &   \ldots &    1.01 \\ 
HE~1506-0113                    &    1.93 &      4 &     0.07 &     0.11 &    0.48 \\ 
HE~2020-5228                    &    2.75 &      1 &   \ldots &   \ldots &    0.69 \\ 
HE~2032-5633                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2047-5612                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2135-1924                    &    2.62 &      1 &   \ldots &   \ldots &    0.94 \\ 
HE~2136-6030                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2139-5432                    &    1.59 &      1 &   \ldots &   \ldots &    0.62 \\ 
HE~2141-0726                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2142-5656                    &    2.31 &      4 &     0.08 &     0.10 &    0.18 \\ 
HE~2202-4831                    &    2.42 &      1 &   \ldots &   \ldots &    0.21 \\ 
HE~2246-2410                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2247-7400                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
\cutinhead{Ni}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    3.39 &      1 &   \ldots &   \ldots &    0.15 \\ 
 53327-2044-515\tablenotemark{c}&    2.35 &      2 &     0.04 &     0.15 &    0.13 \\ 
 53327-2044-515\tablenotemark{d}&    2.24 &      2 &     0.03 &     0.15 &    0.12 \\ 
 53436-1996-093                 &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
 54142-2667-094                 &    3.10 &      1 &   \ldots &   \ldots & $-$0.16 \\ 
BS~16545-089                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
CS~30336-049                    &    2.22 &      3 &     0.04 &     0.12 &    0.10 \\ 
HE~0049-3948                    &    2.84 &      1 &   \ldots &   \ldots &    0.30 \\ 
HE~0057-5959                    &    2.30 &      2 &     0.03 &     0.15 &    0.17 \\ 
HE~0102-1213                    &    3.03 &      2 &     0.02 &     0.15 &    0.09 \\ 
HE~0146-1548                    &    2.81 &      1 &   \ldots &   \ldots &    0.05 \\ 
HE~0207-1423                    &    3.48 &      1 &   \ldots &   \ldots &    0.21 \\ 
HE~0228-4047\tablenotemark{c}   &    2.96 &      1 &   \ldots &   \ldots &    0.49 \\ 
HE~0228-4047\tablenotemark{d}   &    2.96 &      1 &   \ldots &   \ldots &    0.49 \\ 
HE~0231-6025                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0253-1331                    &    3.34 &      1 &   \ldots &   \ldots &    0.13 \\ 
HE~0314-1739                    &    3.29 &      1 &   \ldots &   \ldots & $-$0.07 \\ 
HE~0355-3728\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0355-3728\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~0945-1435\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1055+0104\tablenotemark{c}   &    3.48 &      2 &     0.05 &     0.15 &    0.13 \\ 
HE~1055+0104\tablenotemark{d}   &    3.45 &      2 &     0.05 &     0.15 &    0.11 \\ 
HE~1116-0054\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1116-0054\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1142-1422                    &    3.50 &      1 &   \ldots &   \ldots &    0.12 \\ 
HE~1201-1512\tablenotemark{c}   &    2.55 &      2 &     0.01 &     0.15 &    0.19 \\ 
HE~1201-1512\tablenotemark{d}   &    2.45 &      2 &     0.00 &     0.14 &    0.15 \\ 
HE~1204-0744                    &    3.33 &      1 &   \ldots &   \ldots & $-$0.18 \\ 
HE~1207-3108                    &    3.20 &      2 &     0.21 &     0.23 & $-$0.33 \\ 
HE~1320-2952                    &    2.38 &      2 &     0.09 &     0.15 & $-$0.15 \\ 
HE~1346-0427\tablenotemark{c}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1346-0427\tablenotemark{d}   &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~1402-0523\tablenotemark{c}   &    3.08 &      1 &   \ldots &   \ldots &    0.03 \\ 
HE~1402-0523\tablenotemark{d}   &    3.07 &      1 &   \ldots &   \ldots &    0.04 \\ 
HE~1506-0113                    &    3.06 &      3 &     0.03 &     0.14 &    0.38 \\ 
HE~2020-5228                    &    3.25 &      1 &   \ldots &   \ldots & $-$0.04 \\ 
HE~2032-5633                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2047-5612                    &    3.37 &      2 &     0.06 &     0.15 &    0.28 \\ 
HE~2135-1924                    &    2.97 &      2 &     0.12 &     0.15 &    0.06 \\ 
HE~2136-6030                    &  \ldots & \ldots &   \ldots &   \ldots &  \ldots \\ 
HE~2139-5432                    &    2.37 &      2 &     0.06 &     0.16 &    0.17 \\ 
HE~2141-0726                    &    3.67 &      2 &     0.24 &     0.25 &    0.17 \\ 
HE~2142-5656                    &    3.06 &      3 &     0.15 &     0.16 & $-$0.29 \\ 
HE~2202-4831                    &    3.37 &      1 &   \ldots &   \ldots & $-$0.07 \\ 
HE~2246-2410                    &    3.36 &      2 &     0.08 &     0.16 &    0.10 \\ 
HE~2247-7400                    &    3.88 &      1 &   \ldots &   \ldots &    0.53 \\ 
\cutinhead{Sr}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    1.05 &      2 &     0.04 &     0.19 &    1.15 \\ 
 53327-2044-515\tablenotemark{c}& $-$0.05 &      2 &     0.02 &     0.16 &    1.09 \\ 
 53327-2044-515\tablenotemark{d}& $-$0.69 &      2 &     0.02 &     0.18 &    0.53 \\ 
 53436-1996-093                 & $-$0.22 &      2 &     0.17 &     0.21 &    0.44 \\ 
 54142-2667-094                 & $-$1.17 &      2 &     0.11 &     0.20 & $-$1.08 \\ 
BS~16545-089                    & $-$0.75 &      2 &     0.00 &     0.17 & $-$0.18 \\ 
CS~30336-049                    & $-$2.86 &      2 &     0.11 &     0.20 & $-$1.63 \\ 
HE~0049-3948                    & $-$1.66 &      1 &   \ldots &   \ldots & $-$0.85 \\ 
HE~0057-5959                    & $-$2.27 &      2 &     0.04 &     0.20 & $-$1.06 \\ 
HE~0102-1213                    & $-$0.71 &      2 &     0.03 &     0.18 & $-$0.30 \\ 
HE~0146-1548                    & $-$0.97 &      2 &     0.04 &     0.26 & $-$0.38 \\ 
HE~0207-1423                    &    0.25 &      1 &   \ldots &   \ldots &    0.33 \\ 
HE~0228-4047\tablenotemark{c}   &$<-$1.46 &      1 &   \ldots &   \ldots &$<-$0.58\tablenotemark{f}  \\ 
HE~0228-4047\tablenotemark{d}   &$<-$1.63 &      1 &   \ldots &   \ldots &$<-$0.75\tablenotemark{f}  \\ 
HE~0231-6025                    & $-$0.19 &      2 &     0.15 &     0.19 &    0.04 \\ 
HE~0253-1331                    &    0.27 &      2 &     0.23 &     0.26 &    0.41 \\ 
HE~0314-1739                    & $-$0.56 &      2 &     0.06 &     0.20 & $-$0.57 \\ 
HE~0355-3728\tablenotemark{c}   & $-$0.10 &      1 &   \ldots &   \ldots &    0.45 \\ 
HE~0355-3728\tablenotemark{d}   &    0.38 &      1 &   \ldots &   \ldots &    0.92 \\ 
HE~0945-1435\tablenotemark{c}   &$<-$1.61 &      1 &   \ldots &   \ldots &$<-$0.71\tablenotemark{f}  \\ 
HE~0945-1435\tablenotemark{d}   &$<-$1.84 &      1 &   \ldots &   \ldots &$<-$0.93\tablenotemark{f}  \\ 
HE~1055+0104\tablenotemark{c}   & $-$0.11 &      2 &     0.08 &     0.17 & $-$0.11 \\ 
HE~1055+0104\tablenotemark{d}   & $-$0.38 &      2 &     0.05 &     0.17 & $-$0.37 \\ 
HE~1116-0054\tablenotemark{c}   & $-$0.69 &      2 &     0.05 &     0.17 & $-$0.07 \\ 
HE~1116-0054\tablenotemark{d}   & $-$0.87 &      2 &     0.05 &     0.17 & $-$0.25 \\ 
HE~1142-1422                    &    0.50 &      2 &     0.06 &     0.21 &    0.48 \\ 
HE~1201-1512\tablenotemark{c}   &$<-$1.86 &      1 &   \ldots &   \ldots &$<-$0.87\tablenotemark{f}  \\ 
HE~1201-1512\tablenotemark{d}   &$<-$2.32 &      1 &   \ldots &   \ldots &$<-$1.27\tablenotemark{f}  \\ 
HE~1204-0744                    & $-$0.14 &      2 &     0.05 &     0.19 & $-$0.30 \\ 
HE~1207-3108                    & $-$0.21 &      2 &     0.11 &     0.26 & $-$0.38 \\ 
HE~1320-2952                    & $-$1.19 &      2 &     0.06 &     0.19 & $-$0.37 \\ 
HE~1346-0427\tablenotemark{c}   & $-$0.93 &      2 &     0.03 &     0.18 & $-$0.23 \\ 
HE~1346-0427\tablenotemark{d}   & $-$1.19 &      2 &     0.04 &     0.18 & $-$0.48 \\ 
HE~1402-0523\tablenotemark{c}   & $-$0.19 &      2 &     0.11 &     0.19 &    0.11 \\ 
HE~1402-0523\tablenotemark{d}   & $-$0.41 &      2 &     0.09 &     0.19 & $-$0.09 \\ 
HE~1506-0113                    & $-$1.51 &      2 &     0.10 &     0.19 & $-$0.85 \\ 
HE~2020-5228                    & $-$0.26 &      1 &   \ldots &   \ldots & $-$0.20 \\ 
HE~2032-5633                    &$<-$1.44 &      1 &   \ldots &   \ldots &$<-$0.68\tablenotemark{f}  \\ 
HE~2047-5612                    &$<-$1.63 &      1 &   \ldots &   \ldots &$<-$1.36\tablenotemark{f}  \\ 
HE~2135-1924                    & $-$1.11 &      2 &     0.01 &     0.19 & $-$0.66 \\ 
HE~2136-6030                    &    0.03 &      2 &     0.13 &     0.18 &    0.04 \\ 
HE~2139-5432                    & $-$1.71 &      2 &     0.01 &     0.20 & $-$0.55 \\ 
HE~2141-0726                    & $-$0.42 &      2 &     0.01 &     0.19 & $-$0.57 \\ 
HE~2142-5656                    & $-$0.19 &      2 &     0.18 &     0.26 & $-$0.19 \\ 
HE~2202-4831                    & $-$0.76 &      1 &   \ldots &   \ldots & $-$0.85 \\ 
HE~2246-2410                    & $-$0.50 &      2 &     0.05 &     0.19 & $-$0.40 \\ 
HE~2247-7400                    &$<-$0.15 &      1 &   \ldots &   \ldots &$<-$0.15\tablenotemark{f}  \\ 
\cutinhead{Ba}                 &         &        &          &          &         \\ 
 52972-1213-507                 &    0.90 &      4 &     0.09 &     0.13 &    1.70 \\ 
 53327-2044-515\tablenotemark{c}&$<-$1.48 &      1 &   \ldots &   \ldots & $<$0.34\tablenotemark{g} \\ 
 53327-2044-515\tablenotemark{d}&$<-$1.95 &      1 &   \ldots &   \ldots &$<-$0.04\tablenotemark{g} \\ 
 53436-1996-093                 & $<-$1.3 &      1 &   \ldots &   \ldots & $<$0.05\tablenotemark{g} \\ 
 54142-2667-094                 &$<-$1.21 &      1 &   \ldots &   \ldots &$<-$0.43\tablenotemark{g} \\ 
BS~16545-089                    &$<-$1.44 &      1 &   \ldots &   \ldots &$<-$0.18\tablenotemark{g} \\ 
CS~30336-049                    &$<-$3.47 &      1 &   \ldots &   \ldots &$<-$1.55\tablenotemark{g} \\ 
HE~0049-3948                    &$<-$1.36 &      1 &   \ldots &   \ldots & $<$0.14\tablenotemark{g} \\ 
HE~0057-5959                    & $-$2.36 &      1 &   \ldots &   \ldots & $-$0.46 \\ 
HE~0102-1213                    &$<-$1.74 &      1 &   \ldots &   \ldots &$<-$0.64\tablenotemark{g} \\ 
HE~0146-1548                    & $-$2.00 &      3 &     0.14 &     0.19 & $-$0.71 \\ 
HE~0207-1423                    &    0.96 &      4 &     0.10 &     0.12 &    1.73 \\ 
HE~0228-4047\tablenotemark{c}   &$<-$1.17 &      1 &   \ldots &   \ldots & $<$0.40\tablenotemark{g} \\ 
HE~0228-4047\tablenotemark{d}   &$<-$1.33 &      1 &   \ldots &   \ldots & $<$0.24\tablenotemark{g} \\ 
HE~0231-6025                    & $-$1.02 &      1 &   \ldots &   \ldots & $-$0.10 \\ 
HE~0253-1331                    & $-$0.50 &      1 &   \ldots &   \ldots &    0.33 \\ 
HE~0314-1739                    &$<-$0.95 &      1 &   \ldots &   \ldots &$<-$0.27\tablenotemark{g} \\ 
HE~0355-3728\tablenotemark{c}   &$<-$1.03 &      1 &   \ldots &   \ldots & $<$0.21\tablenotemark{g} \\ 
HE~0355-3728\tablenotemark{d}   &$<-$1.14 &      1 &   \ldots &   \ldots & $<$0.09\tablenotemark{g} \\ 
HE~0945-1435\tablenotemark{c}   &$<-$1.34 &      1 &   \ldots &   \ldots & $<$0.25\tablenotemark{g} \\ 
HE~0945-1435\tablenotemark{d}   &$<-$1.56 &      1 &   \ldots &   \ldots & $<$0.04\tablenotemark{g} \\ 
HE~1055+0104\tablenotemark{c}   &$<-$1.08 &      1 &   \ldots &   \ldots &$<-$0.39\tablenotemark{g} \\ 
HE~1055+0104\tablenotemark{d}   &$<-$1.28 &      1 &   \ldots &   \ldots &$<-$0.57\tablenotemark{g} \\ 
HE~1116-0054\tablenotemark{c}   &$<-$1.15 &      1 &   \ldots &   \ldots & $<$0.16\tablenotemark{g} \\ 
HE~1116-0054\tablenotemark{d}   &$<-$1.31 &      1 &   \ldots &   \ldots &$<-$0.01\tablenotemark{g} \\ 
HE~1142-1422                    & $-$0.23 &      3 &     0.05 &     0.15 &    0.44 \\ 
HE~1201-1512\tablenotemark{c}   &$<-$1.63 &      1 &   \ldots &   \ldots & $<$0.05\tablenotemark{g} \\ 
HE~1201-1512\tablenotemark{d}   &$<-$2.08 &      1 &   \ldots &   \ldots &$<-$0.34\tablenotemark{g} \\ 
HE~1204-0744                    &$<-$0.71 &      1 &   \ldots &   \ldots &$<-$0.18\tablenotemark{g} \\ 
HE~1207-3108                    &$<-$2.19 &      1 &   \ldots &   \ldots &$<-$1.67\tablenotemark{g} \\ 
HE~1320-2952                    & $-$2.47 &      1 &   \ldots &   \ldots & $-$0.96 \\ 
HE~1346-0427\tablenotemark{c}   &$<-$1.38 &      1 &   \ldots &   \ldots & $<$0.01\tablenotemark{g} \\ 
HE~1346-0427\tablenotemark{d}   &$<-$1.62 &      1 &   \ldots &   \ldots &$<-$0.22\tablenotemark{g} \\ 
HE~1402-0523\tablenotemark{c}   &$<-$1.08 &      1 &   \ldots &   \ldots &$<-$0.09\tablenotemark{g} \\ 
HE~1402-0523\tablenotemark{d}   &$<-$1.25 &      1 &   \ldots &   \ldots &$<-$0.24\tablenotemark{g} \\ 
HE~1506-0113                    & $-$2.16 &      1 &   \ldots &   \ldots & $-$0.80 \\ 
HE~2020-5228                    &$<-$1.08 &      1 &   \ldots &   \ldots &$<-$0.33\tablenotemark{g} \\ 
HE~2032-5633                    &$<-$1.14 &      1 &   \ldots &   \ldots & $<$0.31\tablenotemark{g} \\ 
HE~2047-5612                    &$<-$1.35 &      1 &   \ldots &   \ldots &$<-$0.39\tablenotemark{g} \\ 
HE~2135-1924                    &$<-$1.13 &      1 &   \ldots &   \ldots & $<$0.00\tablenotemark{g} \\ 
HE~2136-6030                    & $-$0.68 &      1 &   \ldots &   \ldots &    0.02 \\ 
HE~2139-5432                    &$<-$2.17 &      1 &   \ldots &   \ldots &$<-$0.33\tablenotemark{g} \\ 
HE~2141-0726                    &$<-$0.91 &      1 &   \ldots &   \ldots &$<-$0.37\tablenotemark{g} \\ 
HE~2142-5656                    & $-$1.31 &      4 &     0.07 &     0.16 & $-$0.63 \\ 
HE~2202-4831                    & $-$1.88 &      2 &     0.02 &     0.21 & $-$1.28 \\ 
HE~2246-2410                    &$<-$1.08 &      1 &   \ldots &   \ldots &$<-$0.30\tablenotemark{g} \\ 
HE~2247-7400                    & $-$1.62 &      4 &     0.11 &     0.17 & $-$0.94 \\ 
\enddata

\tablenotetext{a}{Standard error of the mean.} 
\tablenotetext{b}{Total error is the quadratic sum of the updated random error and the systematic error (see Section 2.3 for details).} 
\tablenotetext{c}{Dwarf gravity is assumed (see Section 2.1 for details).}
\tablenotetext{d}{Subgiant gravity is assumed (see Section 2.1 for details).}

\tablenotetext{e}{Abundances, or limits, were determined from 
spectrum synthesis of the 4102.94\AA\ Si line.}
\tablenotetext{f}{Abundances limits were determined from 
the 4077.71\AA\ Sr line.}
\tablenotetext{g}{Abundances limits were determined from 
the 4554.03\AA\ Ba line.}


\end{deluxetable}



==> tab4.tex <==
\begin{deluxetable}{lrrrrc}
\tabletypesize{\scriptsize}
%\rotate{90}
\tablecolumns{6} 
\tablewidth{0pc} 
\tablecaption{Abundance Errors from Uncertainties in Atmospheric Parameters 
\newline 
for the 38 Program Stars \label{tab:parvar}}
\tablehead{ 
\colhead{Species} & 
\colhead{$\Delta$\teff} &
\colhead{$\Delta\log g$} &
\colhead{$\Delta\xi_t$} &
\colhead{$\Delta${\rm [M/H]}} &
\colhead{$\Delta${\rm [X/Fe]}} \\
\colhead{} &
\colhead{(100 K)} &
\colhead{(0.3 dex)} &
\colhead{(0.3 \kms)} &
\colhead{(0.3 dex)} &
\colhead{(dex)}  \\
\cline{2-6} 
\colhead{(1)} &
\colhead{(2)} &
\colhead{(3)} &
\colhead{(4)} &
\colhead{(5)} &
\colhead{(6)} 
}
\startdata 
 \noalign{\vskip +0.5ex}
 \multicolumn{6}{c}{52972-1213-507} \cr
 \noalign{\vskip  .8ex}% 
 \hline
 \noalign{\vskip-2ex}\\
     $\Delta$[Na/Fe] &    0.00 & $-$0.08 &    0.00 &    0.04 &    0.09 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.05 &    0.00 &    0.04 &    0.06 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] &    0.01 & $-$0.07 &    0.00 & $-$0.03 &    0.08 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.12 & $-$0.01 &    0.03 &    0.14 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.04 &    0.01 &    0.10 &    0.11 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.10 & $-$0.04 &    0.01 & $-$0.11 &    0.15 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &    0.00 &    0.04 &    0.00 &    0.09 &    0.10 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.05 &    0.01 &    0.08 &    0.10 \\
     $\Delta$[Sr/Fe] & $-$0.02 &    0.05 & $-$0.01 & $-$0.12 &    0.13 \\
     $\Delta$[Ba/Fe] & $-$0.02 &    0.06 & $-$0.01 & $-$0.05 &    0.08 \\
\cutinhead{53327-2044-515\tablenotemark{a}}
     $\Delta$[Na/Fe] & $-$0.03 &    0.03 &    0.01 &    0.05 &    0.07 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.02 &    0.01 &    0.03 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.02 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Si/Fe] & $-$0.01 &    0.02 &    0.01 &    0.02 &    0.03 \\
     $\Delta$[Ca/Fe] &    0.00 & $-$0.04 &    0.00 & $-$0.02 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.12 &    0.01 &    0.05 &    0.14 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.10 &    0.00 &    0.02 &    0.11 \\
     $\Delta$[Cr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.10 &    0.00 & $-$0.01 & $-$0.05 &    0.11 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] & $-$0.01 &    0.04 &    0.00 &    0.03 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.02 &    0.05 &    0.00 & $-$0.06 &    0.08 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{53327-2044-515\tablenotemark{b}}
     $\Delta$[Na/Fe] & $-$0.04 & $-$0.01 &    0.00 &    0.05 &    0.06 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.02 &    0.00 &    0.00 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.00 &    0.01 &    0.04 &    0.05 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.01 &    0.01 &    0.01 &    0.03 \\
     $\Delta$[Ca/Fe] & $-$0.02 & $-$0.02 & $-$0.01 & $-$0.05 &    0.06 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.10 &    0.00 &    0.06 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 &    0.00 &    0.03 &    0.12 \\
     $\Delta$[Cr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 &    0.00 &    0.00 & $-$0.06 &    0.13 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.00 &    0.01 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.10 &    0.00 & $-$0.04 &    0.11 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{53436-1996-093}
     $\Delta$[Na/Fe] & $-$0.02 &    0.01 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.02 &    0.00 &    0.00 &    0.03 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] &    0.01 & $-$0.02 &    0.01 & $-$0.06 &    0.06 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.12 &    0.00 &    0.04 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.11 & $-$0.01 &    0.03 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.00 &    0.00 &    0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.10 & $-$0.01 &    0.01 & $-$0.04 &    0.11 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.11 &    0.00 & $-$0.02 &    0.12 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{54142-2667-094}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.03 &    0.00 &    0.00 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.02 &    0.00 &    0.08 &    0.08 \\
     $\Delta$[Si/Fe] &    0.01 &    0.02 &    0.00 &    0.04 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.03 &    0.00 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.12 & $-$0.01 &    0.07 &    0.15 \\
   $\Delta$[\tii/Fe] & $-$0.01 &    0.01 &    0.00 &    0.08 &    0.08 \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 & $-$0.01 &    0.04 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.01 &    0.02 &    0.01 &    0.08 &    0.08 \\
     $\Delta$[Mn/Fe] &    0.02 &    0.02 &    0.01 &    0.09 &    0.09 \\
    $\Delta$[\fei/H] &    0.09 & $-$0.02 &    0.01 & $-$0.09 &    0.13 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.00 & $-$0.01 &    0.11 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.02 &    0.02 &    0.00 &    0.08 &    0.08 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.11 & $-$0.01 &    0.08 &    0.14 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{BS~16545-089}
     $\Delta$[Na/Fe] & $-$0.02 &    0.00 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Mg/Fe] & $-$0.02 &    0.00 &    0.00 &    0.00 &    0.02 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.01 &    0.00 & $-$0.02 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.10 & $-$0.01 &    0.01 &    0.11 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.10 &    0.00 &    0.02 &    0.11 \\
     $\Delta$[Cr/Fe] &    0.02 &    0.00 &    0.01 &    0.02 &    0.03 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.10 &    0.00 &    0.01 & $-$0.02 &    0.10 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.02 &    0.10 &    0.00 &    0.00 &    0.10 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{CS~30336-049}
     $\Delta$[Na/Fe] & $-$0.03 &    0.01 &    0.01 &    0.07 &    0.08 \\
     $\Delta$[Mg/Fe] & $-$0.04 & $-$0.01 &    0.00 &    0.00 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.02 &    0.01 &    0.08 &    0.08 \\
     $\Delta$[Si/Fe] & $-$0.02 & $-$0.01 &    0.01 & $-$0.08 &    0.08 \\
     $\Delta$[Ca/Fe] & $-$0.03 &    0.01 &    0.01 &    0.06 &    0.07 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.12 &    0.01 &    0.07 &    0.14 \\
   $\Delta$[\tii/Fe] &    0.01 &    0.02 &    0.01 &    0.10 &    0.10 \\
  $\Delta$[\tiii/Fe] & $-$0.07 &    0.11 &    0.00 &    0.05 &    0.14 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.08 &    0.08 \\
     $\Delta$[Mn/Fe] &    0.03 &    0.02 &    0.01 &    0.09 &    0.10 \\
    $\Delta$[\fei/H] &    0.12 & $-$0.04 & $-$0.01 & $-$0.11 &    0.17 \\
   $\Delta$[\feii/H] &    0.03 &    0.09 &    0.00 &    0.00 &    0.09 \\
     $\Delta$[Co/Fe] &    0.02 &    0.02 &    0.00 &    0.09 &    0.09 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.01 &    0.00 &    0.03 &    0.03 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.12 &    0.01 &    0.10 &    0.16 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0049-3948}
     $\Delta$[Na/Fe] & $-$0.03 & $-$0.01 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.05 & $-$0.17 & $-$0.06 &    0.19 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.00 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Ca/Fe] & $-$0.01 & $-$0.01 &    0.00 & $-$0.02 &    0.02 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.10 &    0.00 &    0.01 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.00 &    0.00 &    0.03 &    0.03 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.10 &    0.00 &    0.00 & $-$0.04 &    0.11 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.01 &    0.00 &    0.00 &    0.03 &    0.03 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.09 &    0.00 &    0.03 &    0.10 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0057-5959}
     $\Delta$[Na/Fe] &    0.02 & $-$0.08 &    0.00 & $-$0.04 &    0.09 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.04 &    0.00 & $-$0.01 &    0.05 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.02 &    0.01 &    0.05 &    0.06 \\
     $\Delta$[Si/Fe] & $-$0.01 &    0.01 &    0.00 & $-$0.03 &    0.03 \\
     $\Delta$[Ca/Fe] & $-$0.04 &    0.00 &    0.00 &    0.05 &    0.06 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.11 &    0.00 &    0.08 &    0.14 \\
   $\Delta$[\tii/Fe] &    0.00 &    0.02 &    0.00 &    0.09 &    0.09 \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.10 &    0.00 &    0.04 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.00 & $-$0.01 &    0.08 &    0.08 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.02 &    0.00 & $-$0.09 &    0.14 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.00 &    0.02 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.11 &    0.00 &    0.08 &    0.14 \\
     $\Delta$[Ba/Fe] & $-$0.03 &    0.11 &    0.00 &    0.08 &    0.14 \\
\cutinhead{HE~0102-1213}
     $\Delta$[Na/Fe] & $-$0.02 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.02 & $-$0.01 &    0.01 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Si/Fe] & $-$0.01 &    0.01 &    0.00 &    0.00 &    0.01 \\
     $\Delta$[Ca/Fe] & $-$0.03 &    0.01 & $-$0.01 &    0.04 &    0.05 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.11 &    0.00 &    0.07 &    0.14 \\
   $\Delta$[\tii/Fe] &    0.00 &    0.01 &    0.01 &    0.07 &    0.07 \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 &    0.00 &    0.03 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.01 & $-$0.01 &    0.06 &    0.06 \\
    $\Delta$[\fei/H] &    0.09 & $-$0.01 &    0.01 & $-$0.07 &    0.11 \\
   $\Delta$[\feii/H] &    0.02 &    0.12 &    0.01 &    0.00 &    0.12 \\
     $\Delta$[Co/Fe] &    0.01 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.01 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.11 & $-$0.01 &    0.02 &    0.12 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0146-1548}
     $\Delta$[Na/Fe] & $-$0.03 & $-$0.05 & $-$0.03 & $-$0.11 &    0.13 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.03 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.04 & $-$0.04 & $-$0.02 & $-$0.13 &    0.14 \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.02 &    0.00 & $-$0.04 &    0.05 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &    0.01 &    0.00 &    0.00 &    0.07 &    0.07 \\
  $\Delta$[\tiii/Fe] & $-$0.09 &    0.12 &    0.03 &    0.01 &    0.15 \\
     $\Delta$[Cr/Fe] & $-$0.01 & $-$0.01 &    0.00 &    0.01 &    0.02 \\
     $\Delta$[Mn/Fe] &    0.02 &    0.00 &    0.00 & $-$0.07 &    0.07 \\
    $\Delta$[\fei/H] &    0.12 & $-$0.05 & $-$0.02 & $-$0.09 &    0.16 \\
   $\Delta$[\feii/H] &    0.01 &    0.09 &    0.01 & $-$0.02 &    0.09 \\
     $\Delta$[Co/Fe] &    0.01 &    0.00 &    0.00 & $-$0.01 &    0.01 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.02 &    0.02 &    0.07 &    0.08 \\
     $\Delta$[Sr/Fe] & $-$0.08 &    0.10 & $-$0.01 & $-$0.18 &    0.22 \\
     $\Delta$[Ba/Fe] & $-$0.04 &    0.12 &    0.03 &    0.02 &    0.13 \\
\cutinhead{HE~0207-1423}
     $\Delta$[Na/Fe] &    0.03 & $-$0.05 &    0.00 & $-$0.04 &    0.07 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.08 &    0.00 &    0.03 &    0.09 \\
     $\Delta$[Al/Fe] &    0.01 & $-$0.07 &    0.00 & $-$0.06 &    0.09 \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.05 &    0.01 &    0.00 &    0.07 &    0.09 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] & $-$0.02 &    0.01 &    0.00 &    0.08 &    0.08 \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.11 &    0.00 & $-$0.02 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.01 & $-$0.01 &    0.00 & $-$0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.03 &    0.00 & $-$0.11 &    0.16 \\
   $\Delta$[\feii/H] &    0.01 &    0.10 &    0.00 & $-$0.04 &    0.11 \\
     $\Delta$[Co/Fe] &    0.02 &    0.02 &    0.01 &    0.02 &    0.04 \\
     $\Delta$[Ni/Fe] &    0.00 &    0.02 &    0.00 &    0.04 &    0.04 \\
     $\Delta$[Sr/Fe] & $-$0.01 &    0.03 &    0.00 & $-$0.10 &    0.10 \\
     $\Delta$[Ba/Fe] &    0.01 &    0.02 & $-$0.01 & $-$0.07 &    0.07 \\
\cutinhead{HE~0228-4047\tablenotemark{a}}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.01 &    0.00 &    0.00 &    0.03 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.01 &    0.00 &    0.01 &    0.02 \\
     $\Delta$[Ca/Fe] & $-$0.01 & $-$0.01 & $-$0.01 & $-$0.04 &    0.04 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.10 & $-$0.01 &    0.01 &    0.11 \\
     $\Delta$[Cr/Fe] & $-$0.01 &    0.00 &    0.00 &    0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.09 &    0.00 &    0.01 & $-$0.03 &    0.10 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] & $-$0.01 &    0.00 & $-$0.01 &    0.02 &    0.02 \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0228-4047\tablenotemark{b}}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] & $-$0.02 &    0.00 &    0.01 &    0.00 &    0.02 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.00 &    0.00 &    0.01 &    0.02 \\
     $\Delta$[Ca/Fe] & $-$0.01 & $-$0.01 & $-$0.01 & $-$0.04 &    0.04 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.10 &    0.00 &    0.01 &    0.11 \\
     $\Delta$[Cr/Fe] & $-$0.01 & $-$0.01 & $-$0.01 &    0.02 &    0.03 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.09 &    0.00 &    0.01 & $-$0.03 &    0.10 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.00 &    0.00 & $-$0.01 &    0.02 &    0.02 \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0231-6025}
     $\Delta$[Na/Fe] & $-$0.04 &    0.01 &    0.00 &    0.05 &    0.06 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.04 &    0.00 &    0.01 &    0.05 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.02 &    0.00 &    0.06 &    0.07 \\
     $\Delta$[Si/Fe] & $-$0.03 &    0.01 & $-$0.01 &    0.02 &    0.04 \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.02 & $-$0.01 & $-$0.01 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.11 & $-$0.02 &    0.05 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.07 &    0.12 & $-$0.01 &    0.05 &    0.15 \\
     $\Delta$[Cr/Fe] & $-$0.01 &    0.01 & $-$0.01 &    0.05 &    0.05 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.01 &    0.02 & $-$0.06 &    0.13 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.05 &    0.10 & $-$0.01 &    0.01 &    0.11 \\
     $\Delta$[Ba/Fe] & $-$0.04 &    0.10 & $-$0.01 &    0.05 &    0.12 \\
\cutinhead{HE~0253-1331}
     $\Delta$[Na/Fe] & $-$0.03 &    0.01 & $-$0.01 &    0.05 &    0.06 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.04 & $-$0.01 &    0.01 &    0.05 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.01 & $-$0.01 &    0.05 &    0.06 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.01 & $-$0.01 &    0.02 &    0.03 \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.03 & $-$0.01 &    0.01 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.11 & $-$0.02 &    0.04 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.10 & $-$0.01 &    0.01 &    0.11 \\
     $\Delta$[Cr/Fe] &    0.01 &    0.02 &    0.01 &    0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.10 & $-$0.01 &    0.02 & $-$0.07 &    0.12 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] & $-$0.01 &    0.01 & $-$0.01 &    0.06 &    0.06 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.02 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.09 & $-$0.01 & $-$0.07 &    0.12 \\
     $\Delta$[Ba/Fe] & $-$0.03 &    0.10 & $-$0.02 &    0.04 &    0.11 \\
\cutinhead{HE~0314-1739}
     $\Delta$[Na/Fe] & $-$0.02 &    0.01 &    0.00 &    0.08 &    0.08 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.02 &    0.00 &    0.02 &    0.03 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.03 &    0.01 &    0.08 &    0.09 \\
     $\Delta$[Si/Fe] & $-$0.01 &    0.02 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Ca/Fe] &    0.01 & $-$0.06 &    0.01 & $-$0.05 &    0.08 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.12 &    0.00 &    0.08 &    0.15 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 &    0.00 &    0.03 &    0.12 \\
     $\Delta$[Cr/Fe] & $-$0.01 &    0.02 &    0.00 &    0.07 &    0.07 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.08 & $-$0.02 &    0.00 & $-$0.09 &    0.12 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.01 &    0.02 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.12 &    0.00 &    0.06 &    0.14 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0355-3728\tablenotemark{a}}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.03 &    0.00 &    0.06 &    0.07 \\
     $\Delta$[Ca/Fe] & $-$0.02 & $-$0.02 &    0.00 & $-$0.03 &    0.04 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.12 &    0.00 &    0.02 &    0.14 \\
     $\Delta$[Cr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.12 & $-$0.02 &    0.01 & $-$0.08 &    0.15 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.05 &    0.11 &    0.00 & $-$0.02 &    0.12 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0355-3728\tablenotemark{b}}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] & $-$0.05 &    0.08 &    0.00 &    0.11 &    0.14 \\
     $\Delta$[Ca/Fe] & $-$0.02 & $-$0.03 &    0.00 & $-$0.01 &    0.04 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.13 & $-$0.01 &    0.03 &    0.15 \\
     $\Delta$[Cr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.04 &    0.01 & $-$0.10 &    0.15 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.09 & $-$0.01 & $-$0.12 &    0.16 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0945-1435\tablenotemark{a}}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.01 &    0.00 &    0.01 &    0.03 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.00 &    0.00 &    0.00 &    0.02 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.12 &    0.01 &    0.03 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 &    0.00 &    0.02 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.00 &    0.00 &    0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.08 & $-$0.01 & $-$0.01 & $-$0.03 &    0.09 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~0945-1435\tablenotemark{b}}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] & $-$0.03 &    0.00 &    0.01 &    0.01 &    0.03 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.00 &    0.00 & $-$0.01 &    0.02 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.10 &    0.00 &    0.02 &    0.11 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.10 &    0.00 &    0.02 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 & $-$0.01 & $-$0.01 &    0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.09 &    0.00 &    0.00 & $-$0.02 &    0.09 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1055+0104\tablenotemark{a}}
     $\Delta$[Na/Fe] & $-$0.02 &    0.02 &    0.00 &    0.04 &    0.05 \\
     $\Delta$[Mg/Fe] &    0.00 & $-$0.08 &    0.00 &    0.01 &    0.08 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.03 & $-$0.01 &    0.04 &    0.05 \\
     $\Delta$[Si/Fe] &    0.00 & $-$0.04 &    0.01 & $-$0.02 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.00 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.14 &    0.00 &    0.06 &    0.16 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.04 &    0.13 &    0.00 &    0.03 &    0.14 \\
     $\Delta$[Cr/Fe] & $-$0.01 &    0.02 &    0.00 &    0.04 &    0.05 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.04 &    0.00 &    0.06 &    0.07 \\
    $\Delta$[\fei/H] &    0.09 & $-$0.03 &    0.01 & $-$0.07 &    0.12 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.01 & $-$0.01 &    0.11 \\
     $\Delta$[Co/Fe] &    0.00 &    0.04 &    0.00 &    0.06 &    0.07 \\
     $\Delta$[Ni/Fe] &    0.00 &    0.04 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.11 & $-$0.02 & $-$0.03 &    0.12 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1055+0104\tablenotemark{b}}
     $\Delta$[Na/Fe] & $-$0.01 &    0.01 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.06 &    0.00 & $-$0.03 &    0.07 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.01 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Si/Fe] & $-$0.01 & $-$0.02 &    0.00 & $-$0.06 &    0.06 \\
     $\Delta$[Ca/Fe] & $-$0.02 & $-$0.01 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.11 & $-$0.01 &    0.06 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.04 &    0.11 &    0.00 &    0.03 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.01 &    0.00 &    0.06 &    0.06 \\
    $\Delta$[\fei/H] &    0.09 & $-$0.01 &    0.01 & $-$0.07 &    0.11 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.00 & $-$0.01 &    0.11 \\
     $\Delta$[Co/Fe] &    0.00 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.01 &    0.00 &    0.03 &    0.03 \\
     $\Delta$[Sr/Fe] & $-$0.02 &    0.11 &    0.00 &    0.00 &    0.11 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1116-0054\tablenotemark{a}}
     $\Delta$[Na/Fe] & $-$0.03 &    0.01 &    0.00 &    0.04 &    0.05 \\
     $\Delta$[Mg/Fe] & $-$0.04 & $-$0.02 & $-$0.01 &    0.00 &    0.05 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.03 &    0.00 & $-$0.01 & $-$0.01 &    0.03 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.11 &    0.00 &    0.03 &    0.12 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.07 &    0.10 & $-$0.01 &    0.03 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.04 &    0.04 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.01 &    0.01 & $-$0.04 &    0.12 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.05 &    0.10 & $-$0.01 &    0.01 &    0.11 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1116-0054\tablenotemark{b}}
     $\Delta$[Na/Fe] & $-$0.03 &    0.00 & $-$0.01 &    0.03 &    0.04 \\
     $\Delta$[Mg/Fe] & $-$0.04 & $-$0.01 & $-$0.01 &    0.00 &    0.04 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.03 &    0.00 & $-$0.01 & $-$0.01 &    0.03 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.09 & $-$0.01 &    0.03 &    0.11 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.11 &    0.00 &    0.04 &    0.13 \\
     $\Delta$[Cr/Fe] & $-$0.01 &    0.00 &    0.00 &    0.04 &    0.04 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 &    0.00 &    0.01 & $-$0.04 &    0.12 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.10 & $-$0.01 &    0.02 &    0.11 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1142-1422}
     $\Delta$[Na/Fe] & $-$0.01 &    0.00 &    0.00 &    0.04 &    0.04 \\
     $\Delta$[Mg/Fe] & $-$0.02 &    0.00 &    0.00 & $-$0.04 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.00 &    0.00 &    0.03 &    0.03 \\
     $\Delta$[Si/Fe] &    0.00 &    0.01 &    0.00 &    0.02 &    0.02 \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.00 & $-$0.01 & $-$0.04 &    0.05 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.11 &    0.00 &    0.04 &    0.12 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.10 & $-$0.01 &    0.02 &    0.11 \\
     $\Delta$[Cr/Fe] &    0.00 & $-$0.01 &    0.00 &    0.04 &    0.04 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.00 &    0.00 &    0.05 &    0.05 \\
    $\Delta$[\fei/H] &    0.08 & $-$0.01 &    0.01 & $-$0.06 &    0.10 \\
   $\Delta$[\feii/H] &    0.02 &    0.10 &    0.01 & $-$0.01 &    0.10 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.02 &    0.01 &    0.01 &    0.04 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.02 &    0.10 & $-$0.01 & $-$0.11 &    0.15 \\
     $\Delta$[Ba/Fe] & $-$0.02 &    0.08 & $-$0.01 &    0.02 &    0.09 \\
\cutinhead{HE~1201-1512\tablenotemark{a}}
     $\Delta$[Na/Fe] & $-$0.02 &    0.02 &    0.01 &    0.04 &    0.05 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.01 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.02 &    0.01 &    0.03 &    0.04 \\
     $\Delta$[Si/Fe] & $-$0.01 &    0.00 &    0.01 &    0.00 &    0.01 \\
     $\Delta$[Ca/Fe] & $-$0.02 & $-$0.01 &    0.00 &    0.00 &    0.02 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.11 &    0.01 &    0.04 &    0.12 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.10 &    0.00 &    0.02 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.03 &    0.01 &    0.04 &    0.05 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.03 &    0.00 &    0.03 &    0.04 \\
    $\Delta$[\fei/H] &    0.09 &    0.01 & $-$0.01 & $-$0.04 &    0.10 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &    0.00 &    0.03 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Ni/Fe] &    0.00 &    0.03 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1201-1512\tablenotemark{b}}
     $\Delta$[Na/Fe] & $-$0.02 &    0.01 &    0.01 &    0.06 &    0.06 \\
     $\Delta$[Mg/Fe] & $-$0.03 &    0.00 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.02 &    0.01 &    0.05 &    0.06 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.01 &    0.00 & $-$0.01 &    0.02 \\
     $\Delta$[Ca/Fe] & $-$0.03 &    0.00 &    0.00 &    0.00 &    0.03 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.11 &    0.01 &    0.06 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 &    0.00 &    0.04 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.01 &    0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.00 &    0.00 &    0.05 &    0.05 \\
    $\Delta$[\fei/H] &    0.10 & $-$0.01 & $-$0.01 & $-$0.06 &    0.12 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &    0.00 &    0.01 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Ni/Fe] &    0.00 &    0.00 & $-$0.01 &    0.03 &    0.03 \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1204-0744}
     $\Delta$[Na/Fe] & $-$0.02 &    0.01 &    0.00 &    0.04 &    0.05 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.03 &    0.00 &    0.00 &    0.03 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.03 & $-$0.01 &    0.04 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.01 & $-$0.03 &    0.00 &    0.01 &    0.03 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.12 & $-$0.02 &    0.06 &    0.14 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.12 & $-$0.01 &    0.04 &    0.14 \\
     $\Delta$[Cr/Fe] & $-$0.01 &    0.02 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.09 & $-$0.02 &    0.02 & $-$0.08 &    0.12 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.01 & $-$0.02 &    0.11 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.00 &    0.02 & $-$0.01 &    0.06 &    0.06 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.11 & $-$0.01 &    0.02 &    0.12 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1207-3108}
     $\Delta$[Na/Fe] &    0.01 & $-$0.05 &    0.00 &    0.00 &    0.05 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.06 &    0.00 &    0.01 &    0.06 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.04 &    0.00 &    0.01 &    0.05 \\
     $\Delta$[Si/Fe] &    0.01 & $-$0.05 &    0.01 & $-$0.02 &    0.06 \\
     $\Delta$[Ca/Fe] & $-$0.05 &    0.03 & $-$0.01 &    0.05 &    0.08 \\
     $\Delta$[Sc/Fe] & $-$0.06 &    0.15 &    0.01 &    0.03 &    0.16 \\
   $\Delta$[\tii/Fe] & $-$0.01 &    0.05 &    0.00 &    0.08 &    0.09 \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.15 &    0.00 &    0.02 &    0.16 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.03 & $-$0.01 & $-$0.04 &    0.05 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.01 &    0.00 & $-$0.11 &    0.11 \\
    $\Delta$[\fei/H] &    0.12 & $-$0.05 &    0.01 & $-$0.08 &    0.15 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.01 & $-$0.04 &    0.12 \\
     $\Delta$[Co/Fe] & $-$0.01 &    0.05 &    0.00 &    0.05 &    0.07 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.03 &    0.00 & $-$0.11 &    0.11 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.10 & $-$0.01 & $-$0.19 &    0.22 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1320-2952}
     $\Delta$[Na/Fe] & $-$0.02 &    0.02 &    0.00 &    0.07 &    0.08 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.06 &    0.00 &    0.00 &    0.06 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.03 &    0.01 &    0.07 &    0.08 \\
     $\Delta$[Si/Fe] &    0.00 & $-$0.02 &    0.01 & $-$0.04 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.04 &    0.00 & $-$0.01 &    0.06 &    0.07 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.12 &    0.00 &    0.09 &    0.16 \\
   $\Delta$[\tii/Fe] & $-$0.01 &    0.02 &    0.00 &    0.12 &    0.12 \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.12 &    0.01 &    0.07 &    0.15 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.02 &    0.00 &    0.08 &    0.08 \\
     $\Delta$[Mn/Fe] &    0.02 &    0.02 &    0.00 &    0.10 &    0.10 \\
    $\Delta$[\fei/H] &    0.12 & $-$0.03 &    0.00 & $-$0.13 &    0.18 \\
   $\Delta$[\feii/H] &    0.03 &    0.11 &    0.01 & $-$0.01 &    0.11 \\
     $\Delta$[Co/Fe] &    0.01 &    0.03 &    0.00 &    0.10 &    0.10 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.02 &    0.00 &    0.04 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.05 &    0.12 &    0.00 & $-$0.04 &    0.14 \\
     $\Delta$[Ba/Fe] & $-$0.03 &    0.12 &    0.01 &    0.12 &    0.17 \\
\cutinhead{HE~1346-0427\tablenotemark{a}}
     $\Delta$[Na/Fe] & $-$0.02 &    0.00 &    0.00 &    0.02 &    0.03 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.03 &    0.00 & $-$0.01 &    0.04 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.01 & $-$0.01 &    0.00 &    0.03 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.11 & $-$0.01 &    0.02 &    0.12 \\
   $\Delta$[\tii/Fe] & $-$0.01 &    0.00 & $-$0.01 &    0.02 &    0.02 \\
  $\Delta$[\tiii/Fe] & $-$0.04 &    0.12 &    0.00 &    0.02 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.00 &    0.00 &    0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.08 &    0.00 &    0.01 & $-$0.02 &    0.08 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.11 &    0.00 &    0.01 &    0.11 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1346-0427\tablenotemark{b}}
     $\Delta$[Na/Fe] & $-$0.02 & $-$0.01 &    0.00 &    0.02 &    0.03 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.01 &    0.00 & $-$0.01 &    0.02 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.00 &    0.00 &    0.00 &    0.02 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.10 & $-$0.01 &    0.02 &    0.11 \\
   $\Delta$[\tii/Fe] &    0.00 &    0.01 &    0.00 &    0.03 &    0.03 \\
  $\Delta$[\tiii/Fe] & $-$0.04 &    0.10 & $-$0.01 &    0.02 &    0.11 \\
     $\Delta$[Cr/Fe] &    0.00 & $-$0.01 & $-$0.01 &    0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.08 &    0.00 &    0.01 & $-$0.03 &    0.09 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.09 &    0.00 &    0.01 &    0.10 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1402-0523\tablenotemark{a}}
     $\Delta$[Na/Fe] & $-$0.03 &    0.03 &    0.00 &    0.07 &    0.08 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.05 & $-$0.01 &    0.02 &    0.06 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.03 &    0.00 &    0.07 &    0.08 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.03 &    0.00 &    0.04 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.02 &    0.00 &    0.00 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.14 &    0.00 &    0.07 &    0.16 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.07 &    0.12 & $-$0.01 &    0.04 &    0.14 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.03 &    0.00 &    0.07 &    0.08 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.03 &    0.01 & $-$0.08 &    0.14 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &    0.00 &    0.04 &    0.01 &    0.08 &    0.09 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.04 &    0.01 &    0.06 &    0.07 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.12 &    0.00 & $-$0.01 &    0.13 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1402-0523\tablenotemark{b}}
     $\Delta$[Na/Fe] & $-$0.03 &    0.01 &    0.00 &    0.07 &    0.08 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.03 &    0.00 &    0.00 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.00 &    0.00 &    0.07 &    0.07 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.02 &    0.01 &    0.04 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.01 &    0.00 & $-$0.01 &    0.03 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.11 &    0.00 &    0.07 &    0.14 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.11 &    0.00 &    0.05 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.00 &    0.00 &    0.07 &    0.07 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.01 &    0.01 & $-$0.08 &    0.14 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &    0.00 &    0.01 &    0.00 &    0.07 &    0.07 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.10 & $-$0.01 &    0.00 &    0.11 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~1506-0113}
     $\Delta$[Na/Fe] &    0.02 & $-$0.09 & $-$0.02 & $-$0.06 &    0.11 \\
     $\Delta$[Mg/Fe] &    0.00 & $-$0.08 &    0.00 & $-$0.01 &    0.08 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.00 & $-$0.01 & $-$0.04 &    0.05 \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.03 &    0.00 &    0.00 &    0.05 &    0.06 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &    0.00 &    0.02 &    0.01 &    0.08 &    0.08 \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.12 &    0.00 & $-$0.01 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.01 &    0.04 &    0.04 \\
     $\Delta$[Mn/Fe] &    0.02 &    0.00 & $-$0.01 & $-$0.05 &    0.05 \\
    $\Delta$[\fei/H] &    0.12 & $-$0.02 &    0.01 & $-$0.08 &    0.15 \\
   $\Delta$[\feii/H] &    0.01 &    0.10 &    0.01 &    0.00 &    0.10 \\
     $\Delta$[Co/Fe] &    0.01 &    0.01 &    0.00 &    0.04 &    0.04 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.00 &    0.00 & $-$0.07 &    0.07 \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.12 &    0.01 & $-$0.03 &    0.13 \\
     $\Delta$[Ba/Fe] & $-$0.04 &    0.11 &    0.00 &    0.07 &    0.14 \\
\cutinhead{HE~2020-5228}
     $\Delta$[Na/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.05 & $-$0.01 &    0.02 &    0.06 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.01 &    0.00 &    0.02 &    0.03 \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.12 &    0.00 &    0.08 &    0.15 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.11 & $-$0.01 &    0.05 &    0.14 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.02 &    0.00 &    0.09 &    0.09 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.09 & $-$0.02 &    0.01 & $-$0.11 &    0.14 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.01 & $-$0.01 &    0.11 \\
     $\Delta$[Co/Fe] &    0.00 &    0.02 &    0.00 &    0.09 &    0.09 \\
     $\Delta$[Ni/Fe] &    0.00 &    0.02 &    0.00 &    0.08 &    0.08 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.12 &    0.00 &    0.04 &    0.13 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~2032-5633}
     $\Delta$[Na/Fe] & $-$0.03 &    0.01 & $-$0.00 &    0.04 &    0.05 \\
     $\Delta$[Mg/Fe] & $-$0.03 &    0.00 &    0.00 &    0.00 &    0.03 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.01 &    0.01 &    0.05 &    0.06 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.02 &    0.01 &    0.03 &    0.04 \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.00 &    0.00 & $-$0.08 &    0.08 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.07 &    0.10 & $-$0.01 &    0.01 &    0.12 \\
     $\Delta$[Cr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.01 &    0.00 & $-$0.05 &    0.12 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~2047-5612}
     $\Delta$[Na/Fe] & $-$0.03 &    0.02 &    0.00 &    0.08 &    0.09 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.02 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.03 &    0.00 &    0.08 &    0.09 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.02 &    0.01 &    0.02 &    0.04 \\
     $\Delta$[Ca/Fe] & $-$0.02 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.11 & $-$0.01 &    0.06 &    0.14 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 & $-$0.01 &    0.05 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.02 &    0.00 &    0.08 &    0.08 \\
    $\Delta$[\fei/H] &    0.10 & $-$0.02 &    0.01 & $-$0.09 &    0.14 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.01 & $-$0.01 &    0.11 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.01 &    0.02 &    0.00 &    0.03 &    0.04 \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~2135-1924}
     $\Delta$[Na/Fe] & $-$0.03 &    0.01 &    0.00 &    0.05 &    0.06 \\
     $\Delta$[Mg/Fe] & $-$0.04 & $-$0.01 & $-$0.01 &    0.02 &    0.05 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.02 &    0.00 &    0.05 &    0.06 \\
     $\Delta$[Si/Fe] & $-$0.02 &    0.02 &    0.01 &    0.04 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.04 & $-$0.01 & $-$0.01 &    0.00 &    0.04 \\
     $\Delta$[Sc/Fe] & $-$0.05 &    0.11 &    0.00 &    0.06 &    0.13 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.11 & $-$0.01 &    0.02 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.01 &    0.00 &    0.06 &    0.06 \\
    $\Delta$[\fei/H] &    0.11 & $-$0.01 &    0.01 & $-$0.06 &    0.13 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] & $-$0.01 &    0.01 &    0.00 &    0.05 &    0.05 \\
     $\Delta$[Ni/Fe] &    0.00 &    0.02 &    0.00 &    0.04 &    0.04 \\
     $\Delta$[Sr/Fe] & $-$0.05 &    0.11 & $-$0.01 &    0.04 &    0.13 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~2136-6030}
     $\Delta$[Na/Fe] & $-$0.03 &    0.01 &    0.00 &    0.08 &    0.09 \\
     $\Delta$[Mg/Fe] & $-$0.03 & $-$0.03 &    0.00 &    0.02 &    0.05 \\
     $\Delta$[Al/Fe] & $-$0.02 &    0.01 &    0.00 &    0.07 &    0.07 \\
     $\Delta$[Si/Fe] &    0.00 & $-$0.08 &    0.00 & $-$0.04 &    0.09 \\
     $\Delta$[Ca/Fe] & $-$0.03 & $-$0.02 & $-$0.01 & $-$0.01 &    0.04 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.12 &    0.00 &    0.08 &    0.16 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.00 &    0.00 &    0.08 &    0.08 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.10 & $-$0.01 &    0.01 & $-$0.10 &    0.14 \\
   $\Delta$[\feii/H] &    0.02 &    0.10 &    0.00 & $-$0.02 &    0.10 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sr/Fe] & $-$0.04 &    0.11 &    0.00 & $-$0.01 &    0.12 \\
     $\Delta$[Ba/Fe] & $-$0.03 &    0.10 &    0.00 &    0.08 &    0.13 \\
\cutinhead{HE~2139-5432}
     $\Delta$[Na/Fe] &    0.00 & $-$0.12 & $-$0.01 &    0.03 &    0.12 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.09 &    0.00 &    0.07 &    0.11 \\
     $\Delta$[Al/Fe] & $-$0.03 & $-$0.02 & $-$0.01 & $-$0.01 &    0.04 \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.07 &    0.12 &    0.00 &    0.06 &    0.15 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.12 & $-$0.02 &    0.00 & $-$0.09 &    0.15 \\
   $\Delta$[\feii/H] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Co/Fe] &    0.00 &    0.01 & $-$0.01 &    0.07 &    0.07 \\
     $\Delta$[Ni/Fe] &    0.01 &    0.03 &    0.00 &    0.06 &    0.07 \\
     $\Delta$[Sr/Fe] & $-$0.05 &    0.12 &    0.01 &    0.06 &    0.14 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~2141-0726}
     $\Delta$[Na/Fe] & $-$0.02 &    0.01 & $-$0.01 &    0.06 &    0.06 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.03 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Al/Fe] & $-$0.01 &    0.02 &    0.01 &    0.07 &    0.07 \\
     $\Delta$[Si/Fe] & $-$0.01 &    0.01 &    0.00 &    0.01 &    0.02 \\
     $\Delta$[Ca/Fe] & $-$0.02 & $-$0.01 &    0.00 &    0.02 &    0.03 \\
     $\Delta$[Sc/Fe] & $-$0.03 &    0.12 &    0.00 &    0.06 &    0.14 \\
   $\Delta$[\tii/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
  $\Delta$[\tiii/Fe] & $-$0.05 &    0.11 & $-$0.01 &    0.03 &    0.12 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Mn/Fe] &    0.01 &    0.02 &    0.01 &    0.07 &    0.07 \\
    $\Delta$[\fei/H] &    0.08 & $-$0.02 &    0.00 & $-$0.08 &    0.11 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.00 &    0.00 &    0.11 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.00 &    0.02 &    0.00 &    0.06 &    0.06 \\
     $\Delta$[Sr/Fe] & $-$0.02 &    0.11 &    0.00 &    0.04 &    0.12 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~2142-5656}
     $\Delta$[Na/Fe] &    0.01 & $-$0.06 & $-$0.01 & $-$0.08 &    0.10 \\
     $\Delta$[Mg/Fe] &    0.00 & $-$0.04 &    0.01 &    0.02 &    0.05 \\
     $\Delta$[Al/Fe] & $-$0.01 & $-$0.02 &    0.00 & $-$0.10 &    0.10 \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.04 &    0.01 &    0.00 &    0.06 &    0.07 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &    0.00 &    0.00 &    0.00 &    0.06 &    0.06 \\
  $\Delta$[\tiii/Fe] & $-$0.07 &    0.11 &    0.00 & $-$0.04 &    0.14 \\
     $\Delta$[Cr/Fe] &    0.01 & $-$0.01 &    0.01 & $-$0.05 &    0.05 \\
     $\Delta$[Mn/Fe] &    0.03 & $-$0.02 &    0.00 & $-$0.12 &    0.13 \\
    $\Delta$[\fei/H] &    0.12 & $-$0.02 &    0.00 & $-$0.08 &    0.15 \\
   $\Delta$[\feii/H] &    0.01 &    0.10 &    0.01 & $-$0.02 &    0.10 \\
     $\Delta$[Co/Fe] &    0.02 &    0.00 &    0.01 & $-$0.02 &    0.03 \\
     $\Delta$[Ni/Fe] &    0.02 &    0.00 &    0.00 & $-$0.05 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.03 &    0.07 & $-$0.01 & $-$0.17 &    0.19 \\
     $\Delta$[Ba/Fe] & $-$0.04 &    0.11 &    0.01 & $-$0.01 &    0.12 \\
\cutinhead{HE~2202-4831}
     $\Delta$[Na/Fe] &    0.03 & $-$0.13 &    0.00 &    0.05 &    0.14 \\
     $\Delta$[Mg/Fe] &    0.02 & $-$0.10 &    0.01 &    0.02 &    0.10 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.05 &    0.02 & $-$0.01 &    0.08 &    0.10 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &    0.00 &    0.03 &    0.00 &    0.08 &    0.09 \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.11 & $-$0.01 & $-$0.02 &    0.13 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.01 &    0.00 & $-$0.02 &    0.02 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.11 & $-$0.03 &    0.01 & $-$0.10 &    0.15 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.01 & $-$0.03 &    0.12 \\
     $\Delta$[Co/Fe] &    0.01 &    0.02 &    0.01 & $-$0.01 &    0.03 \\
     $\Delta$[Ni/Fe] & $-$0.01 &    0.03 &    0.00 &    0.07 &    0.08 \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] & $-$0.04 &    0.13 &    0.00 &    0.08 &    0.16 \\
\cutinhead{HE~2246-2410}
     $\Delta$[Na/Fe] & $-$0.01 & $-$0.09 & $-$0.01 & $-$0.01 &    0.09 \\
     $\Delta$[Mg/Fe] & $-$0.02 & $-$0.04 &    0.00 &    0.02 &    0.05 \\
     $\Delta$[Al/Fe] & $-$0.03 &    0.02 & $-$0.01 &    0.07 &    0.08 \\
     $\Delta$[Si/Fe] & $-$0.01 &    0.03 &    0.01 &    0.04 &    0.05 \\
     $\Delta$[Ca/Fe] & $-$0.04 &    0.00 & $-$0.01 &    0.04 &    0.06 \\
     $\Delta$[Sc/Fe] & $-$0.04 &    0.13 &    0.00 &    0.07 &    0.15 \\
   $\Delta$[\tii/Fe] &    0.00 &    0.03 &    0.00 &    0.07 &    0.08 \\
  $\Delta$[\tiii/Fe] & $-$0.06 &    0.13 & $-$0.01 &    0.07 &    0.16 \\
     $\Delta$[Cr/Fe] &    0.00 &    0.02 &    0.00 &    0.07 &    0.07 \\
     $\Delta$[Mn/Fe] &    0.00 &    0.02 &    0.00 &    0.07 &    0.07 \\
    $\Delta$[\fei/H] &    0.10 & $-$0.03 &    0.01 & $-$0.09 &    0.14 \\
   $\Delta$[\feii/H] &    0.02 &    0.11 &    0.00 & $-$0.01 &    0.11 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.00 &    0.02 & $-$0.01 &    0.05 &    0.05 \\
     $\Delta$[Sr/Fe] & $-$0.05 &    0.12 & $-$0.01 &    0.05 &    0.14 \\
     $\Delta$[Ba/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
\cutinhead{HE~2247-7400}
     $\Delta$[Na/Fe] &    0.00 & $-$0.05 & $-$0.02 & $-$0.09 &    0.10 \\
     $\Delta$[Mg/Fe] & $-$0.01 & $-$0.03 &    0.00 &    0.02 &    0.04 \\
     $\Delta$[Al/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Si/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ca/Fe] & $-$0.05 &    0.01 &    0.01 &    0.06 &    0.08 \\
     $\Delta$[Sc/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
   $\Delta$[\tii/Fe] &    0.01 &    0.01 &    0.01 &    0.07 &    0.07 \\
  $\Delta$[\tiii/Fe] & $-$0.08 &    0.12 &    0.01 & $-$0.04 &    0.15 \\
     $\Delta$[Cr/Fe] &    0.01 & $-$0.01 &    0.00 & $-$0.07 &    0.07 \\
     $\Delta$[Mn/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
    $\Delta$[\fei/H] &    0.13 & $-$0.02 &    0.00 & $-$0.09 &    0.16 \\
   $\Delta$[\feii/H] &    0.01 &    0.10 &    0.01 & $-$0.05 &    0.11 \\
     $\Delta$[Co/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ni/Fe] &    0.00 &    0.00 &    0.00 & $-$0.03 &    0.03 \\
     $\Delta$[Sr/Fe] &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
     $\Delta$[Ba/Fe] & $-$0.05 &    0.12 &    0.02 &    0.03 &    0.13 \\
\enddata

\tablenotetext{a}{Dwarf gravity is assumed (see Section 2.1 for details).}
\tablenotetext{b}{Subgiant gravity is assumed (see Section 2.1 for details).}

\end{deluxetable}


==> tab6.tex <==
\begin{deluxetable}{lccccccccc}
\tabletypesize{\scriptsize}
%\tabletypesize{\footnotesize}
\tablecolumns{9} 
\tablewidth{0pc} 
\tablecaption{Model Atmosphere Parameters and [Fe/H] for the Literature Sample\label{tab:param2}}
\tablehead{ 
\colhead{Star} & 
\colhead{RA2000\tablenotemark{a}} &
\colhead{DEC2000\tablenotemark{a}} &
\colhead{\teff} & 
\colhead{$\log g$} & 
\colhead{$\xi_t$} & 
\colhead{[M/H]$_{\rm model}$} & 
\colhead{[Fe/H]$_{\rm derived}$} & 
\colhead{C-rich\tablenotemark{b}} & 
\colhead{Source} \\
\colhead{} & 
\colhead{} &
\colhead{} &
\colhead{(K)} & 
\colhead{(cgs)} & 
\colhead{(\kms)} & 
\colhead{} & 
\colhead{} & 
\colhead{} \\
\colhead{(1)} & 
\colhead{(2)} &
\colhead{(3)} &
\colhead{(4)} & 
\colhead{(5)} & 
\colhead{(6)} & 
\colhead{(7)} & 
\colhead{(8)} & 
\colhead{(9)} & 
\colhead{(10)} 
}
\startdata 
 CS~22957-022 & 00 01 45.5 & $-$05 49 46.6 & 5146 & 2.40 & 1.5 & $-$2.9 & $-$2.92 & 0 &        14 \\
 CS~29503-010 & 00 04 55.4 & $-$24 24 19.3 & 6570 & 4.25 & 1.3 & $-$1.0 & $-$1.00 & 1 &         3 \\
 CS~31085-024 & 00 08 27.9 &   +10 54 19.8 & 5778 & 4.64 & 0.3 & $-$2.8 & $-$2.80 & 0 &        14 \\
 BS~17570-063 & 00 20 36.2 &   +23 47 37.7 & 6233 & 4.46 & 0.8 & $-$3.0 & $-$2.95 & 0 &         5 \\
 HE~0024-2523 & 00 27 27.7 & $-$25 06 28.2 & 6635 & 4.11 & 1.2 & $-$2.8 & $-$2.82 & 0 &         6 \\
 CS~29527-015 & 00 29 10.7 & $-$19 10 07.2 & 6577 & 3.89 & 1.9 & $-$3.3 & $-$3.32 & 1 &         5 \\
 CS~30339-069 & 00 30 16.0 & $-$35 56 51.2 & 6326 & 3.79 & 1.4 & $-$3.1 & $-$3.05 & 0 &         5 \\
 CS~31062-050 & 00 30 31.1 & $-$12 05 10.9 & 5607 & 3.49 & 0.3 & $-$2.3 & $-$2.28 & 1 &         1 \\
 HE~0028-2152 & 00 31 07.7 & $-$21 36 07.3 & 6184 & 3.75 & 1.5 & $-$2.8 & $-$2.74 & 0 &         9 \\
      HD~2796 & 00 31 16.9 & $-$16 47 40.9 & 4923 & 1.84 & 1.6 & $-$2.3 & $-$2.31 & 0 &         7 \\
 CS~31062-041 & 00 35 03.0 & $-$15 54 29.3 & 4990 & 2.00 & 2.0 & $-$2.6 & $-$2.65 & 0 &         3 \\
 SDSS 0036-10 & 00 36 02.2 & $-$10 43 36.3 & 6479 & 4.31 & 1.2 & $-$2.6 & $-$2.60 & 1 &         4 \\
 CS~29497-034 & 00 41 39.8 & $-$26 18 54.4 & 4983 & 1.96 & 2.0 & $-$3.0 & $-$3.00 & 1 &         3 \\
 CS~31062-012 & 00 44 03.6 & $-$13 55 25.9 & 6190 & 4.47 & 1.2 & $-$2.7 & $-$2.67 & 1 &     1,  4 \\
      HD~4306 & 00 45 27.2 & $-$09 32 39.9 & 4854 & 1.61 & 1.6 & $-$3.1 & $-$3.04 & 0 &        13 \\
CD -38$^\circ$ 245 & 00 46 36.2 & $-$37 39 33.5 & 4857 & 1.54 & 2.2 & $-$4.2 & $-$4.15 & 0 &         7 \\
 HE~0054-2123 & 00 56 53.2 & $-$21 07 29.6 & 6424 & 4.35 & 1.6 & $-$2.6 & $-$2.59 & 0 &         9 \\
 CS~22953-003 & 01 02 15.9 & $-$61 43 45.8 & 5002 & 2.01 & 1.6 & $-$3.0 & $-$2.93 & 0 &         7 \\
      HD~6268 & 01 03 18.2 & $-$27 52 49.9 & 4696 & 1.23 & 2.1 & $-$2.8 & $-$2.74 & 0 &        13 \\
 HE~0102-0633 & 01 05 25.7 & $-$06 17 35.4 & 6371 & 3.83 & 1.5 & $-$2.9 & $-$2.90 & 0 &         9 \\
 HE~0105-2202 & 01 07 31.2 & $-$21 46 06.5 & 6267 & 4.44 & 1.4 & $-$2.8 & $-$2.75 & 0 &         9 \\
 CS~22183-031 & 01 09 05.1 & $-$04 43 21.1 & 5202 & 2.54 & 1.1 & $-$3.2 & $-$3.17 & 0 &        13 \\
 HE~0107-5240 & 01 09 29.2 & $-$52 24 34.2 & 5100 & 2.20 & 2.2 & $-$5.3 & $-$5.54 & 1 &         8 \\
 CS~29518-020 & 01 12 13.2 & $-$31 00 05.3 & 6435 & 4.34 & 2.2 & $-$2.7 & $-$2.65 & 0 &         5 \\
 CS~22174-007 & 01 14 06.5 & $-$11 02 35.4 & 5265 & 2.78 & 1.9 & $-$2.4 & $-$2.39 & 0 &         3 \\
 CS~29518-043 & 01 18 38.3 & $-$30 41 02.7 & 6550 & 4.29 & 1.5 & $-$3.2 & $-$3.14 & 0 &         5 \\
 CS~29518-051 & 01 24 10.0 & $-$28 15 21.1 & 5100 & 2.29 & 1.1 & $-$2.6 & $-$2.64 & 0 &         7 \\
 CS~22953-037 & 01 25 06.6 & $-$59 16 00.7 & 6627 & 4.11 & 1.5 & $-$2.7 & $-$2.70 & 0 &         5 \\
 CS~31082-001 & 01 29 31.1 & $-$16 00 45.5 & 4866 & 1.66 & 1.4 & $-$2.9 & $-$2.75 & 0 &     7, 13 \\
 HE~0130-2303 & 01 33 18.2 & $-$22 48 36.8 & 6548 & 4.28 & 1.5 & $-$3.0 & $-$3.02 & 0 &         6 \\
 HE~0132-2439 & 01 34 58.9 & $-$24 24 18.6 & 5249 & 2.63 & 1.6 & $-$3.8 & $-$3.79 & 0 &     6, 11 \\
 HE~0142+0147 & 01 44 47.9 &   +02 02 17.9 & 6244 & 3.79 & 1.5 & $-$2.7 & $-$2.67 & 0 &         9 \\
 HE~0143-0441 & 01 45 37.9 & $-$04 26 43.4 & 6276 & 3.84 & 1.4 & $-$2.3 & $-$2.32 & 1 &     9, 10 \\
 HE~0148-2611 & 01 50 59.6 & $-$25 57 03.2 & 6605 & 4.23 & 1.3 & $-$3.1 & $-$3.05 & 0 &         6 \\
 HE~0206-1916 & 02 09 19.6 & $-$19 01 55.5 & 5073 & 2.23 & 2.0 & $-$2.5 & $-$2.52 & 1 &         3 \\
 HE~0218-2738 & 02 21 03.9 & $-$27 24 40.5 & 6593 & 4.29 & 1.5 & $-$3.6 & $-$3.57 & 0 &         6 \\
 CS~31061-032 & 02 38 43.3 &   +03 19 02.4 & 6448 & 4.33 & 1.3 & $-$2.6 & $-$2.56 & 0 &         5 \\
 CS~22189-009 & 02 41 42.4 & $-$13 28 10.5 & 4944 & 1.83 & 1.9 & $-$3.5 & $-$3.48 & 0 &         7 \\
 HE~0242-0732 & 02 45 00.7 & $-$07 19 42.1 & 6572 & 4.29 & 1.9 & $-$3.3 & $-$3.30 & 0 &         6 \\
 CS~22963-004 & 02 56 46.6 & $-$04 51 17.5 & 5597 & 3.34 & 1.7 & $-$3.5 & $-$3.54 & 0 &        14 \\
 CS~31078-018 & 03 01 00.7 &   +06 16 31.9 & 5100 & 2.27 & 1.5 & $-$3.0 & $-$2.99 & 0 &        14 \\
    LP 831-70 & 03 06 05.4 & $-$22 19 17.9 & 6408 & 4.37 & 1.7 & $-$3.0 & $-$2.95 & 0 &         9 \\
 CS~22968-014 & 03 06 29.5 & $-$54 30 32.5 & 4864 & 1.60 & 1.9 & $-$3.6 & $-$3.58 & 0 &         7 \\
 CS~22172-002 & 03 14 20.8 & $-$10 35 11.3 & 4893 & 1.68 & 2.0 & $-$3.8 & $-$3.77 & 0 &         7 \\
 HE~0336+0113 & 03 38 52.9 &   +01 23 07.8 & 5819 & 3.59 & 1.4 & $-$2.6 & $-$2.60 & 1 &        10 \\
 HE~0400-2030 & 04 02 14.8 & $-$20 21 53.5 & 5579 & 3.53 & 1.5 & $-$1.7 & $-$1.68 & 1 &         3 \\
 CS~22177-009 & 04 07 40.6 & $-$25 02 43.9 & 6423 & 4.37 & 1.3 & $-$3.0 & $-$2.98 & 0 &         5 \\
 CS~22169-035 & 04 12 13.9 & $-$12 05 05.1 & 4654 & 1.10 & 1.9 & $-$2.8 & $-$2.95 & 0 &     7, 13 \\
 CS~22186-025 & 04 24 32.8 & $-$37 09 02.6 & 4871 & 1.66 & 2.0 & $-$3.1 & $-$3.07 & 0 &         7 \\
 HE~0441-0652 & 04 43 29.9 & $-$06 46 53.5 & 4811 & 1.52 & 2.1 & $-$2.8 & $-$2.77 & 1 &         3 \\
   BD~+03$^\circ$ 740 & 05 01 16.6 &   +04 06 37.1 & 6485 & 4.31 & 1.6 & $-$2.7 & $-$2.70 & 0 &     6, 14 \\
 HE~0507-1653 & 05 09 16.6 & $-$16 50 04.6 & 4935 & 1.88 & 1.5 & $-$1.2 & $-$1.32 & 1 &         3 \\
 HE~0508-1555 & 05 10 35.5 & $-$15 51 38.3 & 6451 & 4.32 & 1.4 & $-$2.4 & $-$2.40 & 0 &         9 \\
 HE~0557-4840 & 05 58 39.3 & $-$48 39 56.8 & 4900 & 2.20 & 1.8 & $-$4.8 & $-$4.81 & 1 &        16 \\
 SDSS 0924+40 & 09 24 01.9 &   +40 59 28.8 & 6196 & 3.77 & 1.2 & $-$2.7 & $-$2.68 & 1 &         4 \\
 HE~1005-1439 & 10 07 52.4 & $-$14 54 21.0 & 5202 & 2.55 & 1.6 & $-$3.1 & $-$3.09 & 1 &         3 \\
     HD~88609 & 10 14 29.0 &   +53 33 39.4 & 4541 & 0.80 & 1.6 & $-$3.0 & $-$2.98 & 0 &        13 \\
 HE~1012-1540 & 10 14 53.5 & $-$15 55 53.2 & 5745 & 3.45 & 1.4 & $-$3.5 & $-$3.47 & 1 &        11 \\
 BS~16469-075 & 10 15 10.2 &   +42 53 17.3 & 4919 & 1.78 & 1.6 & $-$3.3 & $-$3.25 & 0 &        13 \\
 HE~1031-0020 & 10 34 24.2 & $-$00 36 08.4 & 5043 & 2.13 & 1.1 & $-$2.8 & $-$2.79 & 1 &        10 \\
 BS~16077-007 & 11 35 18.0 &   +31 00 23.7 & 6486 & 4.31 & 1.6 & $-$2.8 & $-$2.77 & 0 &        14 \\
 HE~1150-0428 & 11 53 06.6 & $-$04 45 03.4 & 5208 & 2.54 & 1.6 & $-$3.5 & $-$3.47 & 1 &        10 \\
 BS~16920-017 & 12 07 16.8 &   +41 39 32.5 & 4851 & 1.58 & 1.7 & $-$3.4 & $-$3.40 & 0 &        13 \\
 BS~16928-053 & 12 22 28.0 &   +34 11 31.8 & 4679 & 1.16 & 1.6 & $-$3.0 & $-$2.93 & 0 &    13, 14 \\
 BS~16085-050 & 12 37 46.7 &   +19 22 49.5 & 4910 & 1.76 & 1.8 & $-$3.2 & $-$3.16 & 0 &        13 \\
 BS~16076-006 & 12 48 22.8 &   +20 56 44.0 & 5566 & 3.32 & 1.7 & $-$3.5 & $-$3.51 & 0 &         5 \\
 HE~1300+0157 & 13 02 56.2 &   +01 41 52.1 & 5529 & 3.25 & 1.5 & $-$3.8 & $-$3.75 & 1 &    11, 12 \\
 BS~16929-005 & 13 03 29.5 &   +33 51 09.1 & 5229 & 2.61 & 1.6 & $-$3.4 & $-$3.34 & 1 & 3, 13, 14 \\
    HD~115444 & 13 16 42.5 &   +36 22 52.9 & 4711 & 1.23 & 0.7 & $-$2.7 & $-$2.65 & 0 &        13 \\
 HE~1320+0038 & 13 22 35.4 &   +00 22 32.6 & 6566 & 3.99 & 1.9 & $-$2.7 & $-$2.68 & 0 &         9 \\
 HE~1319-1935 & 13 22 38.7 & $-$19 51 11.6 & 4691 & 1.27 & 2.8 & $-$2.2 & $-$2.22 & 1 &         3 \\
 HE~1327-2326 & 13 30 06.0 & $-$23 41 49.7 & 6180 & 3.70 & 1.7 & $-$5.5 & $-$5.76 & 1 &         2 \\
 BS~16467-062 & 13 42 00.6 &   +17 48 40.9 & 5310 & 2.80 & 1.7 & $-$3.7 & $-$3.80 & 0 & 7, 11, 14 \\
 BS~16082-129 & 13 47 11.7 &   +28 57 47.1 & 4868 & 1.67 & 0.9 & $-$2.9 & $-$2.84 & 0 &        13 \\
 HE~1347-1025 & 13 50 22.4 & $-$10 40 18.9 & 5206 & 2.52 & 1.8 & $-$3.8 & $-$3.71 & 0 &        11 \\
 HE~1356-0622 & 13 59 30.3 & $-$06 36 35.0 & 4953 & 1.85 & 1.9 & $-$3.7 & $-$3.63 & 0 &        11 \\
 BS~16023-046 & 14 00 54.5 &   +22 46 42.3 & 6571 & 4.25 & 1.4 & $-$2.9 & $-$2.83 & 0 &         5 \\
    HD~122563 & 14 02 31.9 &   +09 41 10.1 & 4843 & 1.62 & 1.8 & $-$2.5 & $-$2.54 & 0 &     7, 13 \\
 BS~16550-087 & 14 10 26.7 &   +18 01 24.0 & 4754 & 1.32 & 2.2 & $-$3.6 & $-$3.54 & 0 &        14 \\
 HE~1424-0241 & 14 26 40.3 & $-$02 54 27.5 & 5260 & 2.66 & 1.6 & $-$4.1 & $-$4.05 & 0 &        11 \\
    HD~126587 & 14 27 00.4 & $-$22 14 38.9 & 4853 & 1.61 & 1.6 & $-$3.0 & $-$3.00 & 0 &        13 \\
 HE~1429-0551 & 14 32 31.3 & $-$06 05 00.3 & 4757 & 1.39 & 1.9 & $-$2.6 & $-$2.60 & 1 &         3 \\
 BS~16477-003 & 14 32 56.9 &   +06 46 07.0 & 4879 & 1.66 & 1.7 & $-$3.4 & $-$3.39 & 0 &         7 \\
 CS~30325-094 & 14 54 39.3 &   +04 21 38.1 & 4948 & 1.85 & 1.6 & $-$3.4 & $-$3.35 & 0 &         7 \\
 BS~16968-061 & 15 01 06.1 &   +03 42 45.5 & 6343 & 3.82 & 1.6 & $-$2.9 & $-$2.85 & 0 &         5 \\
 CS~30325-028 & 15 05 19.8 &   +06 17 07.0 & 4894 & 1.73 & 1.7 & $-$2.9 & $-$2.87 & 0 &        14 \\
 CS~30301-024 & 15 08 29.7 & $-$00 35 59.2 & 6584 & 4.03 & 1.5 & $-$2.6 & $-$2.54 & 0 &         5 \\
 CS~30301-015 & 15 08 56.8 &   +02 30 18.5 & 4889 & 1.73 & 2.4 & $-$2.8 & $-$2.73 & 1 &         1 \\
 CS~30306-132 & 15 14 18.9 &   +07 27 02.8 & 5047 & 2.16 & 1.5 & $-$2.6 & $-$2.56 & 0 &        13 \\
 CS~30312-059 & 15 34 48.8 & $-$01 23 37.3 & 4908 & 1.75 & 1.7 & $-$3.2 & $-$3.22 & 0 &        14 \\
    HD~140283 & 15 43 03.1 & $-$10 56 01.0 & 5711 & 3.53 & 1.1 & $-$2.6 & $-$2.56 & 0 &     6, 13 \\
 CS~30312-100 & 15 43 31.7 &   +02 01 17.4 & 5117 & 2.34 & 1.8 & $-$2.6 & $-$2.66 & 0 &         3 \\
 CS~22884-108 & 15 49 57.6 & $-$09 14 09.2 & 6107 & 4.52 & 1.2 & $-$3.3 & $-$3.30 & 0 &        14 \\
 BS~16084-160 & 16 28 50.8 &   +54 37 06.8 & 4727 & 1.27 & 2.0 & $-$3.2 & $-$3.20 & 0 &        14 \\
 CS~22872-102 & 16 29 20.7 & $-$03 04 56.6 & 5911 & 3.60 & 1.4 & $-$2.9 & $-$2.94 & 0 &        14 \\
 CS~22878-027 & 16 37 35.9 &   +10 22 07.8 & 6319 & 4.41 & 1.4 & $-$2.5 & $-$2.51 & 1 &        14 \\
 BS~16080-054 & 16 39 18.5 &   +60 57 42.6 & 4902 & 1.75 & 1.9 & $-$3.0 & $-$2.94 & 0 &        14 \\
 CS~22878-101 & 16 45 31.4 &   +08 14 45.5 & 4796 & 1.44 & 1.9 & $-$3.4 & $-$3.31 & 0 &     6,  7 \\
 BS~16080-093 & 16 50 38.3 &   +59 13 06.5 & 4945 & 1.85 & 1.9 & $-$3.2 & $-$3.23 & 0 &        14 \\
      G 139-8 & 17 01 44.0 &   +16 09 03.6 & 6266 & 4.42 & 1.0 & $-$2.1 & $-$2.03 & 0 &         6 \\
  BD~+17$^\circ$ 3248 & 17 28 14.5 &   +17 30 35.9 & 5240 & 2.72 & 1.5 & $-$2.2 & $-$2.17 & 0 &         7 \\
  BD~+23$^\circ$ 3130 & 17 32 41.6 &   +23 44 11.7 & 5262 & 2.76 & 1.4 & $-$2.5 & $-$2.52 & 0 &        14 \\
 CS~22891-209 & 19 42 02.2 & $-$61 03 44.7 & 4699 & 1.18 & 2.1 & $-$3.3 & $-$3.32 & 0 &         7 \\
 CS~22896-154 & 19 42 26.9 & $-$56 58 34.0 & 5100 & 2.28 & 1.4 & $-$2.9 & $-$2.85 & 0 &         7 \\
    HD~186478 & 19 45 14.1 & $-$17 29 26.9 & 4629 & 1.07 & 2.0 & $-$2.6 & $-$2.68 & 0 &     7, 13 \\
 CS~22873-055 & 19 53 49.8 & $-$59 40 00.2 & 4551 & 0.82 & 2.1 & $-$3.0 & $-$2.99 & 0 &         7 \\
  BD~-18$^\circ$ 5550 & 19 58 49.7 & $-$18 12 10.9 & 4558 & 0.81 & 1.7 & $-$3.2 & $-$3.20 & 1 &         7 \\
 CS~22873-166 & 20 19 22.0 & $-$61 30 14.9 & 4516 & 0.77 & 1.6 & $-$2.7 & $-$2.74 & 1 &         7 \\
 CS~22885-096 & 20 20 51.2 & $-$39 53 30.2 & 4992 & 1.93 & 1.8 & $-$3.9 & $-$3.86 & 0 &         7 \\
 CS~22950-046 & 20 21 28.4 & $-$13 16 33.6 & 4769 & 1.37 & 1.7 & $-$3.4 & $-$3.39 & 0 &         6 \\
    HD~196944 & 20 40 46.1 & $-$06 47 50.6 & 5255 & 2.74 & 1.6 & $-$2.5 & $-$2.44 & 1 &         1 \\
 CS~22880-086 & 20 45 47.5 & $-$18 33 32.4 & 5196 & 2.54 & 1.5 & $-$3.1 & $-$3.05 & 0 &        14 \\
 CS~22880-074 & 20 46 03.2 & $-$20 59 14.2 & 5621 & 3.50 & 1.3 & $-$2.3 & $-$2.29 & 1 &         1 \\
 SDSS 2047+00 & 20 47 28.8 &   +00 15 53.8 & 6383 & 4.36 & 1.0 & $-$2.4 & $-$2.36 & 1 &         4 \\
 CS~22897-008 & 21 03 11.9 & $-$65 05 08.8 & 4795 & 1.43 & 1.9 & $-$3.5 & $-$3.50 & 1 &         7 \\
 CS~29498-043 & 21 03 52.1 & $-$29 42 50.2 & 4639 & 1.00 & 1.7 & $-$3.5 & $-$3.49 & 1 &         1 \\
 CS~29506-007 & 21 20 28.7 & $-$20 46 22.9 & 6522 & 3.94 & 1.7 & $-$2.8 & $-$2.73 & 0 &     5, 14 \\
 CS~29506-090 & 21 30 28.9 & $-$22 10 41.4 & 6603 & 4.18 & 1.6 & $-$2.6 & $-$2.62 & 0 &         5 \\
 HE~2133-1426 & 21 36 07.2 & $-$14 12 35.4 & 6350 & 4.40 & 1.5 & $-$2.9 & $-$2.89 & 0 &         6 \\
 CS~29495-041 & 21 36 33.3 & $-$28 18 48.6 & 4740 & 1.34 & 1.5 & $-$2.8 & $-$2.74 & 0 &         7 \\
 CS~22948-027 & 21 37 45.8 & $-$39 27 22.3 & 5011 & 2.06 & 1.9 & $-$2.6 & $-$2.45 & 1 &         3 \\
 BS~17583-100 & 21 42 27.8 &   +26 40 35.5 & 5950 & 3.66 & 1.2 & $-$2.5 & $-$2.53 & 0 &        13 \\
 CS~22948-066 & 21 44 51.2 & $-$37 27 55.0 & 5077 & 2.20 & 1.9 & $-$3.2 & $-$3.20 & 0 &         7 \\
 CS~22944-032 & 21 47 43.2 & $-$13 40 22.8 & 5293 & 2.82 & 1.4 & $-$3.0 & $-$2.98 & 0 &        14 \\
 CS~22948-093 & 21 50 31.5 & $-$41 07 49.3 & 6609 & 4.23 & 1.5 & $-$3.2 & $-$3.17 & 0 &         5 \\
 CS~22956-050 & 21 58 05.8 & $-$65 13 27.1 & 4844 & 1.56 & 1.8 & $-$3.4 & $-$3.39 & 0 &         7 \\
 HE~2158-0348 & 22 00 40.0 & $-$03 34 12.2 & 5150 & 2.44 & 0.6 & $-$2.5 & $-$2.57 & 1 &        10 \\
 BS~17569-049 & 22 04 58.4 &   +04 01 32.1 & 4645 & 1.09 & 1.7 & $-$2.9 & $-$2.84 & 0 &         7 \\
 CS~22965-054 & 22 06 30.3 & $-$02 32 34.4 & 6137 & 3.68 & 1.5 & $-$3.1 & $-$3.10 & 0 &     5, 14 \\
 HE~2209-1240 & 22 11 48.8 & $-$12 25 45.4 & 6319 & 3.84 & 1.6 & $-$2.6 & $-$2.59 & 0 &         9 \\
 CS~22892-052 & 22 17 01.7 & $-$16 39 27.1 & 4825 & 1.54 & 1.6 & $-$3.1 & $-$3.03 & 1 &     7, 13 \\
 CS~22886-042 & 22 20 25.8 & $-$10 23 20.2 & 4798 & 1.48 & 2.0 & $-$2.8 & $-$2.83 & 0 &         3 \\
 CS~29502-042 & 22 21 48.8 &   +02 28 44.9 & 5039 & 2.09 & 1.6 & $-$3.3 & $-$3.27 & 0 &         7 \\
 CS~29502-092 & 22 22 36.0 & $-$01 38 27.5 & 5074 & 2.21 & 1.5 & $-$3.0 & $-$2.99 & 1 &        14 \\
 HE~2221-0453 & 22 24 25.6 & $-$04 38 02.2 & 4430 & 0.73 & 1.4 & $-$2.0 & $-$2.00 & 1 &         3 \\
 CS~29516-024 & 22 26 15.4 &   +02 51 46.3 & 4637 & 1.04 & 1.6 & $-$3.1 & $-$3.05 & 0 &         7 \\
 HE~2228-0706 & 22 31 24.5 & $-$06 50 51.2 & 5003 & 2.02 & 1.6 & $-$2.8 & $-$2.78 & 1 &         3 \\
 HE~2232-0603 & 22 34 47.4 & $-$05 48 17.3 & 6085 & 3.85 & 1.0 & $-$1.5 & $-$1.46 & 1 &        10 \\
 CS~29491-053 & 22 36 56.3 & $-$28 31 06.5 & 4700 & 1.21 & 1.9 & $-$3.0 & $-$3.03 & 0 &         7 \\
CD -24$^\circ$ 17504 & 23 07 20.2 & $-$23 52 35.6 & 6236 & 3.70 & 1.6 & $-$3.4 & $-$3.38 & 0 &        15 \\
 CS~22888-031 & 23 11 32.5 & $-$35 26 42.9 & 6241 & 4.47 & 1.3 & $-$3.3 & $-$3.31 & 0 &         5 \\
 CS~30338-089 & 23 15 50.0 &   +10 19 26.2 & 4886 & 1.72 & 1.6 & $-$2.8 & $-$2.78 & 1 &         3 \\
 HE~2323-0256 & 23 26 29.8 & $-$02 39 57.9 & 4958 & 1.84 & 1.9 & $-$4.0 & $-$3.97 & 1 &     7, 11 \\
 HE~2330-0555 & 23 32 54.8 & $-$05 38 50.6 & 4867 & 1.65 & 1.6 & $-$3.0 & $-$2.98 & 1 &         3 \\
 CS~22966-011 & 23 35 07.0 & $-$30 22 54.4 & 6298 & 4.43 & 1.3 & $-$3.0 & $-$3.02 & 0 &         5 \\
 CS~22952-015 & 23 37 28.7 & $-$05 47 56.6 & 4824 & 1.50 & 1.9 & $-$3.5 & $-$3.44 & 0 &     7, 13 \\
 HE~2341-2029 & 23 44 19.6 & $-$20 13 19.8 & 6507 & 4.29 & 1.7 & $-$2.6 & $-$2.60 & 0 &         9 \\
 CS~29522-046 & 23 44 59.9 &   +08 46 52.9 & 5974 & 3.72 & 1.3 & $-$2.1 & $-$2.12 & 0 &        14 \\
 HE~2344-2800 & 23 46 44.4 & $-$27 44 10.7 & 6624 & 4.11 & 1.7 & $-$2.7 & $-$2.65 & 0 &         6 \\
 CS~22966-057 & 23 48 57.8 & $-$29 39 22.9 & 5364 & 3.07 & 1.0 & $-$2.4 & $-$2.43 & 0 &         7 \\
 CS~29499-060 & 23 53 40.3 & $-$26 58 44.0 & 6595 & 4.05 & 1.6 & $-$2.5 & $-$2.50 & 0 &         5 \\
 HE~2356-0410 & 23 59 13.1 & $-$03 53 48.2 & 5170 & 2.45 & 1.4 & $-$3.2 & $-$3.19 & 1 &     1, 10 \\
\enddata

%\tablenotetext{a}{For literature stars, \teff, $\log g$, $\xi_t$, and [Fe/H] 
%have been re-computed. However, the [C/Fe] is the value in the literature 
%reference.}

\tablerefs{
1 = \citet{aoki02}; 
2 = \citet{aoki06};
3 = \citet{aoki07}; 
4 = \citet{aoki08}; 
5 = \citet{bonifacio07,bonifacio09}; 
6 = \citet{carretta02,cohen02}; 
7 = \citet{cayrel04}; 
8 = \citet{christlieb04}; 
9 = \citet{cohen04}; 
10 = \citet{cohen06}; 
11 = \citet{cohen08}; 
12 = \citet{frebel07}; 
13 = \citet{honda04}; 
14 = \citet{lai08}; 
15 = \citet{norris01}; 
16 = \citet{norris07}; 
%1 = \citet{aoki02};
%2 = \citet{aoki07};
%3 = \citet{aoki08};
%4 = \citet{bonifacio07,bonifacio09}; 
%5 = \citet{carretta02}; 
%6 = \citet{cayrel04,spite05}; 
%7 = \citet{cohen04}; 
%8 = \citet{cohen06}; 
%9 = \citet{cohen08}; 
%10 = \citet{honda04}; 
%11 = \citet{lai08}; 
%12 = \citet{norris01}
}

\tablenotetext{a}{Coordinates are from the 2MASS database \citep{2mass}.}
\tablenotetext{b}{1 = CEMP object, adopting the \citet{aoki07} definition and 0 = C-normal (see Section 7.1 for details).}

\end{deluxetable} 


==> tab7.tex <==
\begin{deluxetable}{lrrrrrrrrrrrrrrrrr} 
\tabletypesize{\tiny}
\rotate
\tablecolumns{17} 
\tablewidth{0pc} 
\tablecaption{Chemical Abundances (C-Ba) for the Literature Sample \label{tab:abund2}}
\tablehead{ 
\colhead{Star} & 
\colhead{[C/Fe]\tablenotemark{a}} &
\colhead{[N/Fe]\tablenotemark{a}} &
\colhead{[Na/Fe]} &
\colhead{[Mg/Fe]} &
\colhead{[Al/Fe]} &
\colhead{[Si/Fe]} &
\colhead{[Ca/Fe]} &
\colhead{[Sc/Fe]} &
\colhead{[Ti\,{\sc i}/Fe]} &
\colhead{[Ti\,{\sc ii}/Fe]} &
\colhead{[Cr/Fe]} &
\colhead{[Mn/Fe]} &
\colhead{[\feii/H]} &
\colhead{[Co/Fe]} &
\colhead{[Ni/Fe]} &
\colhead{[Sr/Fe]} &
\colhead{[Ba/Fe]} \\ 
\colhead{(1)} &
\colhead{(2)} &
\colhead{(3)} &
\colhead{(4)} &
\colhead{(5)} &
\colhead{(6)} &
\colhead{(7)} &
\colhead{(8)} &
\colhead{(9)} &
\colhead{(10)} &
\colhead{(11)} &
\colhead{(12)} &
\colhead{(13)} &
\colhead{(14)} &
\colhead{(15)} &
\colhead{(16)} &
\colhead{(17)} &
\colhead{(18)} 
}
\startdata 
 CS~22957-022 &     0.16 &     0.21 &  \ldots &    0.21 &  \ldots &  \ldots &    0.27 &    0.07 &    0.30 &    0.32 & $-$0.31 & $-$0.68 & $-$2.87 &    0.11 &    0.02 & $-$0.19 & $-$1.09 \\
 CS~29503-010 &     1.07 &  $<$1.28 & $-$0.04 & $-$0.06 &  \ldots &  \ldots &    0.11 &  \ldots &    0.28 &    0.21 &  \ldots &  \ldots & $-$1.34 &  \ldots &  \ldots &  \ldots &    1.51 \\
 CS~31085-024 &     0.36 & $<-$0.24 &  \ldots &    0.08 &  \ldots &    0.39 &    0.28 &    0.33 &    0.33 &    0.50 & $-$0.12 & $-$0.60 & $-$2.70 &    0.24 &    0.28 &    0.04 & $-$0.57 \\
 BS~17570-063 &     0.40 &   \ldots &  \ldots &    0.28 &  \ldots &    0.51 &    0.33 &    0.77 &    0.60 &    0.70 & $-$0.14 &  \ldots & $-$3.01 &    0.44 &    0.20 & $-$0.02 &  \ldots \\
 HE~0024-2523 &   \ldots &   \ldots &  \ldots &    0.82 & $-$0.49 &  \ldots &    0.54 &    0.25 &    0.63 &    0.35 & $-$0.38 &  \ldots & $-$2.78 &  \ldots &  \ldots &    0.46 &    1.88 \\
 CS~29527-015 &     1.18 &   \ldots &  \ldots &    0.50 &  \ldots &  \ldots &    0.58 &    0.46 &  \ldots &    0.53 &    0.05 &  \ldots &  \ldots &    0.65 &    0.22 &    0.04 &  \ldots \\
 CS~30339-069 &     0.56 &   \ldots &  \ldots &    0.55 &  \ldots &  \ldots &    0.72 &    0.44 &  \ldots &    0.72 &    0.13 &  \ldots & $-$3.08 &    0.53 &    0.32 &    0.43 &  \ldots \\
 CS~31062-050 &     2.00 &     1.20 &  \ldots &    0.12 & $-$0.45 &  \ldots &  \ldots &  \ldots &    0.34 &    0.67 &  \ldots &  \ldots & $-$2.20 &  \ldots &  \ldots &  \ldots &  \ldots \\
 HE~0028-2152 &   \ldots &   \ldots &  \ldots &    0.48 & $-$0.63 &    0.30 &    0.47 &    0.22 &    0.64 &    0.47 & $-$0.12 & $-$0.65 & $-$2.85 &    0.34 &    0.09 & $-$0.26 & $-$0.54 \\
      HD~2796 &  $-$0.50 &     0.85 &    0.45 &    0.06 & $-$0.51 &  \ldots &    0.23 &    0.43 &    0.12 &    0.50 & $-$0.15 &  \ldots & $-$2.19 & $-$0.06 &    0.04 &  \ldots &  \ldots \\
 CS~31062-041 &     0.58 &  $<$1.59 &    0.40 &    0.32 &  \ldots &  \ldots &    0.34 &  \ldots &    0.29 &    0.30 &  \ldots &  \ldots & $-$2.59 &  \ldots &  \ldots &  \ldots & $-$0.42 \\
 SDSS 0036-10 &     2.32 &   \ldots &    0.79 &    0.14 &  \ldots &  \ldots &    0.31 &  \ldots &  \ldots &    0.35 & $-$0.09 &  \ldots & $-$2.48 &    0.25 & $-$0.07 & $-$0.07 &    0.40 \\
 CS~29497-034 &     2.72 &     2.63 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    0.66 &    0.56 & $-$0.11 &  \ldots & $-$3.01 &  \ldots &  \ldots &  \ldots &    2.28 \\
 CS~31062-012 &     2.12 &     1.20 &    1.18 &    0.20 & $-$0.68 &  \ldots &    0.21 &  \ldots &    0.50 &    0.37 & $-$0.17 &  \ldots & $-$2.60 &    0.24 &    0.07 &    0.33 &    2.32 \\
      HD~4306 &     0.11 &   \ldots &  \ldots &    0.47 & $-$0.44 &  \ldots &    0.51 &  \ldots &    0.42 &    0.51 & $-$0.09 & $-$0.68 & $-$3.00 &    0.12 &    0.02 &    0.04 &  \ldots \\
   CD -38$^\circ$ 245 & $<-$0.33 &     1.07 &    0.03 &    0.17 & $-$0.65 &  \ldots &    0.22 &    0.10 &    0.44 &    0.29 & $-$0.40 &  \ldots & $-$4.11 &    0.35 & $-$0.14 &  \ldots &  \ldots \\
 HE~0054-2123 &   \ldots &   \ldots &  \ldots &    0.34 & $-$0.61 &    0.27 &    0.42 &    0.39 &    0.62 &    0.59 & $-$0.06 & $-$0.81 & $-$2.60 &    0.23 &    0.17 & $-$0.10 & $-$0.27 \\
 CS~22953-003 &     0.30 &     0.12 &    0.32 &    0.20 & $-$0.91 &  \ldots &    0.24 &    0.07 &    0.19 &    0.15 & $-$0.41 &  \ldots & $-$2.90 &    0.02 & $-$0.03 &  \ldots &  \ldots \\
      HD~6268 &  $-$0.67 &   \ldots &  \ldots &    0.30 & $-$0.46 &  \ldots &    0.39 &  \ldots &    0.29 &    0.45 &  \ldots & $-$0.53 & $-$2.62 & $-$0.01 & $-$0.15 &    0.25 &  \ldots \\
 HE~0102-0633 &   \ldots &   \ldots &  \ldots &    0.44 & $-$0.65 &    0.29 &    0.53 &    0.19 &  \ldots &    0.26 & $-$0.20 & $-$0.63 & $-$2.84 &    0.45 &    0.19 & $-$0.39 & $-$0.08 \\
 HE~0105-2202 &   \ldots &   \ldots &  \ldots &    0.29 & $-$0.78 &    0.39 &    0.31 &    0.20 &    0.78 &    0.49 & $-$0.18 & $-$0.69 & $-$2.52 &    0.50 & $-$0.12 & $-$0.15 & $-$0.27 \\
 CS~22183-031 &     0.42 &   \ldots &  \ldots &    0.25 & $-$0.49 &  \ldots &    0.32 &  \ldots &    0.63 &    0.41 &  \ldots & $-$0.70 & $-$3.13 &    0.24 &    0.15 &    0.26 &  \ldots \\
 HE~0107-5240 &     3.85 &     2.43 &    1.11 &    0.26 &  \ldots &  \ldots &    0.12 &  \ldots &  \ldots &    0.04 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots \\
 CS~29518-020 &   \ldots &   \ldots &  \ldots &    0.00 &  \ldots &  \ldots &    0.26 &  \ldots &  \ldots &  \ldots & $-$0.28 &  \ldots &  \ldots &  \ldots & $-$0.08 &  \ldots &  \ldots \\
 CS~22174-007 &     0.41 &  $<$1.42 &    0.26 &    0.19 &  \ldots &  \ldots &    0.30 &  \ldots &    0.39 &    0.38 & $-$0.09 &  \ldots & $-$2.34 &  \ldots &  \ldots &  \ldots & $-$0.14 \\
 CS~29518-043 &   \ldots &   \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    0.80 &  \ldots &  \ldots &    0.77 &  \ldots &  \ldots & $-$3.03 &  \ldots &    0.63 &  \ldots &  \ldots \\
 CS~29518-051 &  $-$0.13 &     0.82 &    0.48 &    0.16 & $-$0.70 &  \ldots &    0.30 &    0.23 &    0.26 &    0.45 & $-$0.20 &  \ldots & $-$2.75 &    0.03 &    0.13 &  \ldots &  \ldots \\
 CS~22953-037 &     0.37 &   \ldots &  \ldots &  \ldots &  \ldots &  \ldots & $-$0.18 &  \ldots &    0.75 & $-$0.04 & $-$0.61 &  \ldots & $-$2.80 &  \ldots & $-$0.37 & $-$0.50 &  \ldots \\
 CS~31082-001 &     0.16 &  $-$0.51 &    0.46 &    0.29 & $-$0.57 &  \ldots &    0.31 &    0.18 &    0.44 &    0.38 & $-$0.31 & $-$0.48 & $-$2.76 &    0.02 &    0.18 &    0.63 &  \ldots \\
 HE~0130-2303 &   \ldots &   \ldots &  \ldots &    0.12 & $-$0.78 & $-$0.07 &    0.39 &    0.28 &  \ldots &    0.50 & $-$0.06 & $-$0.50 &  \ldots &  \ldots &  \ldots &    0.09 & $-$0.71 \\
 HE~0132-2439 &     0.62 &     1.07 &    0.07 &    0.32 & $-$0.61 &    0.66 &    0.36 &    1.05 &    0.70 &    0.50 & $-$0.36 & $-$0.86 & $-$3.62 &    0.44 &    0.06 &    0.30 & $-$0.88 \\
 HE~0142+0147 &   \ldots &   \ldots &  \ldots &    0.54 & $-$0.55 &    0.45 &    0.46 &  \ldots &    0.67 &    0.37 & $-$0.26 & $-$0.51 & $-$2.63 &    0.54 &    0.20 & $-$0.09 & $-$0.32 \\
 HE~0143-0441 &     1.82 &     0.85 &  \ldots &    0.65 & $-$0.64 &  \ldots &  \ldots &  \ldots &    0.57 &    0.42 & $-$0.30 & $-$0.82 & $-$2.44 &    0.47 & $-$0.18 &    1.09 &    2.42 \\
 HE~0148-2611 &   \ldots &   \ldots &  \ldots & $-$0.02 & $-$0.89 &  \ldots &    0.15 &    0.21 &  \ldots &    0.14 & $-$0.21 &  \ldots &  \ldots &  \ldots &  \ldots & $-$0.97 &  \ldots \\
 HE~0206-1916 &     2.10 &     1.61 &    0.73 &    0.40 &  \ldots &  \ldots &    0.41 &  \ldots &    0.55 &    0.50 &    0.07 &  \ldots & $-$2.39 &  \ldots &  \ldots &  \ldots &    1.99 \\
 HE~0218-2738 &   \ldots &   \ldots &  \ldots &    0.05 & $-$0.59 &    0.05 &    0.11 &    0.54 &  \ldots &    0.57 & $-$0.10 &  \ldots &  \ldots &  \ldots &  \ldots & $-$0.38 &  \ldots \\
 CS~31061-032 &     0.56 &   \ldots &  \ldots & $-$0.15 &  \ldots &  \ldots &    0.00 & $-$0.11 &    0.28 &    0.09 &  \ldots &  \ldots & $-$2.56 & $-$0.10 & $-$0.34 &  \ldots &  \ldots \\
 CS~22189-009 &     0.31 &     0.27 & $-$0.19 &    0.09 & $-$0.90 &  \ldots &    0.20 &    0.08 &    0.17 &    0.12 & $-$0.44 &  \ldots & $-$3.46 &    0.29 &    0.09 &  \ldots &  \ldots \\
 HE~0242-0732 &   \ldots &   \ldots &  \ldots &    0.33 & $-$0.69 &    0.29 &    0.29 &    0.24 &  \ldots &    0.20 & $-$0.14 &  \ldots & $-$3.48 &  \ldots &  \ldots & $-$1.20 &  \ldots \\
 CS~22963-004 &     0.40 &     0.80 &  \ldots &    0.34 & $-$0.73 &    0.58 &    0.38 &    0.35 &  \ldots &    0.44 & $-$0.30 & $-$0.83 & $-$3.44 &    0.47 &    0.11 & $-$0.68 & $-$0.51 \\
 CS~31078-018 &     0.37 &  $-$0.38 &  \ldots &    0.47 & $-$0.78 &  \ldots &    0.48 &    0.03 &    0.30 &    0.26 & $-$0.27 & $-$0.37 & $-$3.05 &    0.13 &    0.13 &  \ldots &    0.38 \\
    LP 831-70 &   \ldots &   \ldots &  \ldots &    0.49 & $-$0.41 &    0.24 &    0.10 &    0.44 &  \ldots &    0.30 & $-$0.22 & $-$0.62 & $-$2.93 &    0.65 &    0.03 & $-$1.48 &  \ldots \\
 CS~22968-014 &     0.25 &     0.24 & $-$0.24 &    0.21 & $-$0.72 &  \ldots &    0.02 &    0.08 &    0.14 &    0.02 & $-$0.46 &  \ldots & $-$3.56 &    0.47 &    0.27 &  \ldots &  \ldots \\
 CS~22172-002 &     0.00 &     0.24 & $-$0.28 &    0.15 & $-$0.80 &  \ldots &    0.24 &    0.00 &    0.37 &    0.26 & $-$0.44 &  \ldots & $-$3.73 &    0.41 & $-$0.10 &  \ldots &  \ldots \\
 HE~0336+0113 &     2.25 &     1.60 &  \ldots &    1.03 &    0.13 &  \ldots &    0.42 &  \ldots &    0.46 &    0.13 & $-$0.18 & $-$0.20 &  \ldots &    0.13 &  \ldots &    1.87 &    2.69 \\
 HE~0400-2030 &     1.14 &     2.75 &    0.45 &    0.28 &  \ldots &  \ldots &    0.12 &  \ldots &    0.17 &    0.43 &    0.11 &  \ldots & $-$1.80 &  \ldots &  \ldots &  \ldots &    1.85 \\
 CS~22177-009 &     0.38 &   \ldots &  \ldots &    0.24 &  \ldots &    0.10 &    0.42 &    0.27 &  \ldots &    0.47 & $-$0.07 &  \ldots & $-$2.96 &    0.47 &    0.08 & $-$0.18 &  \ldots \\
 CS~22169-035 &  $-$0.24 &     1.02 &  \ldots & $-$0.04 & $-$0.89 &  \ldots &    0.13 & $-$0.08 & $-$0.07 & $-$0.09 & $-$0.46 & $-$0.36 & $-$2.91 & $-$0.33 & $-$0.27 & $-$0.59 &  \ldots \\
 CS~22186-025 &  $-$0.54 &     0.98 &    0.48 &    0.32 & $-$0.72 &  \ldots &    0.36 &    0.28 &    0.36 &    0.50 & $-$0.36 &  \ldots & $-$2.91 &    0.09 &    0.00 &  \ldots &  \ldots \\
 HE~0441-0652 &     1.38 &     0.89 &    0.65 &    0.21 &  \ldots &  \ldots &    0.38 &  \ldots &    0.37 &    0.32 &  \ldots &  \ldots & $-$2.75 &  \ldots &  \ldots &  \ldots &    1.20 \\
    BD +03$^\circ$ 740 &     0.59 &  $<$0.29 &  \ldots &    0.15 & $-$0.83 &    0.17 &    0.39 &    0.37 &    0.69 &    0.60 & $-$0.07 & $-$0.51 & $-$2.61 &    0.35 &    0.06 & $-$0.08 & $-$0.42 \\
 HE~0507-1653 &     1.29 &     0.80 &    0.20 &    0.10 &  \ldots &  \ldots &    0.53 &  \ldots &    0.40 &    0.02 &  \ldots &  \ldots & $-$1.76 &  \ldots &  \ldots &  \ldots &    1.56 \\
 HE~0508-1555 &   \ldots &   \ldots &  \ldots &    0.34 & $-$0.65 &    0.31 &    0.30 &    0.28 &    0.67 &    0.54 & $-$0.21 & $-$0.65 & $-$2.50 &    0.30 &    0.09 &    0.48 & $-$0.13 \\
 HE~0557-4840 &     1.65 &  $<$1.93 & $-$0.18 &    0.17 & $-$0.65 &  \ldots &    0.17 &  \ldots &  \ldots &    0.36 & $-$0.69 &  \ldots &  \ldots &  \ldots & $-$0.17 &  \ldots &  \ldots \\
 SDSS 0924+40 &     2.72 &   \ldots &    1.29 &    0.39 &  \ldots &  \ldots &    0.22 &  \ldots &  \ldots &    0.21 & $-$0.21 &  \ldots & $-$2.67 &  \ldots &    0.15 &    0.77 &    1.73 \\
 HE~1005-1439 &     2.48 &     1.79 &    1.05 &    0.33 &  \ldots &  \ldots &    0.54 &  \ldots &    0.49 &    0.31 & $-$0.34 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    1.17 \\
     HD~88609 &  $-$0.51 &   \ldots &  \ldots &    0.28 & $-$0.42 &  \ldots &    0.25 &  \ldots &    0.18 &    0.51 & $-$0.30 & $-$0.79 & $-$3.07 & $-$0.31 & $-$0.07 &    0.17 &  \ldots \\
 HE~1012-1540 &     2.22 &     1.25 &    1.93 &    1.85 &    0.65 &  \ldots &    0.70 &  \ldots &  \ldots &    0.06 & $-$0.24 & $-$0.51 &  \ldots &    0.23 & $-$0.22 & $-$0.37 & $-$0.25 \\
 BS~16469-075 &     0.21 &   \ldots &  \ldots &    0.24 & $-$0.74 &  \ldots &    0.33 &  \ldots &    0.27 &    0.27 &  \ldots & $-$0.77 & $-$3.19 &    0.18 & $-$0.05 &    0.25 &  \ldots \\
 HE~1031-0020 &     1.63 &     2.48 &  \ldots &    0.48 &    0.66 &  \ldots &    0.96 &  \ldots &    0.33 &    1.13 & $-$0.30 &    0.00 & $-$3.02 &  \ldots &  \ldots &    0.52 &    1.61 \\
 BS~16077-007 &     0.60 &  $<$0.80 &  \ldots &    0.28 &  \ldots &    0.23 &    0.49 &    0.30 &    0.67 &    0.52 & $-$0.12 & $-$0.58 & $-$2.78 &    0.30 &    0.10 &    0.26 & $-$0.23 \\
 HE~1150-0428 &     2.37 &     2.52 &  \ldots &    0.41 &  \ldots &  \ldots &    1.16 &  \ldots &    0.59 &    0.73 & $-$0.56 &  \ldots &  \ldots &  \ldots &  \ldots & $-$0.12 & $-$0.48 \\
 BS~16920-017 & $<-$0.07 &   \ldots &  \ldots &    0.11 & $-$0.70 &  \ldots &    0.16 &  \ldots &    0.55 &    0.57 & $-$0.13 & $-$0.23 & $-$3.18 &    0.19 &    0.21 & $-$0.36 &  \ldots \\
 BS~16928-053 &  $-$0.24 &     1.05 &    0.17 &    0.09 & $-$0.79 &  \ldots &    0.18 &  \ldots &    0.00 &    0.23 & $-$0.14 & $-$0.74 & $-$2.99 & $-$0.20 & $-$0.16 & $-$0.04 & $-$0.79 \\
 BS~16085-050 & $<-$0.52 &   \ldots &  \ldots &    0.56 & $-$0.46 &  \ldots &    0.44 &  \ldots &    0.27 &    0.36 & $-$0.38 & $-$0.37 & $-$3.03 &    0.12 &    0.20 & $-$1.57 &  \ldots \\
 BS~16076-006 &     0.34 &   \ldots &  \ldots &    0.44 &  \ldots &    0.31 &    0.72 &    0.38 &    0.73 &    0.63 & $-$0.09 &  \ldots & $-$3.58 &    0.38 &    0.07 &  \ldots &  \ldots \\
 HE~1300+0157 &     1.31 &  $<$0.71 & $-$0.02 &    0.33 & $-$0.64 &  \ldots &    0.39 &    0.30 &    0.62 &    0.36 & $-$0.38 & $-$0.76 & $-$3.78 &    0.49 &    0.08 & $-$1.36 &  \ldots \\
 BS~16929-005 &     0.99 &     0.32 &    0.03 &    0.30 & $-$0.72 &  \ldots &    0.34 &    0.01 &    0.52 &    0.40 & $-$0.35 & $-$0.78 & $-$3.27 &    0.28 &    0.07 &    0.54 & $-$0.41 \\
    HD~115444 &  $-$0.41 &   \ldots &  \ldots &    0.05 & $-$0.31 &  \ldots &    0.22 &  \ldots &    0.17 &    0.68 &    0.13 & $-$0.70 & $-$2.88 & $-$0.09 &    0.28 &    0.26 &  \ldots \\
 HE~1320+0038 &   \ldots &   \ldots &  \ldots &    0.36 & $-$0.60 &    0.05 &    0.34 &    0.17 &  \ldots &    0.43 & $-$0.11 & $-$0.50 & $-$2.61 &    0.44 &    0.06 & $-$0.46 & $-$0.41 \\
 HE~1319-1935 &     1.45 &     0.46 &  \ldots &    0.36 &  \ldots &  \ldots &    0.61 &  \ldots &  \ldots &    0.32 &  \ldots &  \ldots & $-$2.12 &  \ldots &  \ldots &  \ldots &    1.68 \\
 HE~1327-2326 &     4.26 &     4.56 &    2.48 &    1.55 &    1.23 &  \ldots &    0.29 &  \ldots &  \ldots &    0.80 &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    1.04 &  \ldots \\
 BS~16467-062 &     0.40 &  $<$0.45 & $-$0.11 &    0.18 & $-$0.74 &    0.46 &    0.33 &    0.26 &    0.50 &    0.36 & $-$0.41 & $-$0.70 & $-$3.71 &    0.63 &    0.26 & $-$1.58 &  \ldots \\
 BS~16082-129 &     0.29 &   \ldots &  \ldots &    0.14 & $-$0.76 &  \ldots &    0.25 &  \ldots &    0.14 &    0.35 &    0.02 & $-$0.71 & $-$2.87 &    0.01 &    0.17 & $-$0.16 &  \ldots \\
 HE~1347-1025 &     0.15 &   \ldots &    0.00 &    0.43 & $-$0.48 &    0.79 &    0.39 &    0.12 &  \ldots &    0.44 & $-$0.38 & $-$0.81 & $-$3.35 &    0.45 & $-$0.06 & $-$0.93 & $-$0.50 \\
 HE~1356-0622 & $<-$0.05 &   \ldots &    0.84 &    0.51 & $-$0.67 &    0.97 &    0.48 &    0.32 &    0.45 &    0.37 & $-$0.46 & $-$1.00 & $-$3.47 &    0.16 & $-$0.10 & $-$1.79 & $-$1.11 \\
 BS~16023-046 &     0.55 &   \ldots &  \ldots & $-$0.03 &  \ldots & $-$0.05 &    0.26 &    0.00 &    0.68 &    0.24 & $-$0.10 &  \ldots & $-$2.98 &    0.24 &    0.00 & $-$0.26 &  \ldots \\
    HD~122563 &  $-$0.44 &     0.70 &    0.39 &    0.28 & $-$0.26 &  \ldots &    0.18 &    0.39 &    0.18 &    0.36 & $-$0.30 & $-$0.24 & $-$2.58 &    0.02 &    0.14 &    0.25 &  \ldots \\
 BS~16550-087 &  $-$0.49 &     1.11 &    0.13 &    0.53 & $-$0.47 &    0.59 &    0.30 &    0.05 &    0.23 &    0.11 & $-$0.63 & $-$0.90 & $-$3.52 &    0.14 & $-$0.05 &    0.65 & $-$0.75 \\
 HE~1424-0241 &  $<$0.63 &  $<$1.13 &    0.30 &    0.43 & $-$0.73 & $-$0.89 & $-$0.50 & $-$0.01 &  \ldots & $-$0.04 & $-$0.32 & $-$0.23 & $-$3.81 &    0.89 &    0.32 &  \ldots & $-$0.75 \\
    HD~126587 &     0.19 &   \ldots &  \ldots &    0.40 & $-$0.54 &  \ldots &    0.42 &  \ldots &    0.32 &    0.40 &  \ldots & $-$0.66 & $-$3.01 &    0.06 &    0.03 &    0.34 &  \ldots \\
 HE~1429-0551 &     2.28 &     1.39 &    0.99 &    0.21 &  \ldots &  \ldots &    1.08 &  \ldots &    0.32 &    0.36 &  \ldots &  \ldots & $-$2.59 &  \ldots &  \ldots &  \ldots &    1.47 \\
 BS~16477-003 &     0.29 & $<-$0.26 &    0.21 &    0.24 & $-$0.53 &  \ldots &    0.34 &    0.15 &    0.37 &    0.32 & $-$0.40 &  \ldots & $-$3.32 &    0.25 &    0.08 &  \ldots &  \ldots \\
 CS~30325-094 &     0.00 &     0.18 &    0.20 &    0.42 & $-$0.54 &  \ldots &    0.40 &    0.40 &    0.35 &    0.32 & $-$0.44 &  \ldots & $-$3.39 &    0.18 &    0.07 &  \ldots &  \ldots \\
 BS~16968-061 &     0.45 &   \ldots &  \ldots &  \ldots &  \ldots &    0.33 &    0.13 &    0.40 &    0.59 &    0.19 & $-$0.23 &  \ldots & $-$2.93 &    0.56 &    0.16 &  \ldots &  \ldots \\
 CS~30325-028 &     0.38 &  $-$0.22 &  \ldots &    0.36 &  \ldots &  \ldots &    0.30 &    0.09 &    0.28 &    0.30 & $-$0.27 & $-$0.66 & $-$2.93 &    0.01 &    0.01 &    0.38 & $-$0.49 \\
 CS~30301-024 &     0.23 &   \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &  \ldots &    0.18 &  \ldots &  \ldots &  \ldots & $-$2.65 & $-$0.02 &  \ldots & $-$0.38 &  \ldots \\
 CS~30301-015 &     1.60 &     1.70 &  \ldots &    0.44 &  \ldots &  \ldots &  \ldots &  \ldots &    0.07 &    0.51 &  \ldots &  \ldots & $-$2.53 &  \ldots &  \ldots &  \ldots &  \ldots \\
 CS~30306-132 &     0.34 &   \ldots &  \ldots &    0.31 & $-$0.45 &  \ldots &    0.37 &  \ldots &    0.34 &    0.45 & $-$0.11 & $-$0.34 & $-$2.53 & $-$0.03 & $-$0.08 &    0.45 &  \ldots \\
 CS~30312-059 &     0.27 & $<-$0.48 &    0.35 &    0.28 & $-$0.78 &  \ldots &    0.37 & $-$0.01 &    0.29 &    0.33 & $-$0.42 & $-$0.83 & $-$3.31 &    0.11 & $-$0.02 &    0.14 & $-$0.14 \\
    HD~140283 &     0.28 &   \ldots &  \ldots &    0.07 & $-$0.92 &    0.39 &    0.21 &    0.14 &    0.27 &    0.31 & $-$0.19 & $-$0.56 & $-$2.53 &    0.17 &    0.23 & $-$0.10 & $-$0.94 \\
 CS~30312-100 &     0.54 &  $<$1.85 &    0.25 &    0.28 &  \ldots &  \ldots &    0.30 &  \ldots &    0.34 &    0.35 &    0.22 &  \ldots & $-$2.61 &  \ldots &  \ldots &  \ldots & $-$0.73 \\
 CS~22884-108 &  $<$0.92 &  $<$1.22 &  \ldots &  \ldots & $-$0.61 &    0.26 &    0.42 &    0.40 &  \ldots &    0.66 & $-$0.20 & $-$0.54 & $-$3.18 &  \ldots &    0.01 &    0.37 &    0.15 \\
 BS~16084-160 &  $-$0.12 &     0.78 & $-$0.08 &    0.17 & $-$0.81 &    0.87 &    0.24 & $-$0.04 &    0.03 &    0.03 & $-$0.44 & $-$0.78 & $-$3.24 & $-$0.03 & $-$0.11 & $-$2.06 & $-$2.06 \\
 CS~22872-102 &     0.60 &  $<$0.55 &    0.07 &    0.31 & $-$0.62 &    0.44 &    0.47 &    0.04 &    0.49 &    0.31 & $-$0.25 & $-$0.63 & $-$2.96 &    0.16 &    0.04 & $-$0.10 & $-$0.62 \\
 CS~22878-027 &     0.86 &  $<$1.06 & $-$0.17 & $-$0.11 &  \ldots &  \ldots &    0.07 &    0.02 &    0.39 &    0.30 &    0.02 & $-$0.34 & $-$2.52 &  \ldots &    0.09 & $-$0.26 &  \ldots \\
 BS~16080-054 &  $-$0.45 &     0.75 &    0.66 &    0.27 & $-$0.11 &    0.67 &    0.38 &    0.20 &    0.25 &    0.49 & $-$0.47 & $-$0.53 & $-$2.81 & $-$0.05 &    0.03 &    0.57 & $-$0.21 \\
 CS~22878-101 &  $-$0.29 &     1.33 &    0.33 &    0.53 & $-$0.73 &    0.56 &    0.34 &    0.27 &    0.36 &    0.40 & $-$0.45 & $-$0.92 & $-$3.17 &    0.16 & $-$0.16 & $-$0.18 & $-$0.64 \\
 BS~16080-093 & $<-$0.63 &   \ldots &  \ldots &    0.40 & $-$0.45 &    0.64 &    0.36 &    0.30 &    0.44 &    0.51 & $-$0.36 & $-$0.86 & $-$3.04 &    0.19 &    0.04 &    0.11 & $-$0.19 \\
      G 139-8 &   \ldots &   \ldots &  \ldots & $-$0.26 & $-$1.18 &    0.11 &    0.06 &    0.27 &    0.31 &    0.34 & $-$0.16 & $-$0.60 & $-$2.17 &  \ldots &  \ldots & $-$1.18 & $-$0.82 \\
   BD+17$^\circ$ 3248 &  $-$0.37 &     0.65 &    0.66 &    0.01 & $-$0.63 &  \ldots &    0.31 &    0.69 &    0.38 &    0.81 & $-$0.23 &  \ldots & $-$1.80 & $-$0.04 & $-$0.01 &  \ldots &  \ldots \\
   BD+23$^\circ$ 3130 &     0.11 &  $-$0.54 &    0.06 &    0.10 & $-$0.90 &  \ldots &    0.24 &    0.07 &    0.17 &    0.25 & $-$0.28 & $-$0.68 & $-$2.55 &    0.02 & $-$0.10 & $-$0.15 & $-$0.56 \\
 CS~22891-209 &  $-$0.65 &     1.12 &    0.68 &    0.33 & $-$0.36 &  \ldots &    0.29 &    0.22 &    0.30 &    0.35 & $-$0.41 &  \ldots & $-$3.24 &    0.08 &    0.06 &  \ldots &  \ldots \\
 CS~22896-154 &     0.23 &  $-$0.23 &    0.38 &    0.28 & $-$0.64 &  \ldots &    0.39 &    0.02 &    0.29 &    0.29 & $-$0.21 &  \ldots & $-$2.92 &    0.08 & $-$0.11 &  \ldots &  \ldots \\
    HD~186478 &  $-$0.28 &     0.62 &    0.40 &    0.41 & $-$0.39 &  \ldots &    0.47 &    0.25 &    0.29 &    0.35 & $-$0.29 & $-$0.51 & $-$2.70 & $-$0.10 & $-$0.22 &    0.16 &  \ldots \\
 CS~22873-055 &  $-$0.73 &     1.07 &    0.94 &    0.44 & $-$0.02 &  \ldots &    0.30 &    0.17 &    0.17 &    0.30 & $-$0.34 &  \ldots & $-$2.91 & $-$0.01 &    0.10 &  \ldots &  \ldots \\
   BD-18$^\circ$ 5550 &  $-$0.02 &  $-$0.36 &    0.24 &    0.42 & $-$0.33 &  \ldots &    0.41 &    0.13 &    0.16 &    0.19 & $-$0.36 &  \ldots & $-$3.22 & $-$0.06 &    0.00 &  \ldots &  \ldots \\
 CS~22873-166 &  $-$0.13 &     1.05 &    0.51 &    0.43 & $-$0.18 &  \ldots &    0.19 &    0.38 &    0.06 &    0.39 & $-$0.31 &  \ldots & $-$2.89 & $-$0.14 &    0.01 &  \ldots &  \ldots \\
 CS~22885-096 &     0.26 &     0.26 &    0.07 &    0.27 & $-$0.73 &  \ldots &    0.41 &    0.25 &    0.39 &    0.20 & $-$0.45 &  \ldots & $-$3.95 &    0.44 &    0.04 &  \ldots &  \ldots \\
 CS~22950-046 &   \ldots &   \ldots &  \ldots &    0.36 & $-$0.73 &    0.68 &    0.15 &    0.11 &    0.27 &    0.16 & $-$0.55 & $-$0.90 & $-$3.50 &  \ldots &  \ldots & $-$0.11 & $-$1.23 \\
    HD~196944 &     1.20 &     1.30 &  \ldots & $-$0.02 & $-$0.49 &  \ldots &    0.37 &  \ldots &    0.33 &    0.69 &    0.04 & $-$0.37 & $-$2.07 &    0.02 &  \ldots &  \ldots &  \ldots \\
 CS~22880-086 &     0.24 &   \ldots &  \ldots &    0.28 & $-$0.84 &  \ldots &    0.35 &  \ldots &    0.27 &    0.32 & $-$0.32 & $-$0.51 & $-$3.00 &    0.33 &    0.16 &    0.07 & $-$0.85 \\
 CS~22880-074 &     1.30 &  $-$0.10 &  \ldots & $-$0.10 & $-$1.00 &  \ldots &  \ldots &  \ldots &    0.14 &  \ldots & $-$0.19 &  \ldots & $-$2.23 &  \ldots &  \ldots &  \ldots &  \ldots \\
 SDSS 2047+00 &     2.00 &   \ldots &  \ldots &    0.20 &  \ldots &  \ldots &    0.43 &  \ldots &  \ldots &    0.45 & $-$0.02 &  \ldots & $-$2.38 &  \ldots &    0.17 &    1.03 &    1.70 \\
 CS~22897-008 &     0.56 &     0.24 & $-$0.01 &    0.34 & $-$0.70 &  \ldots &    0.26 & $-$0.04 &    0.29 &    0.19 & $-$0.37 &  \ldots & $-$3.51 &    0.29 &    0.14 &  \ldots &  \ldots \\
 CS~29498-043 &     1.90 &     2.30 &  \ldots &    1.52 &  \ldots &  \ldots &    0.00 &  \ldots &    0.11 &    0.12 & $-$0.23 &  \ldots & $-$3.60 &  \ldots &  \ldots &  \ldots &  \ldots \\
 CS~29506-007 &     0.49 &  $<$0.93 &  \ldots &    0.25 & $-$0.76 &    0.14 &    0.44 &    0.25 &    0.81 &    0.52 &    0.05 & $-$0.60 & $-$2.78 &    0.40 &    0.19 &    0.13 &    0.09 \\
 CS~29506-090 &     0.41 &   \ldots &  \ldots &    0.24 &  \ldots &    0.19 &    0.38 &    0.31 &    0.72 &    0.47 & $-$0.12 &  \ldots & $-$2.70 &    0.32 &    0.05 &    0.27 &  \ldots \\
 HE~2133-1426 &   \ldots &   \ldots &  \ldots &    0.28 & $-$0.61 &  \ldots &    0.33 &    0.26 &    0.60 &    0.40 & $-$0.10 & $-$0.47 & $-$2.81 &  \ldots &  \ldots & $-$0.14 & $-$0.42 \\
 CS~29495-041 &  $-$0.07 &     0.40 &    0.43 &    0.31 & $-$0.47 &  \ldots &    0.32 &    0.33 &    0.19 &    0.37 & $-$0.26 &  \ldots & $-$2.80 & $-$0.22 &    0.04 &  \ldots &  \ldots \\
 CS~22948-027 &     2.12 &     2.43 &    0.71 &    0.20 &  \ldots &  \ldots &    0.68 &  \ldots &    0.91 &    0.44 & $-$0.03 &  \ldots & $-$2.36 &  \ldots &  \ldots &  \ldots &    2.45 \\
 BS~17583-100 &     0.53 &   \ldots &  \ldots &    0.08 & $-$0.88 &  \ldots &    0.28 &  \ldots &    0.48 &    0.33 & $-$0.21 & $-$0.61 & $-$2.62 &    0.26 &    0.13 &    0.34 &  \ldots \\
 CS~22948-066 &     0.00 &     1.22 &    0.32 &    0.23 & $-$0.76 &  \ldots &    0.28 &    0.51 &    0.34 &    0.46 & $-$0.28 &  \ldots & $-$2.96 &    0.32 &    0.22 &  \ldots &  \ldots \\
 CS~22944-032 &     0.31 & $<-$0.44 &  \ldots &    0.34 & $-$0.77 &  \ldots &    0.35 &    0.10 &    0.36 &    0.31 & $-$0.33 & $-$0.62 & $-$3.01 &    0.29 &    0.17 & $-$0.13 & $-$0.76 \\
 CS~22948-093 &   \ldots &   \ldots &  \ldots &  \ldots &  \ldots &    0.51 &    0.39 &    0.13 &    0.87 &    0.22 & $-$0.08 &  \ldots & $-$3.13 &    0.77 &    0.30 & $-$0.09 &  \ldots \\
 CS~22956-050 &     0.27 &     0.31 &  \ldots &    0.36 & $-$0.61 &  \ldots &    0.45 &    0.00 &    0.40 &    0.32 & $-$0.39 &  \ldots & $-$3.37 &    0.24 &    0.01 &  \ldots &  \ldots \\
 HE~2158-0348 &     1.87 &     1.52 &  \ldots &    0.56 &    0.09 &  \ldots &    0.96 &  \ldots &    0.40 &    1.03 & $-$0.63 &    0.19 & $-$2.72 & $-$0.13 &  \ldots &    0.64 &    1.75 \\
 BS~17569-049 &  $-$0.12 &     0.86 &    0.59 &    0.19 & $-$0.31 &  \ldots &    0.32 &    0.28 &    0.24 &    0.38 & $-$0.20 &  \ldots & $-$2.85 & $-$0.12 &    0.08 &  \ldots &  \ldots \\
 CS~22965-054 &     0.62 &   \ldots &  \ldots &    0.36 & $-$0.52 &    0.08 &    0.38 &    0.16 &    0.52 &    0.31 & $-$0.22 & $-$0.33 & $-$2.95 &    0.26 & $-$0.02 &    0.27 &  \ldots \\
 HE~2209-1240 &   \ldots &   \ldots &  \ldots &    0.45 & $-$0.35 &    0.26 &    0.34 &    0.08 &  \ldots &    0.37 & $-$0.11 & $-$0.49 & $-$2.63 &    0.37 &    0.16 &    0.06 & $-$0.13 \\
 CS~22892-052 &     0.90 &     0.51 &    0.24 &    0.25 & $-$0.52 &  \ldots &    0.21 &    0.27 &    0.15 &    0.22 & $-$0.38 & $-$0.44 & $-$3.05 & $-$0.03 & $-$0.11 &    0.68 &  \ldots \\
 CS~22886-042 &     0.12 &  $<$2.03 &    0.31 &    0.26 &  \ldots &  \ldots &    0.32 &  \ldots &    0.25 &    0.23 & $-$0.19 &  \ldots & $-$2.79 &  \ldots &  \ldots &  \ldots & $-$0.32 \\
 CS~29502-042 &     0.16 &  $-$0.43 & $-$0.33 &    0.31 & $-$0.76 &  \ldots &    0.23 &    0.18 &    0.30 &    0.20 & $-$0.40 &  \ldots & $-$3.33 &    0.22 & $-$0.05 &  \ldots &  \ldots \\
 CS~29502-092 &     0.96 &     0.81 &  \ldots &    0.28 & $-$0.68 &  \ldots &    0.24 &    0.30 &    0.20 &    0.28 & $-$0.26 & $-$0.48 & $-$2.99 &    0.23 &    0.16 & $-$0.15 & $-$1.20 \\
 HE~2221-0453 &     1.83 &     0.84 &  \ldots &  \ldots &  \ldots &  \ldots &    0.74 &  \ldots &    0.44 &    0.34 &  \ldots &  \ldots & $-$2.00 &  \ldots &  \ldots &  \ldots &    1.76 \\
 CS~29516-024 &  $-$0.06 &  $-$0.76 &    0.57 &    0.56 & $-$0.44 &  \ldots &    0.50 &    0.21 &    0.30 &    0.31 & $-$0.26 &  \ldots & $-$3.12 & $-$0.05 & $-$0.09 &  \ldots &  \ldots \\
 HE~2228-0706 &     2.32 &     1.13 &  \ldots &    0.88 &  \ldots &  \ldots &    0.66 &  \ldots &    0.87 &    0.27 &    0.19 &  \ldots & $-$2.75 &  \ldots &  \ldots &  \ldots &    2.46 \\
 HE~2232-0603 &     1.22 &     0.47 &  \ldots &    0.33 & $-$0.30 &  \ldots &    0.39 &  \ldots &    0.39 &    0.35 & $-$0.22 & $-$0.62 & $-$1.94 & $-$0.04 & $-$0.33 &    0.59 &    1.50 \\
 CS~29491-053 &  $-$0.27 &     0.82 &    0.45 &    0.46 & $-$0.32 &  \ldots &    0.37 &    0.23 &    0.28 &    0.36 & $-$0.39 &  \ldots & $-$3.01 &    0.02 & $-$0.02 &  \ldots &  \ldots \\
 CD -24$^\circ$ 17504 &   \ldots &   \ldots &  \ldots &    0.16 & $-$0.61 &    0.13 &    0.28 &    0.26 &  \ldots &    0.28 & $-$0.07 & $-$0.22 & $-$3.45 &    0.52 &    0.31 &  \ldots &  \ldots \\
 CS~22888-031 &     0.38 &   \ldots &  \ldots &    0.34 &  \ldots &    0.36 &    0.44 &    0.42 &    0.78 &    0.62 & $-$0.05 &  \ldots & $-$3.28 &    0.53 &    0.20 & $-$0.14 &  \ldots \\
 CS~30338-089 &     2.06 &     1.27 &    0.61 &    0.19 &  \ldots &  \ldots &    0.60 &  \ldots &    0.40 &    0.66 &    0.11 &  \ldots & $-$2.76 &  \ldots &  \ldots &  \ldots &    2.30 \\
 HE~2323-0256 &     1.06 &     2.16 &    2.10 &    1.38 &    0.02 &  \ldots &    0.39 &    0.29 &    0.45 &    0.45 & $-$0.37 & $-$0.87 & $-$3.86 &    0.37 & $-$0.10 &    0.55 & $-$0.52 \\
 HE~2330-0555 &     2.09 &     1.00 &    0.81 &    0.34 &  \ldots &  \ldots &    0.45 &  \ldots &    0.35 &    0.29 & $-$0.03 &  \ldots & $-$3.01 &  \ldots &  \ldots &  \ldots &    1.17 \\
 CS~22966-011 &     0.45 &   \ldots &  \ldots &    0.21 &  \ldots &    0.13 &    0.49 &    0.47 &    0.72 &    0.73 & $-$0.01 &  \ldots & $-$3.12 &    0.55 &    0.20 &    0.67 &  \ldots \\
 CS~22952-015 &  $-$0.41 &     1.31 &  \ldots & $-$0.13 & $-$0.48 &  \ldots &    0.24 & $-$0.01 &    0.20 &    0.14 & $-$0.45 & $-$0.59 & $-$3.33 &    0.11 & $-$0.08 & $-$0.52 &  \ldots \\
 HE~2341-2029 &   \ldots &   \ldots &  \ldots &    0.31 & $-$0.72 &    0.33 &    0.39 &    0.38 &    0.72 &    0.49 & $-$0.14 & $-$0.55 & $-$2.48 &    0.58 & $-$0.08 &    0.00 & $-$0.43 \\
 CS~29522-046 &     0.42 &  $-$0.33 &  \ldots &    0.24 &  \ldots &  \ldots &    0.40 &    0.02 &    0.36 &    0.33 & $-$0.14 & $-$0.63 & $-$2.22 &    0.00 &    0.01 &    0.33 & $-$0.13 \\
 HE~2344-2800 &   \ldots &   \ldots &  \ldots &    0.04 & $-$0.73 &  \ldots &    0.21 &    0.04 &    0.76 &    0.68 &    0.27 &    0.12 & $-$2.67 &  \ldots &  \ldots & $-$0.08 & $-$0.37 \\
 CS~22966-057 &     0.06 &     0.10 &    0.61 & $-$0.02 & $-$0.72 &  \ldots &    0.22 &    0.27 &    0.28 &    0.43 & $-$0.05 &  \ldots & $-$2.50 &    0.14 &    0.24 &  \ldots &  \ldots \\
 CS~29499-060 &     0.38 &   \ldots &  \ldots & $-$0.01 &  \ldots &    0.05 & $-$0.06 &  \ldots &    0.33 &  \ldots &  \ldots &  \ldots & $-$2.66 &    0.19 & $-$0.21 & $-$0.63 &  \ldots \\
 HE~2356-0410 &     2.27 &     1.75 &  \ldots &    0.30 & $-$0.10 &  \ldots &    0.45 &  \ldots &    0.40 &    0.52 & $-$0.17 & $-$0.10 & $-$3.01 &    0.22 &  \ldots & $-$0.86 & $-$0.80 \\
\enddata

\tablenotetext{a}{For [C/Fe] and [N/Fe], the values are taken from the literature reference.} 

%\tablerefs{
%1 = \citet{aoki02};
%2 = \citet{aoki07};
%3 = \citet{aoki08};
%4 = \citet{bonifacio07,bonifacio09}; 
%5 = \citet{carretta02}; 
%6 = \citet{cayrel04,spite05}; 
%7 = \citet{cohen04}; 
%8 = \citet{cohen06}; 
%9 = \citet{cohen08}; 
%10 = \citet{honda04}; 
%11 = \citet{lai08}; 
%12 = \citet{norris01}
%}

\end{deluxetable}


==> tabA1.tex <==
\begin{deluxetable}{lrrrrrrrrrrrrrrrrrrrrrrrr}
\voffset=1.0in
\hoffset=-0.25in
\tablenum{A1}
\tablecolumns{27} 
\tablewidth{0pc} 
\rotate
\tabletypesize{\tiny}
\tablecaption{Model Atmosphere Parameters and Chemical Abundances, [X/Fe], for the Complete Sample 
(Including Literature Values for Sr and Ba) \label{tab:app}}
\tablehead{ 
\colhead{Star} & 
\colhead{RA2000\tablenotemark{a}} & 
\colhead{DEC2000\tablenotemark{a}} &
\colhead{\teff} & 
\colhead{$\log g$} & 
%\colhead{$\xi_t$} & 
%\colhead{[M/H]$_{\rm model}$} &
\colhead{[Fe/H]} &
\colhead{C-rich\tablenotemark{b}} &
\colhead{C\tablenotemark{c}} &
\colhead{N\tablenotemark{c}} &
\colhead{Na} &
\colhead{Mg} &
\colhead{Al} &
\colhead{Si} &
\colhead{Ca} &
\colhead{Sc} &
\colhead{\tii} &
\colhead{\tiii} &
\colhead{Cr} &
\colhead{Mn}&
\colhead{\feii} &
\colhead{Co} &
\colhead{Ni} &
\colhead{Sr} &
\colhead{Ba}&
\colhead{Source} \\ 
\colhead{} & 
\colhead{} & 
\colhead{} & 
\colhead{(K)} & 
\colhead{(cgs)} & 
%\colhead{(km s$^{-1}$)} & 
%\colhead{(dex)} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} \\
\colhead{(1)} &
\colhead{(2)} &
\colhead{(3)} &
\colhead{(4)} &
\colhead{(5)} &
\colhead{(6)} &
\colhead{(7)} &
\colhead{(8)} &
\colhead{(9)} & 
\colhead{(10)} &
\colhead{(11)} &
\colhead{(12)} &
\colhead{(13)} &
\colhead{(14)} &
\colhead{(15)} &
\colhead{(16)} &
\colhead{(17)} &
\colhead{(18)} &
\colhead{(19)} &
\colhead{(20)} &
\colhead{(21)} &
\colhead{(22)} &
\colhead{(23)} &
\colhead{(24)} &
\colhead{(25)}  
%\colhead{(26)} &
%\colhead{(27)} \\ 
%			SEE COMMENTS FOR DY BELOW
}
\startdata 
CS~22957-022                         &   00 01 45.5 &$-$05 49 46.6 & 5146 & 2.40 & $-$2.92 & 0 &     0.16 &     0.21 &   \ldots &     0.21 &   \ldots &   \ldots &     0.27 &     0.07 &     0.30 &     0.32 &  $-$0.31 &  $-$0.68 &  $-$2.87 &     0.11 &     0.02 &                   $-$0.19 &                   $-$1.09 &         14 \\
CS~29503-010                         &   00 04 55.4 &$-$24 24 19.3 & 6570 & 4.25 & $-$1.00 & 1 &     1.07 &  $<$1.28 &  $-$0.04 &  $-$0.06 &   \ldots &   \ldots &     0.11 &   \ldots &     0.28 &     0.21 &   \ldots &   \ldots &  $-$1.34 &   \ldots &   \ldots &                    \ldots &                      1.51 &          3 \\
CS~31085-024                         &   00 08 27.9 &  +10 54 19.8 & 5778 & 4.64 & $-$2.80 & 0 &     0.36 & $<-$0.24 &   \ldots &     0.08 &   \ldots &     0.39 &     0.28 &     0.33 &     0.33 &     0.50 &  $-$0.12 &  $-$0.60 &  $-$2.70 &     0.24 &     0.28 &                      0.04 &                   $-$0.57 &         14 \\
BS~17570-063                         &   00 20 36.2 &  +23 47 37.7 & 6233 & 4.46 & $-$2.95 & 0 &     0.40 &   \ldots &   \ldots &     0.28 &   \ldots &     0.51 &     0.33 &     0.77 &     0.60 &     0.70 &  $-$0.14 &   \ldots &  $-$3.01 &     0.44 &     0.20 &                   $-$0.02 &  $-$0.26\tablenotemark{f} &          5 \\
HE~0024-2523                         &   00 27 27.7 &$-$25 06 28.2 & 6635 & 4.11 & $-$2.82 & 0 &   \ldots &   \ldots &   \ldots &     0.82 &  $-$0.49 &   \ldots &     0.54 &     0.25 &     0.63 &     0.35 &  $-$0.38 &   \ldots &  $-$2.78 &   \ldots &   \ldots &                      0.46 &                      1.88 &          6 \\
CS~29527-015                         &   00 29 10.7 &$-$19 10 07.2 & 6577 & 3.89 & $-$3.32 & 1 &     1.18 &   \ldots &   \ldots &     0.50 &   \ldots &   \ldots &     0.58 &     0.46 &   \ldots &     0.53 &     0.05 &   \ldots &   \ldots &     0.65 &     0.22 &                      0.04 &                    \ldots &          5 \\
CS~30339-069                         &   00 30 16.0 &$-$35 56 51.2 & 6326 & 3.79 & $-$3.05 & 0 &     0.56 &   \ldots &   \ldots &     0.55 &   \ldots &   \ldots &     0.72 &     0.44 &   \ldots &     0.72 &     0.13 &   \ldots &  $-$3.08 &     0.53 &     0.32 &                      0.43 &                    \ldots &          5 \\
CS~31062-050                         &   00 30 31.1 &$-$12 05 10.9 & 5607 & 3.49 & $-$2.28 & 1 &     2.00 &     1.20 &   \ldots &     0.12 &  $-$0.45 &   \ldots &   \ldots &   \ldots &     0.34 &     0.67 &   \ldots &   \ldots &  $-$2.20 &   \ldots &   \ldots &     0.91\tablenotemark{f} &     2.30\tablenotemark{f} &          1 \\
HE~0028-2152                         &   00 31 07.7 &$-$21 36 07.3 & 6184 & 3.75 & $-$2.74 & 0 &   \ldots &   \ldots &   \ldots &     0.48 &  $-$0.63 &     0.30 &     0.47 &     0.22 &     0.64 &     0.47 &  $-$0.12 &  $-$0.65 &  $-$2.85 &     0.34 &     0.09 &                   $-$0.26 &                   $-$0.54 &          9 \\
HD~2796                              &   00 31 16.9 &$-$16 47 40.9 & 4923 & 1.84 & $-$2.31 & 0 &  $-$0.50 &     0.85 &     0.45 &     0.06 &  $-$0.51 &   \ldots &     0.23 &     0.43 &     0.12 &     0.50 &  $-$0.15 &   \ldots &  $-$2.19 &  $-$0.06 &     0.04 &     0.25\tablenotemark{f} &  $-$0.14\tablenotemark{f} &          7 \\
CS~31062-041                         &   00 35 03.0 &$-$15 54 29.3 & 4990 & 2.00 & $-$2.65 & 0 &     0.58 &  $<$1.59 &     0.40 &     0.32 &   \ldots &   \ldots &     0.34 &   \ldots &     0.29 &     0.30 &   \ldots &   \ldots &  $-$2.59 &   \ldots &   \ldots &                    \ldots &                   $-$0.42 &          3 \\
SDSS  0036-10                        &   00 36 02.2 &$-$10 43 36.3 & 6479 & 4.31 & $-$2.60 & 1 &     2.32 &   \ldots &     0.79 &     0.14 &   \ldots &   \ldots &     0.31 &   \ldots &   \ldots &     0.35 &  $-$0.09 &   \ldots &  $-$2.48 &     0.25 &  $-$0.07 &                   $-$0.07 &                      0.40 &          4 \\
CS~29497-034                         &   00 41 39.8 &$-$26 18 54.4 & 4983 & 1.96 & $-$3.00 & 1 &     2.72 &     2.63 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &     0.66 &     0.56 &  $-$0.11 &   \ldots &  $-$3.01 &   \ldots &   \ldots &                    \ldots &                      2.28 &          3 \\
CS~31062-012                         &   00 44 03.6 &$-$13 55 25.9 & 6190 & 4.47 & $-$2.67 & 1 &     2.12 &     1.20 &     1.18 &     0.20 &  $-$0.68 &   \ldots &     0.21 &   \ldots &     0.50 &     0.37 &  $-$0.17 &   \ldots &  $-$2.60 &     0.24 &     0.07 &                      0.33 &                      2.32 &      1,  4 \\
HD~4306                              &   00 45 27.2 &$-$09 32 39.9 & 4854 & 1.61 & $-$3.04 & 0 &     0.11 &   \ldots &   \ldots &     0.47 &  $-$0.44 &   \ldots &     0.51 &   \ldots &     0.42 &     0.51 &  $-$0.09 &  $-$0.68 &  $-$3.00 &     0.12 &     0.02 &                      0.04 &  $-$1.17\tablenotemark{f} &         13 \\
CD -38$^\circ$ 245                   &   00 46 36.2 &$-$37 39 33.5 & 4857 & 1.54 & $-$4.15 & 0 & $<-$0.33 &     1.07 &     0.03 &     0.17 &  $-$0.65 &   \ldots &     0.22 &     0.10 &     0.44 &     0.29 &  $-$0.40 &   \ldots &  $-$4.11 &     0.35 &  $-$0.14 &  $-$0.71\tablenotemark{f} &  $-$0.76\tablenotemark{f} &          7 \\
HE~0049-3948                         &   00 52 13.4 &$-$39 32 36.9 & 6466 & 3.78 & $-$3.68 & 0 &  $<$1.81 &  $<$2.40 &  $-$0.08 &     0.29 &   \ldots &  $-$0.01 &     0.11 &   \ldots &   \ldots &     0.40 &     0.23 &   \ldots &  $-$3.51 &   \ldots &     0.30 &                   $-$0.85 &                   $<$0.14 & This Paper \\
HE~0054-2123                         &   00 56 53.2 &$-$21 07 29.6 & 6424 & 4.35 & $-$2.59 & 0 &   \ldots &   \ldots &   \ldots &     0.34 &  $-$0.61 &     0.27 &     0.42 &     0.39 &     0.62 &     0.59 &  $-$0.06 &  $-$0.81 &  $-$2.60 &     0.23 &     0.17 &                   $-$0.10 &                   $-$0.27 &          9 \\
HE~0057-5959                         &   00 59 54.0 &$-$59 43 29.9 & 5257 & 2.65 & $-$4.08 & 1 &     0.86 &     2.15 &     1.98 &     0.51 &   \ldots &   \ldots &     0.65 &     0.17 &     0.68 &     0.40 &  $-$0.50 &   \ldots &   \ldots &   \ldots &     0.17 &                   $-$1.06 &                   $-$0.46 & This Paper \\
CS~22953-003                         &   01 02 15.9 &$-$61 43 45.8 & 5002 & 2.01 & $-$2.93 & 0 &     0.30 &     0.12 &     0.32 &     0.20 &  $-$0.91 &   \ldots &     0.24 &     0.07 &     0.19 &     0.15 &  $-$0.41 &   \ldots &  $-$2.90 &     0.02 &  $-$0.03 &     0.22\tablenotemark{f} &     0.49\tablenotemark{f} &          7 \\
HD~6268                              &   01 03 18.2 &$-$27 52 49.9 & 4696 & 1.23 & $-$2.74 & 0 &  $-$0.67 &   \ldots &   \ldots &     0.30 &  $-$0.46 &   \ldots &     0.39 &   \ldots &     0.29 &     0.45 &   \ldots &  $-$0.53 &  $-$2.62 &  $-$0.01 &  $-$0.15 &                      0.25 &  $-$0.04\tablenotemark{f} &         13 \\
HE~0102-0633                         &   01 05 25.7 &$-$06 17 35.4 & 6371 & 3.83 & $-$2.90 & 0 &   \ldots &   \ldots &   \ldots &     0.44 &  $-$0.65 &     0.29 &     0.53 &     0.19 &   \ldots &     0.26 &  $-$0.20 &  $-$0.63 &  $-$2.84 &     0.45 &     0.19 &                   $-$0.39 &                   $-$0.08 &          9 \\
HE~0102-1213                         &   01 05 28.0 &$-$11 57 31.1 & 6100 & 3.65 & $-$3.28 & 0 &  $<$1.31 &   \ldots &  $-$0.02 &     0.06 &  $-$0.69 &     0.16 &     0.42 &     0.10 &     0.76 &     0.35 &  $-$0.13 &  $-$0.66 &  $-$3.03 &     0.64 &     0.09 &                   $-$0.30 &                  $<-$0.64 & This Paper \\
HE~0105-2202                         &   01 07 31.2 &$-$21 46 06.5 & 6267 & 4.44 & $-$2.75 & 0 &   \ldots &   \ldots &   \ldots &     0.29 &  $-$0.78 &     0.39 &     0.31 &     0.20 &     0.78 &     0.49 &  $-$0.18 &  $-$0.69 &  $-$2.52 &     0.50 &  $-$0.12 &                   $-$0.15 &                   $-$0.27 &          9 \\
CS~22183-031                         &   01 09 05.1 &$-$04 43 21.1 & 5202 & 2.54 & $-$3.17 & 0 &     0.42 &   \ldots &   \ldots &     0.25 &  $-$0.49 &   \ldots &     0.32 &   \ldots &     0.63 &     0.41 &   \ldots &  $-$0.70 &  $-$3.13 &     0.24 &     0.15 &                      0.26 &  $-$0.33\tablenotemark{f} &         13 \\
HE~0107-5240                         &   01 09 29.2 &$-$52 24 34.2 & 5100 & 2.20 & $-$5.54 & 1 &     3.85 &     2.43 &     1.11 &     0.26 &   \ldots &   \ldots &     0.12 &   \ldots &   \ldots &     0.04 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots & $<-$0.52\tablenotemark{f} & $<$+0.82\tablenotemark{f} &          8 \\
CS~29518-020                         &   01 12 13.2 &$-$31 00 05.3 & 6435 & 4.34 & $-$2.65 & 0 &   \ldots &   \ldots &   \ldots &     0.00 &   \ldots &   \ldots &     0.26 &   \ldots &   \ldots &   \ldots &  $-$0.28 &   \ldots &   \ldots &   \ldots &  $-$0.08 &   \ldots\tablenotemark{f} &                    \ldots &          5 \\
CS~22174-007                         &   01 14 06.5 &$-$11 02 35.4 & 5265 & 2.78 & $-$2.39 & 0 &     0.41 &  $<$1.42 &     0.26 &     0.19 &   \ldots &   \ldots &     0.30 &   \ldots &     0.39 &     0.38 &  $-$0.09 &   \ldots &  $-$2.34 &   \ldots &   \ldots &                    \ldots &                   $-$0.14 &          3 \\
CS~29518-043                         &   01 18 38.3 &$-$30 41 02.7 & 6550 & 4.29 & $-$3.14 & 0 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &     0.80 &   \ldots &   \ldots &     0.77 &   \ldots &   \ldots &  $-$3.03 &   \ldots &     0.63 &     0.08\tablenotemark{f} &                    \ldots &          5 \\
CS~29518-051                         &   01 24 10.0 &$-$28 15 21.1 & 5100 & 2.29 & $-$2.64 & 0 &  $-$0.13 &     0.82 &     0.48 &     0.16 &  $-$0.70 &   \ldots &     0.30 &     0.23 &     0.26 &     0.45 &  $-$0.20 &   \ldots &  $-$2.75 &     0.03 &     0.13 &     0.18\tablenotemark{f} &  $-$0.45\tablenotemark{f} &          7 \\
CS~22953-037                         &   01 25 06.6 &$-$59 16 00.7 & 6627 & 4.11 & $-$2.70 & 0 &     0.37 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &  $-$0.18 &   \ldots &     0.75 &  $-$0.04 &  $-$0.61 &   \ldots &  $-$2.80 &   \ldots &  $-$0.37 &                   $-$0.50 &                    \ldots &          5 \\
CS~31082-001                         &   01 29 31.1 &$-$16 00 45.5 & 4866 & 1.66 & $-$2.75 & 0 &     0.16 &  $-$0.51 &     0.46 &     0.29 &  $-$0.57 &   \ldots &     0.31 &     0.18 &     0.44 &     0.38 &  $-$0.31 &  $-$0.48 &  $-$2.76 &     0.02 &     0.18 &                      0.63 &     1.02\tablenotemark{f} &      7, 13 \\
HE~0130-2303                         &   01 33 18.2 &$-$22 48 36.8 & 6548 & 4.28 & $-$3.02 & 0 &   \ldots &   \ldots &   \ldots &     0.12 &  $-$0.78 &  $-$0.07 &     0.39 &     0.28 &   \ldots &     0.50 &  $-$0.06 &  $-$0.50 &   \ldots &   \ldots &   \ldots &                      0.09 &                   $-$0.71 &          6 \\
HE~0132-2439                         &   01 34 58.9 &$-$24 24 18.6 & 5249 & 2.63 & $-$3.79 & 0 &     0.62 &     1.07 &     0.07 &     0.32 &  $-$0.61 &     0.66 &     0.36 &     1.05 &     0.70 &     0.50 &  $-$0.36 &  $-$0.86 &  $-$3.62 &     0.44 &     0.06 &                      0.30 &                   $-$0.88 &      6, 11 \\
53327-2044-515 \tablenotemark{d}     &   01 40 36.2 &  +23 44 58.1 & 5703 & 4.68 & $-$4.00 & 1 &     1.13 &   \ldots &     0.11 &     0.32 &  $-$0.19 &   \ldots &     0.17 &     0.32 &   \ldots &     0.50 &   \ldots &   \ldots &   \ldots &   \ldots &     0.13 &                      1.09 &                   $<$0.34 & This Paper \\
53327-2044-515\tablenotemark{e}      &   01 40 36.2 &  +23 44 58.1 & 5703 & 3.36 & $-$4.09 & 1 &     1.57 &   \ldots &     0.17 &     0.48 &  $-$0.16 &   \ldots &     0.20 &  $-$0.07 &   \ldots &     0.04 &   \ldots &   \ldots &   \ldots &   \ldots &     0.12 &                      0.53 &                  $<-$0.04 & This Paper \\
HE~0142+0147                         &   01 44 47.9 &  +02 02 17.9 & 6244 & 3.79 & $-$2.67 & 0 &   \ldots &   \ldots &   \ldots &     0.54 &  $-$0.55 &     0.45 &     0.46 &   \ldots &     0.67 &     0.37 &  $-$0.26 &  $-$0.51 &  $-$2.63 &     0.54 &     0.20 &                   $-$0.09 &                   $-$0.32 &          9 \\
HE~0143-0441                         &   01 45 37.9 &$-$04 26 43.4 & 6276 & 3.84 & $-$2.32 & 1 &     1.82 &     0.85 &   \ldots &     0.65 &  $-$0.64 &   \ldots &   \ldots &   \ldots &     0.57 &     0.42 &  $-$0.30 &  $-$0.82 &  $-$2.44 &     0.47 &  $-$0.18 &                      1.09 &                      2.42 &      9, 10 \\
HE~0146-1548                         &   01 48 34.7 &$-$15 33 24.4 & 4636 & 0.99 & $-$3.46 & 1 &     0.84 &   \ldots &     1.17 &     0.87 &     0.14 &     0.50 &     0.22 &   \ldots &     0.17 &     0.18 &  $-$0.38 &  $-$0.59 &  $-$3.33 &     0.30 &     0.05 &                   $-$0.38 &                   $-$0.71 & This Paper \\
HE~0148-2611                         &   01 50 59.6 &$-$25 57 03.2 & 6605 & 4.23 & $-$3.05 & 0 &   \ldots &   \ldots &   \ldots &  $-$0.02 &  $-$0.89 &   \ldots &     0.15 &     0.21 &   \ldots &     0.14 &  $-$0.21 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.97 &                    \ldots &          6 \\
HE~0206-1916                         &   02 09 19.6 &$-$19 01 55.5 & 5073 & 2.23 & $-$2.52 & 1 &     2.10 &     1.61 &     0.73 &     0.40 &   \ldots &   \ldots &     0.41 &   \ldots &     0.55 &     0.50 &     0.07 &   \ldots &  $-$2.39 &   \ldots &   \ldots &                    \ldots &                      1.99 &          3 \\
HE~0207-1423                         &   02 10 00.7 &$-$14 09 11.1 & 5023 & 2.07 & $-$2.95 & 1 &     2.38 &   \ldots &     0.61 &     0.54 &     0.10 &     0.50 &     0.43 &   \ldots &     0.22 &     0.31 &     0.09 &   \ldots &  $-$2.87 &  $-$0.07 &     0.21 &                      0.33 &                      1.73 & This Paper \\
HE~0218-2738                         &   02 21 03.9 &$-$27 24 40.5 & 6593 & 4.29 & $-$3.57 & 0 &   \ldots &   \ldots &   \ldots &     0.05 &  $-$0.59 &     0.05 &     0.11 &     0.54 &   \ldots &     0.57 &  $-$0.10 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.38 &                    \ldots &          6 \\
HE~0228-4047\tablenotemark{d}        &   02 30 33.7 &$-$40 33 54.8 & 6515 & 4.35 & $-$3.75 & 0 &  $<$1.88 &   \ldots &   \ldots &     0.26 &   \ldots &     0.35 &     0.39 &   \ldots &   \ldots &     0.57 &  $-$0.01 &   \ldots &   \ldots &   \ldots &     0.49 &                  $<-$0.58 &                   $<$0.40 & This Paper \\
HE~0228-4047\tablenotemark{e}        &   02 30 33.7 &$-$40 33 54.8 & 6515 & 3.80 & $-$3.75 & 0 &  $<$1.98 &   \ldots &   \ldots &     0.26 &   \ldots &     0.34 &     0.39 &   \ldots &   \ldots &     0.38 &     0.00 &   \ldots &   \ldots &   \ldots &     0.49 &                  $<-$0.75 &                   $<$0.24 & This Paper \\
HE~0231-6025                         &   02 32 30.6 &$-$60 12 11.2 & 6437 & 4.36 & $-$3.10 & 0 &  $<$1.64 &   \ldots &     0.01 &     0.39 &  $-$0.64 &     0.02 &     0.42 &     0.27 &   \ldots &     0.65 &  $-$0.02 &   \ldots &   \ldots &   \ldots &   \ldots &                      0.04 &                   $-$0.10 & This Paper \\
CS~31061-032                         &   02 38 43.3 &  +03 19 02.4 & 6448 & 4.33 & $-$2.56 & 0 &     0.56 &   \ldots &   \ldots &  $-$0.15 &   \ldots &   \ldots &     0.00 &  $-$0.11 &     0.28 &     0.09 &   \ldots &   \ldots &  $-$2.56 &  $-$0.10 &  $-$0.34 &     0.21\tablenotemark{f} &  $-$0.40\tablenotemark{f} &          5 \\
CS~22189-009                         &   02 41 42.4 &$-$13 28 10.5 & 4944 & 1.83 & $-$3.48 & 0 &     0.31 &     0.27 &  $-$0.19 &     0.09 &  $-$0.90 &   \ldots &     0.20 &     0.08 &     0.17 &     0.12 &  $-$0.44 &   \ldots &  $-$3.46 &     0.29 &     0.09 &  $-$0.95\tablenotemark{f} &  $-$1.29\tablenotemark{f} &          7 \\
HE~0242-0732                         &   02 45 00.7 &$-$07 19 42.1 & 6572 & 4.29 & $-$3.30 & 0 &   \ldots &   \ldots &   \ldots &     0.33 &  $-$0.69 &     0.29 &     0.29 &     0.24 &   \ldots &     0.20 &  $-$0.14 &   \ldots &  $-$3.48 &   \ldots &   \ldots &                   $-$1.20 &                    \ldots &          6 \\
HE~0253-1331                         &   02 56 06.7 &$-$13 19 27.0 & 6474 & 4.34 & $-$3.01 & 0 &  $<$1.64 &   \ldots &  $-$0.17 &     0.25 &  $-$0.61 &     0.07 &     0.58 &     0.58 &   \ldots &     0.62 &  $-$0.08 &   \ldots &   \ldots &     0.44 &     0.13 &                      0.41 &                      0.33 & This Paper \\
CS~22963-004                         &   02 56 46.6 &$-$04 51 17.5 & 5597 & 3.34 & $-$3.54 & 0 &     0.40 &     0.80 &   \ldots &     0.34 &  $-$0.73 &     0.58 &     0.38 &     0.35 &   \ldots &     0.44 &  $-$0.30 &  $-$0.83 &  $-$3.44 &     0.47 &     0.11 &                   $-$0.68 &                   $-$0.51 &         14 \\
CS~31078-018                         &   03 01 00.7 &  +06 16 31.9 & 5100 & 2.27 & $-$2.99 & 0 &     0.37 &  $-$0.38 &   \ldots &     0.47 &  $-$0.78 &   \ldots &     0.48 &     0.03 &     0.30 &     0.26 &  $-$0.27 &  $-$0.37 &  $-$3.05 &     0.13 &     0.13 &     0.24\tablenotemark{f} &                      0.38 &         14 \\
LP 831-70                            &   03 06 05.4 &$-$22 19 17.9 & 6408 & 4.37 & $-$2.95 & 0 &   \ldots &   \ldots &   \ldots &     0.49 &  $-$0.41 &     0.24 &     0.10 &     0.44 &   \ldots &     0.30 &  $-$0.22 &  $-$0.62 &  $-$2.93 &     0.65 &     0.03 &                   $-$1.48 &  $-$1.55\tablenotemark{f} &          9 \\
CS~22968-014                         &   03 06 29.5 &$-$54 30 32.5 & 4864 & 1.60 & $-$3.58 & 0 &     0.25 &     0.24 &  $-$0.24 &     0.21 &  $-$0.72 &   \ldots &     0.02 &     0.08 &     0.14 &     0.02 &  $-$0.46 &   \ldots &  $-$3.56 &     0.47 &     0.27 &  $-$1.80\tablenotemark{f} &  $-$1.77\tablenotemark{f} &          7 \\
CS~22172-002                         &   03 14 20.8 &$-$10 35 11.3 & 4893 & 1.68 & $-$3.77 & 0 &     0.00 &     0.24 &  $-$0.28 &     0.15 &  $-$0.80 &   \ldots &     0.24 &     0.00 &     0.37 &     0.26 &  $-$0.44 &   \ldots &  $-$3.73 &     0.41 &  $-$0.10 &  $-$1.31\tablenotemark{f} &  $-$1.17\tablenotemark{f} &          7 \\
HE~0314-1739                         &   03 17 01.8 &$-$17 28 54.9 & 6570 & 4.25 & $-$2.86 & 0 &  $<$1.49 &   \ldots &  $-$0.45 &     0.04 &  $-$0.86 &  $-$0.10 &     0.49 &     0.15 &   \ldots &     0.36 &  $-$0.18 &   \ldots &   \ldots &   \ldots &  $-$0.07 &                   $-$0.57 &                  $<-$0.27 & This Paper \\
HE~0336+0113                         &   03 38 52.9 &  +01 23 07.8 & 5819 & 3.59 & $-$2.60 & 1 &     2.25 &     1.60 &   \ldots &     1.03 &     0.13 &   \ldots &     0.42 &   \ldots &     0.46 &     0.13 &  $-$0.18 &  $-$0.20 &   \ldots &     0.13 &   \ldots &                      1.87 &                      2.69 &         10 \\
% DY COMMENTS 0355 updated by hand
HE~0355-3728\tablenotemark{d}        &   03 56 36.5 &$-$44 34 03.4 & 6418 & 4.39 & $-$3.41 & 0 &  $<$2.14 &   \ldots &   \ldots &   \ldots &   \ldots &     0.10 &     0.28 &   \ldots &   \ldots &     0.89 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &                      0.45 &                   $<$0.21 & This Paper \\
HE~0355-3728\tablenotemark{e}        &   03 56 36.5 &$-$44 34 03.4 & 6418 & 3.84 & $-$3.41 & 0 &  $<$2.34 &   \ldots &   \ldots &   \ldots &   \ldots &     0.20 &     0.74 &   \ldots &   \ldots &     0.95 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &                      0.92 &                   $<$0.09 & This Paper \\
HE~0400-2030                         &   04 02 14.8 &$-$20 21 53.5 & 5579 & 3.53 & $-$1.68 & 1 &     1.14 &     2.75 &     0.45 &     0.28 &   \ldots &   \ldots &     0.12 &   \ldots &     0.17 &     0.43 &     0.11 &   \ldots &  $-$1.80 &   \ldots &   \ldots &                    \ldots &                      1.85 &          3 \\
CS~22177-009                         &   04 07 40.6 &$-$25 02 43.9 & 6423 & 4.37 & $-$2.98 & 0 &     0.38 &   \ldots &   \ldots &     0.24 &   \ldots &     0.10 &     0.42 &     0.27 &   \ldots &     0.47 &  $-$0.07 &   \ldots &  $-$2.96 &     0.47 &     0.08 &                   $-$0.18 &                    \ldots &          5 \\
CS~22169-035                         &   04 12 13.9 &$-$12 05 05.1 & 4654 & 1.10 & $-$2.95 & 0 &  $-$0.24 &     1.02 &   \ldots &  $-$0.04 &  $-$0.89 &   \ldots &     0.13 &  $-$0.08 &  $-$0.07 &  $-$0.09 &  $-$0.46 &  $-$0.36 &  $-$2.91 &  $-$0.33 &  $-$0.27 &                   $-$0.59 &  $-$1.19\tablenotemark{f} &      7, 13 \\
CS~22186-025                         &   04 24 32.8 &$-$37 09 02.6 & 4871 & 1.66 & $-$3.07 & 0 &  $-$0.54 &     0.98 &     0.48 &     0.32 &  $-$0.72 &   \ldots &     0.36 &     0.28 &     0.36 &     0.50 &  $-$0.36 &   \ldots &  $-$2.91 &     0.09 &     0.00 &  $-$0.12\tablenotemark{f} &     0.02\tablenotemark{f} &          7 \\
HE~0441-0652                         &   04 43 29.9 &$-$06 46 53.5 & 4811 & 1.52 & $-$2.77 & 1 &     1.38 &     0.89 &     0.65 &     0.21 &   \ldots &   \ldots &     0.38 &   \ldots &     0.37 &     0.32 &   \ldots &   \ldots &  $-$2.75 &   \ldots &   \ldots &                    \ldots &                      1.20 &          3 \\
BD~+03$^\circ$ 740                   &   05 01 16.6 &  +04 06 37.1 & 6485 & 4.31 & $-$2.70 & 0 &     0.59 &  $<$0.29 &   \ldots &     0.15 &  $-$0.83 &     0.17 &     0.39 &     0.37 &     0.69 &     0.60 &  $-$0.07 &  $-$0.51 &  $-$2.61 &     0.35 &     0.06 &                   $-$0.08 &                   $-$0.42 &      6, 14 \\
HE~0507-1653                         &   05 09 16.6 &$-$16 50 04.6 & 4935 & 1.88 & $-$1.32 & 1 &     1.29 &     0.80 &     0.20 &     0.10 &   \ldots &   \ldots &     0.53 &   \ldots &     0.40 &     0.02 &   \ldots &   \ldots &  $-$1.76 &   \ldots &   \ldots &                    \ldots &                      1.56 &          3 \\
HE~0508-1555                         &   05 10 35.5 &$-$15 51 38.3 & 6451 & 4.32 & $-$2.40 & 0 &   \ldots &   \ldots &   \ldots &     0.34 &  $-$0.65 &     0.31 &     0.30 &     0.28 &     0.67 &     0.54 &  $-$0.21 &  $-$0.65 &  $-$2.50 &     0.30 &     0.09 &                      0.48 &                   $-$0.13 &          9 \\
HE~0557-4840                         &   05 58 39.3 &$-$48 39 56.8 & 4900 & 2.20 & $-$4.81 & 1 &     1.65 &  $<$1.93 &  $-$0.18 &     0.17 &  $-$0.65 &   \ldots &     0.17 &   \ldots &   \ldots &     0.36 &  $-$0.69 &   \ldots &   \ldots &   \ldots &  $-$0.17 & $<-$1.07\tablenotemark{f} & $<$+0.03\tablenotemark{f} &         16 \\
54142-2667-094                       &   08 51 36.7 &  +10 18 03.2 & 6456 & 3.87 & $-$2.96 & 0 &  $<$1.39 &   \ldots &   \ldots &     0.23 &  $-$0.72 &  $-$0.05 &     0.34 &     0.30 &     1.03 &     0.39 &  $-$0.14 &  $-$0.38 &  $-$2.90 &   \ldots &  $-$0.16 &                   $-$1.08 &                  $<-$0.43 & This Paper \\
52972-1213-507                       &   09 18 49.9 &  +37 44 26.8 & 6463 & 4.34 & $-$2.98 & 1 &     2.82 &   \ldots &     1.60 &     0.34 &   \ldots &  $<$1.50 &     0.56 &   \ldots &   \ldots &     0.38 &  $-$0.27 &   \ldots &   \ldots &     0.65 &     0.15 &                      1.15 &                      1.70 & This Paper \\
SDSS  0924+40                        &   09 24 01.9 &  +40 59 28.8 & 6196 & 3.77 & $-$2.68 & 1 &     2.72 &   \ldots &     1.29 &     0.39 &   \ldots &   \ldots &     0.22 &   \ldots &   \ldots &     0.21 &  $-$0.21 &   \ldots &  $-$2.67 &   \ldots &     0.15 &                      0.77 &                      1.73 &          4 \\
HE~0945-1435\tablenotemark{d}        &   09 47 50.7 &$-$14 49 06.9 & 6344 & 4.43 & $-$3.77 & 0 &  $<$1.70 &   \ldots &   \ldots &  $-$0.10 &   \ldots &  $<$2.00 &     0.26 &     0.15 &   \ldots &     0.33 &  $-$0.24 &   \ldots &   \ldots &   \ldots &   \ldots &                  $<-$0.71 &                   $<$0.25 & This Paper \\
HE~0945-1435\tablenotemark{e}        &   09 47 50.7 &$-$14 49 06.9 & 6344 & 3.71 & $-$3.78 & 0 &  $<$1.81 &   \ldots &   \ldots &  $-$0.09 &   \ldots &  $<$2.00 &     0.26 &  $-$0.08 &   \ldots &     0.09 &  $-$0.23 &   \ldots &   \ldots &   \ldots &   \ldots &                  $<-$0.93 &                   $<$0.04 & This Paper \\
HE~1005-1439                         &   10 07 52.4 &$-$14 54 21.0 & 5202 & 2.55 & $-$3.09 & 1 &     2.48 &     1.79 &     1.05 &     0.33 &   \ldots &   \ldots &     0.54 &   \ldots &     0.49 &     0.31 &  $-$0.34 &   \ldots &   \ldots &   \ldots &   \ldots &                    \ldots &                      1.17 &          3 \\
HD~88609                             &   10 14 29.0 &  +53 33 39.4 & 4541 & 0.80 & $-$2.98 & 0 &  $-$0.51 &   \ldots &   \ldots &     0.28 &  $-$0.42 &   \ldots &     0.25 &   \ldots &     0.18 &     0.51 &  $-$0.30 &  $-$0.79 &  $-$3.07 &  $-$0.31 &  $-$0.07 &                      0.17 &  $-$1.05\tablenotemark{f} &         13 \\
HE~1012-1540                         &   10 14 53.5 &$-$15 55 53.2 & 5745 & 3.45 & $-$3.47 & 1 &     2.22 &     1.25 &     1.93 &     1.85 &     0.65 &   \ldots &     0.70 &   \ldots &   \ldots &     0.06 &  $-$0.24 &  $-$0.51 &   \ldots &     0.23 &  $-$0.22 &                   $-$0.37 &                   $-$0.25 &         11 \\
BS~16469-075                         &   10 15 10.2 &  +42 53 17.3 & 4919 & 1.78 & $-$3.25 & 0 &     0.21 &   \ldots &   \ldots &     0.24 &  $-$0.74 &   \ldots &     0.33 &   \ldots &     0.27 &     0.27 &   \ldots &  $-$0.77 &  $-$3.19 &     0.18 &  $-$0.05 &                      0.25 &  $-$1.12\tablenotemark{f} &         13 \\
HE~1031-0020                         &   10 34 24.2 &$-$00 36 08.4 & 5043 & 2.13 & $-$2.79 & 1 &     1.63 &     2.48 &   \ldots &     0.48 &     0.66 &   \ldots &     0.96 &   \ldots &     0.33 &     1.13 &  $-$0.30 &     0.00 &  $-$3.02 &   \ldots &   \ldots &                      0.52 &                      1.61 &         10 \\
HE~1055+0104\tablenotemark{d}        &   10 58 04.4 &  +00 48 36.0 & 6287 & 4.43 & $-$2.87 & 0 &  $<$1.20 &   \ldots &  $-$0.07 &     0.21 &  $-$0.66 &     0.46 &     0.40 &     0.24 &   \ldots &     0.54 &  $-$0.23 &  $-$0.63 &  $-$2.96 &     0.40 &     0.13 &                   $-$0.11 &                  $<-$0.39 & This Paper \\
HE~1055+0104\tablenotemark{e}        &   10 58 04.4 &  +00 48 36.0 & 6287 & 3.79 & $-$2.89 & 0 &  $<$1.42 &   \ldots &  $-$0.06 &     0.35 &  $-$0.67 &     0.50 &     0.44 &     0.04 &   \ldots &     0.32 &  $-$0.23 &  $-$0.62 &  $-$3.19 &     0.41 &     0.11 &                   $-$0.37 &                  $<-$0.57 & This Paper \\
HE~1116-0054\tablenotemark{d}        &   11 18 47.8 &$-$01 11 19.4 & 6454 & 4.37 & $-$3.49 & 0 &  $<$1.72 &  $<$2.91 &  $-$0.23 &     0.07 &   \ldots &  $<$1.70 &     0.30 &     0.28 &   \ldots &     0.40 &  $-$0.07 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.07 &                   $<$0.16 & This Paper \\
HE~1116-0054\tablenotemark{e}        &   11 18 47.8 &$-$01 11 19.4 & 6454 & 3.80 & $-$3.48 & 0 &  $<$1.92 &  $<$2.91 &  $-$0.23 &     0.08 &   \ldots &  $<$1.70 &     0.30 &     0.09 &   \ldots &     0.21 &  $-$0.07 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.25 &                  $<-$0.01 & This Paper \\
BS~16545-089                         &   11 24 27.5 &  +36 50 28.8 & 6486 & 3.82 & $-$3.44 & 0 &  $<$1.77 &   \ldots &  $-$0.16 &     0.25 &   \ldots &  $<$1.50 &     0.53 &     0.17 &   \ldots &     0.45 &  $-$0.12 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.18 &                  $<-$0.18 & This Paper \\
53436-1996-093                       &   11 28 13.6 &  +38 41 48.9 & 6449 & 4.38 & $-$3.53 & 0 &  $<$1.66 &   \ldots &  $-$0.13 &     0.21 &   \ldots &  $<$1.80 &     0.30 &     0.44 &   \ldots &     0.45 &     0.05 &   \ldots &   \ldots &   \ldots &   \ldots &                      0.44 &                   $<$0.05 & This Paper \\
BS~16077-007                         &   11 35 18.0 &  +31 00 23.7 & 6486 & 4.31 & $-$2.77 & 0 &     0.60 &  $<$0.80 &   \ldots &     0.28 &   \ldots &     0.23 &     0.49 &     0.30 &     0.67 &     0.52 &  $-$0.12 &  $-$0.58 &  $-$2.78 &     0.30 &     0.10 &                      0.26 &                   $-$0.23 &         14 \\
HE~1142-1422                         &   11 44 59.2 &$-$14 38 49.6 & 6238 & 2.80 & $-$2.84 & 0 &  $<$1.57 &  $<$2.51 &  $-$0.06 &     0.40 &  $-$0.57 &  $-$0.12 &     0.40 &     0.22 &   \ldots &     0.52 &     0.01 &  $-$0.42 &  $-$2.64 &   \ldots &     0.12 &                      0.48 &                      0.44 & This Paper \\
HE~1150-0428                         &   11 53 06.6 &$-$04 45 03.4 & 5208 & 2.54 & $-$3.47 & 1 &     2.37 &     2.52 &   \ldots &     0.41 &   \ldots &   \ldots &     1.16 &   \ldots &     0.59 &     0.73 &  $-$0.56 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.12 &                   $-$0.48 &         10 \\
HE~1201-1512\tablenotemark{d}        &   12 03 37.0 &$-$15 29 33.0 & 5725 & 4.67 & $-$3.86 & 1 &     1.14 &  $<$1.23 &  $-$0.35 &     0.20 &  $-$0.73 &   \ldots &     0.05 &     0.31 &   \ldots &     0.33 &  $-$0.50 &  $-$0.59 &   \ldots &     0.83 &     0.19 &                  $<-$0.87 &                   $<$0.05 & This Paper \\
HE~1201-1512\tablenotemark{e}        &   12 03 37.0 &$-$15 29 33.0 & 5725 & 3.39 & $-$3.92 & 1 &     1.60 &  $<$1.29 &  $-$0.32 &     0.28 &  $-$0.72 &   \ldots &     0.07 &  $-$0.09 &   \ldots &  $-$0.10 &  $-$0.48 &  $-$0.58 &   \ldots &     0.82 &     0.15 &                  $<-$1.27 &                  $<-$0.34 & This Paper \\
HE~1204-0744                         &   12 06 46.2 &$-$08 00 44.1 & 6500 & 4.30 & $-$2.71 & 0 &  $<$1.55 &   \ldots &  $-$0.05 &  $-$0.07 &   \ldots &  $-$0.34 &     0.45 &  $-$0.09 &   \ldots &     0.18 &     0.04 &   \ldots &  $-$1.76 &   \ldots &  $-$0.18 &                   $-$0.30 &                  $<-$0.18 & This Paper \\
BS~16920-017                         &   12 07 16.8 &  +41 39 32.5 & 4851 & 1.58 & $-$3.40 & 0 & $<-$0.07 &   \ldots &   \ldots &     0.11 &  $-$0.70 &   \ldots &     0.16 &   \ldots &     0.55 &     0.57 &  $-$0.13 &  $-$0.23 &  $-$3.18 &     0.19 &     0.21 &                   $-$0.36 &  $-$1.83\tablenotemark{f} &         13 \\
HE~1207-3108                         &   12 09 54.0 &$-$31 25 10.6 & 5294 & 2.85 & $-$2.70 & 0 & $<-$0.27 &     0.42 &     0.54 &  $-$0.38 &  $-$1.19 &     0.16 &  $-$0.25 &  $-$0.55 &  $-$0.29 &  $-$0.31 &  $-$0.41 &  $-$0.35 &  $-$2.62 &  $-$0.31 &  $-$0.33 &                   $-$0.38 &                  $<-$1.67 & This Paper \\
BS~16928-053                         &   12 22 28.0 &  +34 11 31.8 & 4679 & 1.16 & $-$2.93 & 0 &  $-$0.24 &     1.05 &     0.17 &     0.09 &  $-$0.79 &   \ldots &     0.18 &   \ldots &     0.00 &     0.23 &  $-$0.14 &  $-$0.74 &  $-$2.99 &  $-$0.20 &  $-$0.16 &                   $-$0.04 &                   $-$0.79 &     13, 14 \\
BS~16085-050                         &   12 37 46.7 &  +19 22 49.5 & 4910 & 1.76 & $-$3.16 & 0 & $<-$0.52 &   \ldots &   \ldots &     0.56 &  $-$0.46 &   \ldots &     0.44 &   \ldots &     0.27 &     0.36 &  $-$0.38 &  $-$0.37 &  $-$3.03 &     0.12 &     0.20 &                   $-$1.57 &  $-$1.56\tablenotemark{f} &         13 \\
BS~16076-006                         &   12 48 22.8 &  +20 56 44.0 & 5566 & 3.32 & $-$3.51 & 0 &     0.34 &   \ldots &   \ldots &     0.44 &   \ldots &     0.31 &     0.72 &     0.38 &     0.73 &     0.63 &  $-$0.09 &   \ldots &  $-$3.58 &     0.38 &     0.07 &                    \ldots & $<-$1.00\tablenotemark{f} &          5 \\
HE~1300+0157                         &   13 02 56.2 &  +01 41 52.1 & 5529 & 3.25 & $-$3.75 & 1 &     1.31 &  $<$0.71 &  $-$0.02 &     0.33 &  $-$0.64 &   \ldots &     0.39 &     0.30 &     0.62 &     0.36 &  $-$0.38 &  $-$0.76 &  $-$3.78 &     0.49 &     0.08 &                   $-$1.36 & $<-$0.85\tablenotemark{f} &     11, 12 \\
BS~16929-005                         &   13 03 29.5 &  +33 51 09.1 & 5229 & 2.61 & $-$3.34 & 1 &     0.99 &     0.32 &     0.03 &     0.30 &  $-$0.72 &   \ldots &     0.34 &     0.01 &     0.52 &     0.40 &  $-$0.35 &  $-$0.78 &  $-$3.27 &     0.28 &     0.07 &                      0.54 &                   $-$0.41 &  3, 13, 14 \\
HD~115444                            &   13 16 42.5 &  +36 22 52.9 & 4711 & 1.23 & $-$2.65 & 0 &  $-$0.41 &   \ldots &   \ldots &     0.05 &  $-$0.31 &   \ldots &     0.22 &   \ldots &     0.17 &     0.68 &     0.13 &  $-$0.70 &  $-$2.88 &  $-$0.09 &     0.28 &                      0.26 &     0.14\tablenotemark{f} &         13 \\
HE~1320+0038                         &   13 22 35.4 &  +00 22 32.6 & 6566 & 3.99 & $-$2.68 & 0 &   \ldots &   \ldots &   \ldots &     0.36 &  $-$0.60 &     0.05 &     0.34 &     0.17 &   \ldots &     0.43 &  $-$0.11 &  $-$0.50 &  $-$2.61 &     0.44 &     0.06 &                   $-$0.46 &                   $-$0.41 &          9 \\
HE~1319-1935                         &   13 22 38.7 &$-$19 51 11.6 & 4691 & 1.27 & $-$2.22 & 1 &     1.45 &     0.46 &   \ldots &     0.36 &   \ldots &   \ldots &     0.61 &   \ldots &   \ldots &     0.32 &   \ldots &   \ldots &  $-$2.12 &   \ldots &   \ldots &                    \ldots &                      1.68 &          3 \\
HE~1320-2952                         &   13 22 54.9 &$-$30 08 05.3 & 5106 & 2.26 & $-$3.69 & 0 &  $<$0.52 &  $<$0.86 &     0.09 &     0.40 &  $-$0.60 &     0.68 &     0.31 &     0.00 &     0.54 &     0.22 &  $-$0.34 &  $-$0.78 &  $-$3.62 &     0.29 &  $-$0.15 &                   $-$0.37 &                   $-$0.96 & This Paper \\
HE~1327-2326                         &   13 30 06.0 &$-$23 41 49.7 & 6180 & 3.70 & $-$5.76 & 1 &     4.26 &     4.56 &     2.48 &     1.55 &     1.23 &   \ldots &     0.29 &   \ldots &   \ldots &     0.80 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &                      1.04 &                    \ldots &          2 \\
BS~16467-062                         &   13 42 00.6 &  +17 48 40.9 & 5310 & 2.80 & $-$3.80 & 0 &     0.40 &  $<$0.45 &  $-$0.11 &     0.18 &  $-$0.74 &     0.46 &     0.33 &     0.26 &     0.50 &     0.36 &  $-$0.41 &  $-$0.70 &  $-$3.71 &     0.63 &     0.26 &                   $-$1.58 &                    \ldots &  7, 11, 14 \\
BS~16082-129                         &   13 47 11.7 &  +28 57 47.1 & 4868 & 1.67 & $-$2.84 & 0 &     0.29 &   \ldots &   \ldots &     0.14 &  $-$0.76 &   \ldots &     0.25 &   \ldots &     0.14 &     0.35 &     0.02 &  $-$0.71 &  $-$2.87 &     0.01 &     0.17 &                   $-$0.16 &  $-$0.97\tablenotemark{f} &         13 \\
HE~1346-0427\tablenotemark{d}        &   13 49 25.1 &$-$04 42 14.8 & 6255 & 4.47 & $-$3.57 & 0 &  $<$1.10 &   \ldots &  $-$0.15 &     0.25 &   \ldots &  $<$1.80 &     0.37 &     0.21 &     0.80 &     0.36 &  $-$0.22 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.23 &                   $<$0.01 & This Paper \\
HE~1346-0427\tablenotemark{e}        &   13 49 25.1 &$-$04 42 14.8 & 6255 & 3.69 & $-$3.58 & 0 &  $<$1.31 &   \ldots &  $-$0.14 &     0.28 &   \ldots &  $<$1.80 &     0.37 &  $-$0.04 &     0.80 &     0.11 &  $-$0.21 &   \ldots &   \ldots &   \ldots &   \ldots &                   $-$0.48 &                  $<-$0.22 & This Paper \\
HE~1347-1025                         &   13 50 22.4 &$-$10 40 18.9 & 5206 & 2.52 & $-$3.71 & 0 &     0.15 &   \ldots &     0.00 &     0.43 &  $-$0.48 &     0.79 &     0.39 &     0.12 &   \ldots &     0.44 &  $-$0.38 &  $-$0.81 &  $-$3.35 &     0.45 &  $-$0.06 &                   $-$0.93 &                   $-$0.50 &         11 \\
HE~1356-0622                         &   13 59 30.3 &$-$06 36 35.0 & 4953 & 1.85 & $-$3.63 & 0 & $<-$0.05 &   \ldots &     0.84 &     0.51 &  $-$0.67 &     0.97 &     0.48 &     0.32 &     0.45 &     0.37 &  $-$0.46 &  $-$1.00 &  $-$3.47 &     0.16 &  $-$0.10 &                   $-$1.79 &                   $-$1.11 &         11 \\
BS~16023-046                         &   14 00 54.5 &  +22 46 42.3 & 6571 & 4.25 & $-$2.83 & 0 &     0.55 &   \ldots &   \ldots &  $-$0.03 &   \ldots &  $-$0.05 &     0.26 &     0.00 &     0.68 &     0.24 &  $-$0.10 &   \ldots &  $-$2.98 &     0.24 &     0.00 &                   $-$0.26 &                    \ldots &          5 \\
HD~122563                            &   14 02 31.9 &  +09 41 10.1 & 4843 & 1.62 & $-$2.54 & 0 &  $-$0.44 &     0.70 &     0.39 &     0.28 &  $-$0.26 &   \ldots &     0.18 &     0.39 &     0.18 &     0.36 &  $-$0.30 &  $-$0.24 &  $-$2.58 &     0.02 &     0.14 &                      0.25 &  $-$1.12\tablenotemark{f} &      7, 13 \\
HE~1402-0523\tablenotemark{d}        &   14 04 38.0 &$-$05 38 13.5 & 6418 & 4.38 & $-$3.17 & 0 &  $<$1.50 &  $<$1.84 &  $-$0.15 &     0.29 &  $-$0.79 &     0.10 &     0.35 &     0.44 &   \ldots &     0.57 &  $-$0.16 &   \ldots &   \ldots &     0.99 &     0.03 &                      0.11 &                  $<-$0.09 & This Paper \\
HE~1402-0523\tablenotemark{e}        &   14 04 38.0 &$-$05 38 13.5 & 6418 & 3.82 & $-$3.19 & 0 &  $<$1.62 &  $<$1.96 &  $-$0.13 &     0.36 &  $-$0.77 &     0.09 &     0.38 &     0.27 &   \ldots &     0.39 &  $-$0.14 &   \ldots &   \ldots &     1.01 &     0.04 &                   $-$0.09 &                  $<-$0.24 & This Paper \\
BS~16550-087                         &   14 10 26.7 &  +18 01 24.0 & 4754 & 1.32 & $-$3.54 & 0 &  $-$0.49 &     1.11 &     0.13 &     0.53 &  $-$0.47 &     0.59 &     0.30 &     0.05 &     0.23 &     0.11 &  $-$0.63 &  $-$0.90 &  $-$3.52 &     0.14 &  $-$0.05 &                      0.65 &                   $-$0.75 &         14 \\
HE~1424-0241                         &   14 26 40.3 &$-$02 54 27.5 & 5260 & 2.66 & $-$4.05 & 0 &  $<$0.63 &  $<$1.13 &     0.30 &     0.43 &  $-$0.73 &  $-$0.89 &  $-$0.50 &  $-$0.01 &   \ldots &  $-$0.04 &  $-$0.32 &  $-$0.23 &  $-$3.81 &     0.89 &     0.32 & $<-$1.69\tablenotemark{f} &                   $-$0.75 &         11 \\
HD~126587                            &   14 27 00.4 &$-$22 14 38.9 & 4853 & 1.61 & $-$3.00 & 0 &     0.19 &   \ldots &   \ldots &     0.40 &  $-$0.54 &   \ldots &     0.42 &   \ldots &     0.32 &     0.40 &   \ldots &  $-$0.66 &  $-$3.01 &     0.06 &     0.03 &                      0.34 &  $-$0.10\tablenotemark{f} &         13 \\
HE~1429-0551                         &   14 32 31.3 &$-$06 05 00.3 & 4757 & 1.39 & $-$2.60 & 1 &     2.28 &     1.39 &     0.99 &     0.21 &   \ldots &   \ldots &     1.08 &   \ldots &     0.32 &     0.36 &   \ldots &   \ldots &  $-$2.59 &   \ldots &   \ldots &                    \ldots &                      1.47 &          3 \\
BS~16477-003                         &   14 32 56.9 &  +06 46 07.0 & 4879 & 1.66 & $-$3.39 & 0 &     0.29 & $<-$0.26 &     0.21 &     0.24 &  $-$0.53 &   \ldots &     0.34 &     0.15 &     0.37 &     0.32 &  $-$0.40 &   \ldots &  $-$3.32 &     0.25 &     0.08 &     0.01\tablenotemark{f} &  $-$0.45\tablenotemark{f} &          7 \\
CS~30325-094                         &   14 54 39.3 &  +04 21 38.1 & 4948 & 1.85 & $-$3.35 & 0 &     0.00 &     0.18 &     0.20 &     0.42 &  $-$0.54 &   \ldots &     0.40 &     0.40 &     0.35 &     0.32 &  $-$0.44 &   \ldots &  $-$3.39 &     0.18 &     0.07 &  $-$2.24\tablenotemark{f} &  $-$1.88\tablenotemark{f} &          7 \\
BS~16968-061                         &   15 01 06.1 &  +03 42 45.5 & 6343 & 3.82 & $-$2.85 & 0 &     0.45 &   \ldots &   \ldots &   \ldots &   \ldots &     0.33 &     0.13 &     0.40 &     0.59 &     0.19 &  $-$0.23 &   \ldots &  $-$2.93 &     0.56 &     0.16 &  $-$0.57\tablenotemark{f} &                    \ldots &          5 \\
CS~30325-028                         &   15 05 19.8 &  +06 17 07.0 & 4894 & 1.73 & $-$2.87 & 0 &     0.38 &  $-$0.22 &   \ldots &     0.36 &   \ldots &   \ldots &     0.30 &     0.09 &     0.28 &     0.30 &  $-$0.27 &  $-$0.66 &  $-$2.93 &     0.01 &     0.01 &                      0.38 &                   $-$0.49 &         14 \\
CS~30301-024                         &   15 08 29.7 &$-$00 35 59.2 & 6584 & 4.03 & $-$2.54 & 0 &     0.23 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &     0.18 &   \ldots &   \ldots &   \ldots &  $-$2.65 &  $-$0.02 &   \ldots &                   $-$0.38 &  $-$0.28\tablenotemark{f} &          5 \\
CS~30301-015                         &   15 08 56.8 &  +02 30 18.5 & 4889 & 1.73 & $-$2.73 & 1 &     1.60 &     1.70 &   \ldots &     0.44 &   \ldots &   \ldots &   \ldots &   \ldots &     0.07 &     0.51 &   \ldots &   \ldots &  $-$2.53 &   \ldots &   \ldots &     0.30\tablenotemark{f} &     1.45\tablenotemark{f} &          1 \\
HE~1506-0113                         &   15 09 14.3 &$-$01 24 56.6 & 5016 & 2.01 & $-$3.54 & 1 &     1.47 &     0.61 &     1.65 &     0.89 &  $-$0.53 &     0.50 &     0.19 &   \ldots &     0.53 &     0.44 &  $-$0.15 &  $-$0.32 &  $-$3.49 &     0.48 &     0.38 &                   $-$0.85 &                   $-$0.80 & This Paper \\
CS~30306-132                         &   15 14 18.9 &  +07 27 02.8 & 5047 & 2.16 & $-$2.56 & 0 &     0.34 &   \ldots &   \ldots &     0.31 &  $-$0.45 &   \ldots &     0.37 &   \ldots &     0.34 &     0.45 &  $-$0.11 &  $-$0.34 &  $-$2.53 &  $-$0.03 &  $-$0.08 &                      0.45 &     0.22\tablenotemark{f} &         13 \\
CS~30312-059                         &   15 34 48.8 &$-$01 23 37.3 & 4908 & 1.75 & $-$3.22 & 0 &     0.27 & $<-$0.48 &     0.35 &     0.28 &  $-$0.78 &   \ldots &     0.37 &  $-$0.01 &     0.29 &     0.33 &  $-$0.42 &  $-$0.83 &  $-$3.31 &     0.11 &  $-$0.02 &                      0.14 &                   $-$0.14 &         14 \\
HD~140283                            &   15 43 03.1 &$-$10 56 01.0 & 5711 & 3.53 & $-$2.56 & 0 &     0.28 &   \ldots &   \ldots &     0.07 &  $-$0.92 &     0.39 &     0.21 &     0.14 &     0.27 &     0.31 &  $-$0.19 &  $-$0.56 &  $-$2.53 &     0.17 &     0.23 &                   $-$0.10 &                   $-$0.94 &      6, 13 \\
CS~30312-100                         &   15 43 31.7 &  +02 01 17.4 & 5117 & 2.34 & $-$2.66 & 0 &     0.54 &  $<$1.85 &     0.25 &     0.28 &   \ldots &   \ldots &     0.30 &   \ldots &     0.34 &     0.35 &     0.22 &   \ldots &  $-$2.61 &   \ldots &   \ldots &                    \ldots &                   $-$0.73 &          3 \\
CS~22884-108                         &   15 49 57.6 &$-$09 14 09.2 & 6107 & 4.52 & $-$3.30 & 0 &  $<$0.92 &  $<$1.22 &   \ldots &   \ldots &  $-$0.61 &     0.26 &     0.42 &     0.40 &   \ldots &     0.66 &  $-$0.20 &  $-$0.54 &  $-$3.18 &   \ldots &     0.01 &                      0.37 &                      0.15 &         14 \\
BS~16084-160                         &   16 28 50.8 &  +54 37 06.8 & 4727 & 1.27 & $-$3.20 & 0 &  $-$0.12 &     0.78 &  $-$0.08 &     0.17 &  $-$0.81 &     0.87 &     0.24 &  $-$0.04 &     0.03 &     0.03 &  $-$0.44 &  $-$0.78 &  $-$3.24 &  $-$0.03 &  $-$0.11 &                   $-$2.06 &                   $-$2.06 &         14 \\
CS~22872-102                         &   16 29 20.7 &$-$03 04 56.6 & 5911 & 3.60 & $-$2.94 & 0 &     0.60 &  $<$0.55 &     0.07 &     0.31 &  $-$0.62 &     0.44 &     0.47 &     0.04 &     0.49 &     0.31 &  $-$0.25 &  $-$0.63 &  $-$2.96 &     0.16 &     0.04 &                   $-$0.10 &                   $-$0.62 &         14 \\
CS~22878-027                         &   16 37 35.9 &  +10 22 07.8 & 6319 & 4.41 & $-$2.51 & 1 &     0.86 &  $<$1.06 &  $-$0.17 &  $-$0.11 &   \ldots &   \ldots &     0.07 &     0.02 &     0.39 &     0.30 &     0.02 &  $-$0.34 &  $-$2.52 &   \ldots &     0.09 &                   $-$0.26 & $<-$0.75\tablenotemark{f} &         14 \\
BS~16080-054                         &   16 39 18.5 &  +60 57 42.6 & 4902 & 1.75 & $-$2.94 & 0 &  $-$0.45 &     0.75 &     0.66 &     0.27 &  $-$0.11 &     0.67 &     0.38 &     0.20 &     0.25 &     0.49 &  $-$0.47 &  $-$0.53 &  $-$2.81 &  $-$0.05 &     0.03 &                      0.57 &                   $-$0.21 &         14 \\
CS~22878-101                         &   16 45 31.4 &  +08 14 45.5 & 4796 & 1.44 & $-$3.31 & 0 &  $-$0.29 &     1.33 &     0.33 &     0.53 &  $-$0.73 &     0.56 &     0.34 &     0.27 &     0.36 &     0.40 &  $-$0.45 &  $-$0.92 &  $-$3.17 &     0.16 &  $-$0.16 &                   $-$0.18 &                   $-$0.64 &      6,  7 \\
BS~16080-093                         &   16 50 38.3 &  +59 13 06.5 & 4945 & 1.85 & $-$3.23 & 0 & $<-$0.63 &   \ldots &   \ldots &     0.40 &  $-$0.45 &     0.64 &     0.36 &     0.30 &     0.44 &     0.51 &  $-$0.36 &  $-$0.86 &  $-$3.04 &     0.19 &     0.04 &                      0.11 &                   $-$0.19 &         14 \\
G 139-8                              &   17 01 44.0 &  +16 09 03.6 & 6266 & 4.42 & $-$2.03 & 0 &   \ldots &   \ldots &   \ldots &  $-$0.26 &  $-$1.18 &     0.11 &     0.06 &     0.27 &     0.31 &     0.34 &  $-$0.16 &  $-$0.60 &  $-$2.17 &   \ldots &   \ldots &                   $-$1.18 &                   $-$0.82 &          6 \\
BD~+17$^\circ$ 3248                  &   17 28 14.5 &  +17 30 35.9 & 5240 & 2.72 & $-$2.17 & 0 &  $-$0.37 &     0.65 &     0.66 &     0.01 &  $-$0.63 &   \ldots &     0.31 &     0.69 &     0.38 &     0.81 &  $-$0.23 &   \ldots &  $-$1.80 &  $-$0.04 &  $-$0.01 &     0.05\tablenotemark{f} &     0.69\tablenotemark{f} &          7 \\
BD~+23$^\circ$ 3130                  &   17 32 41.6 &  +23 44 11.7 & 5262 & 2.76 & $-$2.52 & 0 &     0.11 &  $-$0.54 &     0.06 &     0.10 &  $-$0.90 &   \ldots &     0.24 &     0.07 &     0.17 &     0.25 &  $-$0.28 &  $-$0.68 &  $-$2.55 &     0.02 &  $-$0.10 &                   $-$0.15 &                   $-$0.56 &         14 \\
CS~22891-209                         &   19 42 02.2 &$-$61 03 44.7 & 4699 & 1.18 & $-$3.32 & 0 &  $-$0.65 &     1.12 &     0.68 &     0.33 &  $-$0.36 &   \ldots &     0.29 &     0.22 &     0.30 &     0.35 &  $-$0.41 &   \ldots &  $-$3.24 &     0.08 &     0.06 &     0.08\tablenotemark{f} &  $-$0.55\tablenotemark{f} &          7 \\
CS~22896-154                         &   19 42 26.9 &$-$56 58 34.0 & 5100 & 2.28 & $-$2.85 & 0 &     0.23 &  $-$0.23 &     0.38 &     0.28 &  $-$0.64 &   \ldots &     0.39 &     0.02 &     0.29 &     0.29 &  $-$0.21 &   \ldots &  $-$2.92 &     0.08 &  $-$0.11 &     0.54\tablenotemark{f} &     0.51\tablenotemark{f} &          7 \\
HD~186478                            &   19 45 14.1 &$-$17 29 26.9 & 4629 & 1.07 & $-$2.68 & 0 &  $-$0.28 &     0.62 &     0.40 &     0.41 &  $-$0.39 &   \ldots &     0.47 &     0.25 &     0.29 &     0.35 &  $-$0.29 &  $-$0.51 &  $-$2.70 &  $-$0.10 &  $-$0.22 &                      0.16 &  $-$0.04\tablenotemark{f} &      7, 13 \\
CS~22873-055                         &   19 53 49.8 &$-$59 40 00.2 & 4551 & 0.82 & $-$2.99 & 0 &  $-$0.73 &     1.07 &     0.94 &     0.44 &  $-$0.02 &   \ldots &     0.30 &     0.17 &     0.17 &     0.30 &  $-$0.34 &   \ldots &  $-$2.91 &  $-$0.01 &     0.10 &  $-$0.48\tablenotemark{f} &  $-$0.45\tablenotemark{f} &          7 \\
BD~-18$^\circ$ 5550                  &   19 58 49.7 &$-$18 12 10.9 & 4558 & 0.81 & $-$3.20 & 1 &  $-$0.02 &  $-$0.36 &     0.24 &     0.42 &  $-$0.33 &   \ldots &     0.41 &     0.13 &     0.16 &     0.19 &  $-$0.36 &   \ldots &  $-$3.22 &  $-$0.06 &     0.00 &  $-$1.01\tablenotemark{f} &  $-$0.74\tablenotemark{f} &          7 \\
CS~22873-166                         &   20 19 22.0 &$-$61 30 14.9 & 4516 & 0.77 & $-$2.74 & 1 &  $-$0.13 &     1.05 &     0.51 &     0.43 &  $-$0.18 &   \ldots &     0.19 &     0.38 &     0.06 &     0.39 &  $-$0.31 &   \ldots &  $-$2.89 &  $-$0.14 &     0.01 &     0.13\tablenotemark{f} &  $-$0.70\tablenotemark{f} &          7 \\
CS~22885-096                         &   20 20 51.2 &$-$39 53 30.2 & 4992 & 1.93 & $-$3.86 & 0 &     0.26 &     0.26 &     0.07 &     0.27 &  $-$0.73 &   \ldots &     0.41 &     0.25 &     0.39 &     0.20 &  $-$0.45 &   \ldots &  $-$3.95 &     0.44 &     0.04 &  $-$1.39\tablenotemark{f} &  $-$1.10\tablenotemark{f} &          7 \\
CS~22950-046                         &   20 21 28.4 &$-$13 16 33.6 & 4769 & 1.37 & $-$3.39 & 0 &   \ldots &   \ldots &   \ldots &     0.36 &  $-$0.73 &     0.68 &     0.15 &     0.11 &     0.27 &     0.16 &  $-$0.55 &  $-$0.90 &  $-$3.50 &   \ldots &   \ldots &                   $-$0.11 &                   $-$1.23 &          6 \\
HE~2020-5228                         &   20 24 17.1 &$-$52 19 02.3 & 6305 & 3.79 & $-$2.93 & 0 &  $<$1.66 &  $<$2.30 &   \ldots &     0.22 &   \ldots &     0.10 &     0.44 &     0.25 &   \ldots &     0.25 &  $-$0.23 &   \ldots &  $-$2.81 &     0.69 &  $-$0.04 &                   $-$0.20 &                  $<-$0.33 & This Paper \\
HE~2032-5633                         &   20 36 24.9 &$-$56 23 05.8 & 6457 & 3.78 & $-$3.63 & 0 &  $<$2.36 &  $<$2.60 &     0.00 &     0.29 &  $-$0.51 &     0.33 &     0.61 &   \ldots &   \ldots &     0.39 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &                  $<-$0.68 &                   $<$0.31 & This Paper \\
HD~196944                            &   20 40 46.1 &$-$06 47 50.6 & 5255 & 2.74 & $-$2.44 & 1 &     1.20 &     1.30 &   \ldots &  $-$0.02 &  $-$0.49 &   \ldots &     0.37 &   \ldots &     0.33 &     0.69 &     0.04 &  $-$0.37 &  $-$2.07 &     0.02 &   \ldots &     0.84\tablenotemark{f} &     1.10\tablenotemark{f} &          1 \\
CS~30336-049                         &   20 45 23.5 &$-$28 42 35.9 & 4725 & 1.19 & $-$4.10 & 0 &  $<$0.23 &     0.97 &  $-$0.01 &     0.15 &  $-$0.77 &     0.43 &     0.22 &  $-$0.03 &     0.17 &     0.02 &  $-$0.48 &  $-$0.91 &  $-$4.10 &     0.38 &     0.10 &                   $-$1.63 &                  $<-$1.55 & This Paper \\
CS~22880-086                         &   20 45 47.5 &$-$18 33 32.4 & 5196 & 2.54 & $-$3.05 & 0 &     0.24 &   \ldots &   \ldots &     0.28 &  $-$0.84 &   \ldots &     0.35 &   \ldots &     0.27 &     0.32 &  $-$0.32 &  $-$0.51 &  $-$3.00 &     0.33 &     0.16 &                      0.07 &                   $-$0.85 &         14 \\
CS~22880-074                         &   20 46 03.2 &$-$20 59 14.2 & 5621 & 3.50 & $-$2.29 & 1 &     1.30 &  $-$0.10 &   \ldots &  $-$0.10 &  $-$1.00 &   \ldots &   \ldots &   \ldots &     0.14 &   \ldots &  $-$0.19 &   \ldots &  $-$2.23 &   \ldots &   \ldots &     0.39\tablenotemark{f} &     1.31\tablenotemark{f} &          1 \\
SDSS  2047+00                        &   20 47 28.8 &  +00 15 53.8 & 6383 & 4.36 & $-$2.36 & 1 &     2.00 &   \ldots &   \ldots &     0.20 &   \ldots &   \ldots &     0.43 &   \ldots &   \ldots &     0.45 &  $-$0.02 &   \ldots &  $-$2.38 &   \ldots &     0.17 &                      1.03 &                      1.70 &          4 \\
HE~2047-5612                         &   20 51 22.1 &$-$56 00 52.9 & 6128 & 3.68 & $-$3.14 & 0 &  $<$1.37 &  $<$1.91 &  $-$0.26 &  $-$0.02 &  $-$0.89 &     0.05 &     0.16 &     0.18 &   \ldots &     0.24 &     0.02 &  $-$0.61 &  $-$3.13 &   \ldots &     0.28 &                  $<-$1.36 &                  $<-$0.39 & This Paper \\
CS~22897-008                         &   21 03 11.9 &$-$65 05 08.8 & 4795 & 1.43 & $-$3.50 & 1 &     0.56 &     0.24 &  $-$0.01 &     0.34 &  $-$0.70 &   \ldots &     0.26 &  $-$0.04 &     0.29 &     0.19 &  $-$0.37 &   \ldots &  $-$3.51 &     0.29 &     0.14 &     0.44\tablenotemark{f} &  $-$1.00\tablenotemark{f} &          7 \\
CS~29498-043                         &   21 03 52.1 &$-$29 42 50.2 & 4639 & 1.00 & $-$3.49 & 1 &     1.90 &     2.30 &   \ldots &     1.52 &   \ldots &   \ldots &     0.00 &   \ldots &     0.11 &     0.12 &  $-$0.23 &   \ldots &  $-$3.60 &   \ldots &   \ldots &  $-$0.35\tablenotemark{f} &  $-$0.45\tablenotemark{f} &          1 \\
CS~29506-007                         &   21 20 28.7 &$-$20 46 22.9 & 6522 & 3.94 & $-$2.73 & 0 &     0.49 &  $<$0.93 &   \ldots &     0.25 &  $-$0.76 &     0.14 &     0.44 &     0.25 &     0.81 &     0.52 &     0.05 &  $-$0.60 &  $-$2.78 &     0.40 &     0.19 &                      0.13 &                      0.09 &      5, 14 \\
CS~29506-090                         &   21 30 28.9 &$-$22 10 41.4 & 6603 & 4.18 & $-$2.62 & 0 &     0.41 &   \ldots &   \ldots &     0.24 &   \ldots &     0.19 &     0.38 &     0.31 &     0.72 &     0.47 &  $-$0.12 &   \ldots &  $-$2.70 &     0.32 &     0.05 &                      0.27 &  $-$0.35\tablenotemark{f} &          5 \\
HE~2133-1426                         &   21 36 07.2 &$-$14 12 35.4 & 6350 & 4.40 & $-$2.89 & 0 &   \ldots &   \ldots &   \ldots &     0.28 &  $-$0.61 &   \ldots &     0.33 &     0.26 &     0.60 &     0.40 &  $-$0.10 &  $-$0.47 &  $-$2.81 &   \ldots &   \ldots &                   $-$0.14 &                   $-$0.42 &          6 \\
CS~29495-041                         &   21 36 33.3 &$-$28 18 48.6 & 4740 & 1.34 & $-$2.74 & 0 &  $-$0.07 &     0.40 &     0.43 &     0.31 &  $-$0.47 &   \ldots &     0.32 &     0.33 &     0.19 &     0.37 &  $-$0.26 &   \ldots &  $-$2.80 &  $-$0.22 &     0.04 &  $-$0.15\tablenotemark{f} &  $-$0.65\tablenotemark{f} &          7 \\
CS~22948-027                         &   21 37 45.8 &$-$39 27 22.3 & 5011 & 2.06 & $-$2.45 & 1 &     2.12 &     2.43 &     0.71 &     0.20 &   \ldots &   \ldots &     0.68 &   \ldots &     0.91 &     0.44 &  $-$0.03 &   \ldots &  $-$2.36 &   \ldots &   \ldots &                    \ldots &                      2.45 &          3 \\
HE~2135-1924                         &   21 38 04.7 &$-$19 11 04.4 & 6449 & 4.37 & $-$3.31 & 0 &  $<$1.74 &   \ldots &  $-$0.04 &  $-$0.05 &  $-$0.80 &  $-$0.04 &     0.74 &     0.06 &   \ldots &     0.21 &  $-$0.37 &  $-$0.41 &   \ldots &     0.94 &     0.06 &                   $-$0.66 &                   $<$0.00 & This Paper \\
HE~2136-6030                         &   21 40 39.5 &$-$60 16 26.4 & 6409 & 3.85 & $-$2.88 & 0 &  $<$1.71 &   \ldots &  $-$0.39 &     0.08 &  $-$0.64 &     1.21 &     0.51 &   \ldots &   \ldots &     0.40 &  $-$0.19 &   \ldots &  $-$2.64 &   \ldots &   \ldots &                      0.04 &                      0.02 & This Paper \\
BS~17583-100                         &   21 42 27.8 &  +26 40 35.5 & 5950 & 3.66 & $-$2.53 & 0 &     0.53 &   \ldots &   \ldots &     0.08 &  $-$0.88 &   \ldots &     0.28 &   \ldots &     0.48 &     0.33 &  $-$0.21 &  $-$0.61 &  $-$2.62 &     0.26 &     0.13 &                      0.34 &  $-$0.33\tablenotemark{f} &         13 \\
HE~2139-5432                         &   21 42 42.4 &$-$54 18 42.9 & 5416 & 3.04 & $-$4.02 & 1 &     2.59 &     2.08 &     2.15 &     1.61 &     0.36 &     1.00 &   \ldots &   \ldots &   \ldots &     0.31 &     0.34 &   \ldots &  $-$3.52 &     0.62 &     0.17 &                   $-$0.55 &                  $<-$0.33 & This Paper \\
HE~2141-0726                         &   21 44 06.6 &$-$07 12 48.9 & 6551 & 4.26 & $-$2.72 & 0 &  $<$1.55 &   \ldots &  $-$0.36 &     0.06 &  $-$0.87 &  $-$0.05 &     0.16 &     0.07 &   \ldots &     0.25 &  $-$0.08 &  $-$0.54 &  $-$2.53 &   \ldots &     0.17 &                   $-$0.57 &                  $<-$0.37 & This Paper \\
CS~22948-066                         &   21 44 51.2 &$-$37 27 55.0 & 5077 & 2.20 & $-$3.20 & 0 &     0.00 &     1.22 &     0.32 &     0.23 &  $-$0.76 &   \ldots &     0.28 &     0.51 &     0.34 &     0.46 &  $-$0.28 &   \ldots &  $-$2.96 &     0.32 &     0.22 &  $-$0.46\tablenotemark{f} &  $-$0.94\tablenotemark{f} &          7 \\
HE~2142-5656                         &   21 46 20.4 &$-$56 42 19.1 & 4939 & 1.85 & $-$2.87 & 1 &     0.95 &     0.54 &     0.81 &     0.33 &  $-$0.62 &     0.35 &     0.30 &   \ldots &     0.31 &     0.18 &  $-$0.19 &  $-$0.63 &  $-$2.82 &     0.18 &  $-$0.29 &                   $-$0.19 &                   $-$0.63 & This Paper \\
CS~22944-032                         &   21 47 43.2 &$-$13 40 22.8 & 5293 & 2.82 & $-$2.98 & 0 &     0.31 & $<-$0.44 &   \ldots &     0.34 &  $-$0.77 &   \ldots &     0.35 &     0.10 &     0.36 &     0.31 &  $-$0.33 &  $-$0.62 &  $-$3.01 &     0.29 &     0.17 &                   $-$0.13 &                   $-$0.76 &         14 \\
CS~22948-093                         &   21 50 31.5 &$-$41 07 49.3 & 6609 & 4.23 & $-$3.17 & 0 &   \ldots &   \ldots &   \ldots &   \ldots &   \ldots &     0.51 &     0.39 &     0.13 &     0.87 &     0.22 &  $-$0.08 &   \ldots &  $-$3.13 &     0.77 &     0.30 &                   $-$0.09 &                    \ldots &          5 \\
CS~22956-050                         &   21 58 05.8 &$-$65 13 27.1 & 4844 & 1.56 & $-$3.39 & 0 &     0.27 &     0.31 &   \ldots &     0.36 &  $-$0.61 &   \ldots &     0.45 &     0.00 &     0.40 &     0.32 &  $-$0.39 &   \ldots &  $-$3.37 &     0.24 &     0.01 &  $-$0.42\tablenotemark{f} &  $-$0.78\tablenotemark{f} &          7 \\
HE~2158-0348                         &   22 00 40.0 &$-$03 34 12.2 & 5150 & 2.44 & $-$2.57 & 1 &     1.87 &     1.52 &   \ldots &     0.56 &     0.09 &   \ldots &     0.96 &   \ldots &     0.40 &     1.03 &  $-$0.63 &     0.19 &  $-$2.72 &  $-$0.13 &   \ldots &                      0.64 &                      1.75 &         10 \\
BS~17569-049                         &   22 04 58.4 &  +04 01 32.1 & 4645 & 1.09 & $-$2.84 & 0 &  $-$0.12 &     0.86 &     0.59 &     0.19 &  $-$0.31 &   \ldots &     0.32 &     0.28 &     0.24 &     0.38 &  $-$0.20 &   \ldots &  $-$2.85 &  $-$0.12 &     0.08 &     0.31\tablenotemark{f} &     0.20\tablenotemark{f} &          7 \\
HE~2202-4831                         &   22 06 05.8 &$-$48 16 53.0 & 5331 & 2.95 & $-$2.78 & 1 &     2.41 &   \ldots &     1.44 &     0.12 &   \ldots &   \ldots &     0.17 &   \ldots &     0.21 &     0.46 &     0.08 &   \ldots &  $-$2.55 &     0.21 &  $-$0.07 &                   $-$0.85 &                   $-$1.28 & This Paper \\
CS~22965-054                         &   22 06 30.3 &$-$02 32 34.4 & 6137 & 3.68 & $-$3.10 & 0 &     0.62 &   \ldots &   \ldots &     0.36 &  $-$0.52 &     0.08 &     0.38 &     0.16 &     0.52 &     0.31 &  $-$0.22 &  $-$0.33 &  $-$2.95 &     0.26 &  $-$0.02 &                      0.27 & $<-$0.48\tablenotemark{f} &      5, 14 \\
HE~2209-1240                         &   22 11 48.8 &$-$12 25 45.4 & 6319 & 3.84 & $-$2.59 & 0 &   \ldots &   \ldots &   \ldots &     0.45 &  $-$0.35 &     0.26 &     0.34 &     0.08 &   \ldots &     0.37 &  $-$0.11 &  $-$0.49 &  $-$2.63 &     0.37 &     0.16 &                      0.06 &                   $-$0.13 &          9 \\
CS~22892-052                         &   22 17 01.7 &$-$16 39 27.1 & 4825 & 1.54 & $-$3.03 & 1 &     0.90 &     0.51 &     0.24 &     0.25 &  $-$0.52 &   \ldots &     0.21 &     0.27 &     0.15 &     0.22 &  $-$0.38 &  $-$0.44 &  $-$3.05 &  $-$0.03 &  $-$0.11 &                      0.68 &     1.01\tablenotemark{f} &      7, 13 \\
CS~22886-042                         &   22 20 25.8 &$-$10 23 20.2 & 4798 & 1.48 & $-$2.83 & 0 &     0.12 &  $<$2.03 &     0.31 &     0.26 &   \ldots &   \ldots &     0.32 &   \ldots &     0.25 &     0.23 &  $-$0.19 &   \ldots &  $-$2.79 &   \ldots &   \ldots &                    \ldots &                   $-$0.32 &          3 \\
CS~29502-042                         &   22 21 48.8 &  +02 28 44.9 & 5039 & 2.09 & $-$3.27 & 0 &     0.16 &  $-$0.43 &  $-$0.33 &     0.31 &  $-$0.76 &   \ldots &     0.23 &     0.18 &     0.30 &     0.20 &  $-$0.40 &   \ldots &  $-$3.33 &     0.22 &  $-$0.05 &  $-$1.98\tablenotemark{f} &  $-$1.69\tablenotemark{f} &          7 \\
CS~29502-092                         &   22 22 36.0 &$-$01 38 27.5 & 5074 & 2.21 & $-$2.99 & 1 &     0.96 &     0.81 &   \ldots &     0.28 &  $-$0.68 &   \ldots &     0.24 &     0.30 &     0.20 &     0.28 &  $-$0.26 &  $-$0.48 &  $-$2.99 &     0.23 &     0.16 &                   $-$0.15 &                   $-$1.20 &         14 \\
HE~2221-0453                         &   22 24 25.6 &$-$04 38 02.2 & 4430 & 0.73 & $-$2.00 & 1 &     1.83 &     0.84 &   \ldots &   \ldots &   \ldots &   \ldots &     0.74 &   \ldots &     0.44 &     0.34 &   \ldots &   \ldots &  $-$2.00 &   \ldots &   \ldots &                    \ldots &                      1.76 &          3 \\
CS~29516-024                         &   22 26 15.4 &  +02 51 46.3 & 4637 & 1.04 & $-$3.05 & 0 &  $-$0.06 &  $-$0.76 &     0.57 &     0.56 &  $-$0.44 &   \ldots &     0.50 &     0.21 &     0.30 &     0.31 &  $-$0.26 &   \ldots &  $-$3.12 &  $-$0.05 &  $-$0.09 &  $-$0.59\tablenotemark{f} &  $-$0.90\tablenotemark{f} &          7 \\
HE~2228-0706                         &   22 31 24.5 &$-$06 50 51.2 & 5003 & 2.02 & $-$2.78 & 1 &     2.32 &     1.13 &   \ldots &     0.88 &   \ldots &   \ldots &     0.66 &   \ldots &     0.87 &     0.27 &     0.19 &   \ldots &  $-$2.75 &   \ldots &   \ldots &                    \ldots &                      2.46 &          3 \\
HE~2232-0603                         &   22 34 47.4 &$-$05 48 17.3 & 6085 & 3.85 & $-$1.46 & 1 &     1.22 &     0.47 &   \ldots &     0.33 &  $-$0.30 &   \ldots &     0.39 &   \ldots &     0.39 &     0.35 &  $-$0.22 &  $-$0.62 &  $-$1.94 &  $-$0.04 &  $-$0.33 &                      0.59 &                      1.50 &         10 \\
CS~29491-053                         &   22 36 56.3 &$-$28 31 06.5 & 4700 & 1.21 & $-$3.03 & 0 &  $-$0.27 &     0.82 &     0.45 &     0.46 &  $-$0.32 &   \ldots &     0.37 &     0.23 &     0.28 &     0.36 &  $-$0.39 &   \ldots &  $-$3.01 &     0.02 &  $-$0.02 &  $-$0.24\tablenotemark{f} &  $-$0.89\tablenotemark{f} &          7 \\
HE~2246-2410                         &   22 48 59.6 &$-$23 54 39.0 & 6431 & 4.36 & $-$2.96 & 0 &  $<$1.39 &  $<$2.28 &     1.42 &     0.13 &  $-$0.83 &     0.02 &     0.40 &     0.27 &   \ldots &     0.32 &  $-$0.27 &  $-$0.35 &  $-$2.87 &   \ldots &     0.10 &                   $-$0.40 &                  $<-$0.30 & This Paper \\
HE~2247-7400                         &   22 51 19.4 &$-$73 44 23.6 & 4829 & 1.56 & $-$2.87 & 1 &     0.70 &   \ldots &     0.82 &     0.33 &   \ldots &     0.80 &     0.43 &   \ldots &     0.34 &     0.13 &  $-$0.11 &   \ldots &  $-$2.66 &   \ldots &     0.53 &                  $<-$0.15 &                   $-$0.94 & This Paper \\
CD -24$^\circ$ 17504                 &   23 07 20.2 &$-$23 52 35.6 & 6236 & 3.70 & $-$3.38 & 0 &   \ldots &   \ldots &   \ldots &     0.16 &  $-$0.61 &     0.13 &     0.28 &     0.26 &   \ldots &     0.28 &  $-$0.07 &  $-$0.22 &  $-$3.45 &     0.52 &     0.31 & $<-$1.61\tablenotemark{f} & $<-$0.59\tablenotemark{f} &         15 \\
CS~22888-031                         &   23 11 32.5 &$-$35 26 42.9 & 6241 & 4.47 & $-$3.31 & 0 &     0.38 &   \ldots &   \ldots &     0.34 &   \ldots &     0.36 &     0.44 &     0.42 &     0.78 &     0.62 &  $-$0.05 &   \ldots &  $-$3.28 &     0.53 &     0.20 &                   $-$0.14 &                    \ldots &          5 \\
CS~30338-089                         &   23 15 50.0 &  +10 19 26.2 & 4886 & 1.72 & $-$2.78 & 1 &     2.06 &     1.27 &     0.61 &     0.19 &   \ldots &   \ldots &     0.60 &   \ldots &     0.40 &     0.66 &     0.11 &   \ldots &  $-$2.76 &   \ldots &   \ldots &                    \ldots &                      2.30 &          3 \\
HE~2323-0256                         &   23 26 29.8 &$-$02 39 57.9 & 4958 & 1.84 & $-$3.97 & 1 &     1.06 &     2.16 &     2.10 &     1.38 &     0.02 &   \ldots &     0.39 &     0.29 &     0.45 &     0.45 &  $-$0.37 &  $-$0.87 &  $-$3.86 &     0.37 &  $-$0.10 &                      0.55 &                   $-$0.52 &      7, 11 \\
HE~2330-0555                         &   23 32 54.8 &$-$05 38 50.6 & 4867 & 1.65 & $-$2.98 & 1 &     2.09 &     1.00 &     0.81 &     0.34 &   \ldots &   \ldots &     0.45 &   \ldots &     0.35 &     0.29 &  $-$0.03 &   \ldots &  $-$3.01 &   \ldots &   \ldots &                    \ldots &                      1.17 &          3 \\
CS~22966-011                         &   23 35 07.0 &$-$30 22 54.4 & 6298 & 4.43 & $-$3.02 & 0 &     0.45 &   \ldots &   \ldots &     0.21 &   \ldots &     0.13 &     0.49 &     0.47 &     0.72 &     0.73 &  $-$0.01 &   \ldots &  $-$3.12 &     0.55 &     0.20 &                      0.67 &  $-$0.05\tablenotemark{f} &          5 \\
CS~22952-015                         &   23 37 28.7 &$-$05 47 56.6 & 4824 & 1.50 & $-$3.44 & 0 &  $-$0.41 &     1.31 &   \ldots &  $-$0.13 &  $-$0.48 &   \ldots &     0.24 &  $-$0.01 &     0.20 &     0.14 &  $-$0.45 &  $-$0.59 &  $-$3.33 &     0.11 &  $-$0.08 &                   $-$0.52 &  $-$1.33\tablenotemark{f} &      7, 13 \\
HE~2341-2029                         &   23 44 19.6 &$-$20 13 19.8 & 6507 & 4.29 & $-$2.60 & 0 &   \ldots &   \ldots &   \ldots &     0.31 &  $-$0.72 &     0.33 &     0.39 &     0.38 &     0.72 &     0.49 &  $-$0.14 &  $-$0.55 &  $-$2.48 &     0.58 &  $-$0.08 &                      0.00 &                   $-$0.43 &          9 \\
CS~29522-046                         &   23 44 59.9 &  +08 46 52.9 & 5974 & 3.72 & $-$2.12 & 0 &     0.42 &  $-$0.33 &   \ldots &     0.24 &   \ldots &   \ldots &     0.40 &     0.02 &     0.36 &     0.33 &  $-$0.14 &  $-$0.63 &  $-$2.22 &     0.00 &     0.01 &                      0.33 &                   $-$0.13 &         14 \\
HE~2344-2800                         &   23 46 44.4 &$-$27 44 10.7 & 6624 & 4.11 & $-$2.65 & 0 &   \ldots &   \ldots &   \ldots &     0.04 &  $-$0.73 &   \ldots &     0.21 &     0.04 &     0.76 &     0.68 &     0.27 &     0.12 &  $-$2.67 &   \ldots &   \ldots &                   $-$0.08 &                   $-$0.37 &          6 \\
CS~22966-057                         &   23 48 57.8 &$-$29 39 22.9 & 5364 & 3.07 & $-$2.43 & 0 &     0.06 &     0.10 &     0.61 &  $-$0.02 &  $-$0.72 &   \ldots &     0.22 &     0.27 &     0.28 &     0.43 &  $-$0.05 &   \ldots &  $-$2.50 &     0.14 &     0.24 &  $-$0.10\tablenotemark{f} &  $-$0.24\tablenotemark{f} &          7 \\
CS~29499-060                         &   23 53 40.3 &$-$26 58 44.0 & 6595 & 4.05 & $-$2.50 & 0 &     0.38 &   \ldots &   \ldots &  $-$0.01 &   \ldots &     0.05 &  $-$0.06 &   \ldots &     0.33 &   \ldots &   \ldots &   \ldots &  $-$2.66 &     0.19 &  $-$0.21 &                   $-$0.63 &                    \ldots &          5 \\
HE~2356-0410                         &   23 59 13.1 &$-$03 53 48.2 & 5170 & 2.45 & $-$3.19 & 1 &     2.27 &     1.75 &   \ldots &     0.30 &  $-$0.10 &   \ldots &     0.45 &   \ldots &     0.40 &     0.52 &  $-$0.17 &  $-$0.10 &  $-$3.01 &     0.22 &   \ldots &                   $-$0.86 &                   $-$0.80 &      1, 10 \\
\enddata

\tablerefs{
1 = \citet{aoki02}; 
2 = \citet{aoki06};
3 = \citet{aoki07}; 
4 = \citet{aoki08}; 
5 = \citet{bonifacio07,bonifacio09}; 
6 = \citet{carretta02,cohen02}; 
7 = \citet{cayrel04,spite05,francois07}; 
8 = \citet{christlieb04}; 
9 = \citet{cohen04}; 
10 = \citet{cohen06}; 
11 = \citet{cohen08}; 
12 = \citet{frebel07}; 
13 = \citet{honda04}; 
14 = \citet{lai08}; 
15 = \citet{norris01}; 
16 = \citet{norris07}; 
%1 = \citet{aoki02};
%2 = \citet{aoki07};
%3 = \citet{aoki08};
%4 = \citet{bonifacio07,bonifacio09}; 
%5 = \citet{carretta02}; 
%6 = \citet{cayrel04,spite05}; 
%7 = \citet{cohen04}; 
%8 = \citet{cohen06}; 
%9 = \citet{cohen08}; 
%10 = \citet{honda04}; 
%11 = \citet{lai08}; 
%12 = \citet{norris01}
}

\tablenotetext{a}{Coordinates are from the 2MASS database \citep{2mass}.}
\tablenotetext{b}{1 = CEMP object, adopting the \citet{aoki07} definition and 0 = C-normal (see Section 7.1 for details).}
\tablenotetext{c}{For literature stars, [C/Fe] and [N/Fe] values are taken from the literature reference.}
\tablenotetext{d}{For this set of results, a dwarf gravity is assumed (see Section 2.1 for details).}
\tablenotetext{e}{For this set of results, a subgiant gravity is assumed (see Section 2.1 for details).}
\tablenotetext{f}{These abundances, or limits, were taken from the literature source.} 

\end{deluxetable} 


